Graphical combinatorics and a distributive law for modular operads

This work presents a detailed analysis of the combinatorics of modular operads. These are operad-like structures that admit a contraction operation as well as an operadic multiplication. Their combinatorics are governed by graphs that admit cycles, and are known for their complexity. In 2011, Joyal and Kock introduced a powerful graphical formalism for modular operads. This paper extends that work. A monad for modular operads is constructed and a corresponding nerve theorem is proved, using Weber's abstract nerve theory, in the terms originally stated by Joyal and Kock. This is achieved using a distributive law that sheds new light on the combinatorics of modular operads.

==> 0322Macros.tex <==

\newcommand\B{\mathcal{B}}
\newcommand\Gconn{\mathcal{G}_{\mbox{conn}}}
\newcommand\Bconn{\mathcal{B}_{\mbox{conn}}}
\newcommand\GU{\mathcal{G}_\mathcal{U}}
\newcommand\C{\mathcal{C}}
\newcommand\D{\mathcal{D}}
\newcommand\up{\uparrow}
\newcommand\down{(\downarrow)}
\newcommand\esdown{es^(\downarrow)}
\newcommand\eldown{el^(\downarrow)}

\newcommand\PC{\mathcal P (\mathcal C)}
\newcommand\Open{\mathcal{O}}
\newcommand\E{\mathcal{E}}
\newcommand\bcd{B(\underline c, \underline d)}
\newcommand\g{\tilde {\mathcal G}_0^-}
\newcommand{\defeq}{\overset{\textup{def}}{=}}
\newcommand\0{\bm 0}
\newcommand\U{\mathcal U}
\newcommand\X{\mathcal X}
\newcommand\Y{\mathcal Y}
%\newcommand\{\mathcal{L} }
\newcommand\lt{\mathcal{L} \mathcal{T}}
\newcommand\CC{\textswab C}
%\newcommand\DD{\textswab D}
\newcommand\II{\textswab I}
\newcommand\OO{\textswab O}
\newcommand\whe{\circlearrowleft}
\newcommand\PP{\mathcal {P}}
\newcommand\tm{\mathcal{T}}
\newcommand\GS{\mathsf {GS}}
\newcommand\GG{\mathbf {GG}}


\newcommand\Grsim{\mathsf{Gr}_{sim}}
\newcommand\Tsim{T_{sim}}
\newcommand\Grsimp{\mathsf{Gr}_{sim_*}}
\newcommand\Graug{\mathsf{Gr}^\bot_{sim*}}
\newcommand\Mod{\mathbf {Mod}}
%\newcommand\MO{\mathsf {MO}}
\newcommand\CSM{\mathsf {MO}}
%\newcommand\MO{\mathsf {MO}}
\newcommand\CO{\mathsf {CO}}
\newcommand{\Comp}{\mathsf{Comp}}
\newcommand\nuCSM{\mathsf {MO}^-}
\newcommand\Klgr{\Xi}%{\widetilde{\mathsf{\Gr}_*}}
\newcommand\trdown{\mathsf {Tr}^{(\downarrow)}}
\newcommand\trds{\mathsf {Tr}^{(\downarrow), *}}


\newcommand\modx{\mathcal {\mathbf {X}}}
%%%%TIKX
\tikzset{->-/.style={decoration={
			markings,
			mark=at position #1 with {\arrow{>}}},postaction={decorate}}}
\tikzset{-<-/.style={decoration={
			markings,
			mark=at position #1 with {\arrow{<}}},postaction={decorate}}}

\newcommand{\multiplication}{ \draw[thick](0,0)--(0,-2)
	(0,0)--(-1.5,2)
	(0,0) --( 0,2)
	(0,0)--(1.5,2)
	(0,2)--(-1,4)
	(0,2)--(-.5,4)
	(0,2)--(1,4)
	;
	
	\node at (.3,1){\tiny{c}};
	
	\draw[dashed]
	(-.3,4)--(.8,4);
	
	\draw[decoration={brace, raise=5pt},decorate]
	(-1,4) -- node[above=6pt] {\small{$X$}} (1,4);
	%					
	
	%\draw[decoration={brace,raise=5pt},decorate]
	%  (-1.5,2.1) -- node[above=6pt] {\small{$n$ inputs}} (1.5,2.1);
	
	\draw  [ draw=red,   fill=white]
	(0,2)circle (15pt)
	(0,-0) circle (15pt);
	
	\node at(0,0) {\small{$\phi_1 $}};
	\node at(0,2) {\small{$\phi_2 $}};
	
}


\newcommand{\product}{ \draw[thick](0,0)--(0,-2)
	(0,0)--(-1.5,2)
	%(0,0) --( 0,2)
	(0,0)--(1.5,2)
	(0,0)--(-1,2.2)
	(0,0)--(-.5,2.2)
	(0,0)--(1,2.2);
	
	\draw[dashed]
	(-.3,2.2)--(.8,2.2);
	
	\draw[decoration={brace, raise=5pt},decorate]
	(-1.5,2.5) -- node[above=6pt] {\small{$n\amalgm-1$}} (1.5,2.5);
	
	
	%\draw[decoration={brace,raise=5pt},decorate]
	%  (-1.5,2.1) -- node[above=6pt] {\small{$n$ inputs}} (1.5,2.1);
	
	\draw  [ draw=red,   fill=white]
	(0,0) ellipse (30pt and 15 pt);
	
	\node at(0,0) {\small{$\phi_1 \square_2 \phi_2 $}};
}

%%FRONTMATTER
%%%%%NOTATION SECTION
%%%SETS
\newcommand\CCC{\mathfrak{C}}
\newcommand\DDD[1][D]{\mathfrak{#1}}
%%%Directed stuff
%\newcommand{\Cor}{\mathcal{Cor}}% For directed rooted corollas for rooted trees.. 
\newcommand\Di{\mathfrak{Di}}% \{\In, \Out\}
\newcommand\DiD[1][\mathfrak D]{{{#1}^{Di}}}%\DDD \times \Di
\newcommand{\Disig}{\sigma_{\Di}}% involution on \Di
\newcommand{\DisigD}[1][\DDD]{\sigma^{#1}_{\Di}}% involution on \DiD
\newcommand{\Dipal}{(\Di, \sigma_{\Di})}%
\newcommand{\DipalD}[1][\DDD]{({#1} \times \Di,\sigma^{#1}_{\Di})}%
\newcommand{\DiGS}{\overrightarrow{\GS}}% Directed species
\newcommand{\DDiGS}[1][\mathfrak D]{{\overrightarrow{\GS}}^{#1}}%\DDD coloured directed


\newcommand{\mm}[1][m]{\mathbf{#1}}
\newcommand{\nul}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\two}{\mathbf{2}}
\newcommand{\nn}{\mathbf{n}}

%%CATEGORIES 
\newcommand\Set{\mathsf{Set}}
\newcommand\Cat{\mathsf {Cat}}
\newcommand\fin{\mathsf{Set_f}}
\newcommand\sSet{\mathsf{sSet}}
\newcommand{\prs}[1]{\mathsf{ps_{\sSet}}(#1)}
\newcommand{\fiso}{{\mathbf{B}}}%{{\mathsf{Bij}}}%{\mathbb {P}}%NEED BETTER NOTATION HERE...
\newcommand{\fisinv}{{\fiso}^{\circlearrowleft}}%{\mathbb{P}^\circlearrowleft}
\newcommand{\fisinvdi}{{(\fiso \times \fiso^{\mathrm{op}})^{\downarrow}}}
\newcommand{\Bifiso}{{\fiso^{\downarrow}}}%{{\fiso}^{(\downarrow) }}


%%Rooted trees
\newcommand{\Tr}[1][T]{\mathbf{#1}}

%%Monads 
\newcommand{\TT}{\mathbb T}
\newcommand{\TTp}{\mathbb T_*}
\newcommand{\DD}{\mathbb D}
\newcommand{\LL}{\mathbb L}
%\newcommand{\PProd}{\mathbb P}
\newcommand{\Sbold}{{\mathbf{S}}}
\newcommand{\GSbold}[1]{{\mathbf{#1}}}

%partial maps
%\newcommand\pto{\mathrel{\ooalign{\hfil$\mapstochar$\hfil\cr$\to$\cr}}}
\newcommand\pto{\rightharpoonup}

%%%prehseaf category $\mathsf C^\mathrm{op} \to \Set$
\newcommand{\pr}[1]{\mathsf{ps}(#1)}
\newcommand{\sh}[1]{\mathsf{sh}(#1)}
%maximal subgroupoid
\newcommand{\iso}[1]{{#1}_{iso}}

%%Functor category
\newcommand{\Fun}[1][\mathsf C, \mathsf D]{\mathsf{Fun}(#1)}

%%%Curve arrows
\newcommand{\CricArrowRight}[1]{%
	\setlength{\@Si(\Di, \sigma_{\Di})eOfCirc}{\maxof{\widthof{#1}}{\heightof{#1}}}%
	\tikz [x=1.0ex,y=1.0ex,line width=.15ex, draw=black]%
	\draw [->,anchor=center]%
	node (0,0) {#1}%
	(0,1.2\@SizeOfCirc) arc (-90:180:1.2\@SizeOfCirc);%
}%
\newcommand \inv{%
	\tikz{ [x=1.0ex,y=1.0ex,line width=.15ex, draw=black]%
		\draw [<->,anchor=center]%
		node (0,0)%
		(0,1.2) arc (-90:180:1.2);}%
}%


%%%Profunctor notation (from nlab)
\makeatletter
\def\slashedarrowfill@#1#2#3#4#5{%
	$\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
	\relax#5#1\mkern-7mu%
	\cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
	\mathclap{#3}\mathclap{#2}%
	\cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
	\mkern-7mu#4$%
}
\def\rightslashedarrowfill@{%
	\slashedarrowfill@\relbar\relbar\mapstochar\rightarrow}
\newcommand\xslashedrightarrow[2][]{%
	\ext@arrow 0055{\rightslashedarrowfill@}{#1}{#2}}
\makeatother

\def\proarrow{\xslashedrightarrow{}}



%%quotient notation
\newcommand\quotient[2]{
	\mathchoice
	{% \displaystyle
		\text{\raise1ex\hbox{$#1$}\Big/\lower1ex\hbox{$#2$}}%
	}
	{% \textstyle
		#1\,/\,#2
	}
	{% \scriptstyle
		#1\,/\,#2
	}
	{% \scriptscriptstyle  
		#1\,/\,#2
	}
}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\newcommand\alert[1]{\marginpar{\warn{\scriptsize{#1}}}}
%%GRAPH CATEGORIES
%%%%Defining connectedness and establishing universal properties
\newcommand{\diag}{\mathsf{\mathtt D}}
\newcommand{\GrShape}{\mathsf{ps_f}(\mathtt D)}

\newcommand\Gr{\mathsf{CetGr}}
%\newcommand\el{\mathsf{elGr}}
\newcommand{\Grbig}{\mathsf{Gr}\GrShape}
\newcommand{\Gret}{\mathsf{etGr}}
\newcommand{\Griso}{\mathsf{CGr_{iso}}}

%%% GRAPH NOTATION
%$$$GRAPH NOTATION
\newcommand\G{\mathcal{G}}
\renewcommand\H{\mathcal{H}}
\newcommand\W{\mathcal W}
\newcommand\I{\mathcal{I}}
%%%line and wheel graphs
\newcommand{\Lk}[1][k]{\ensuremath{\mathcal L^{#1}}}
\newcommand{\Wl}[1][m]{\ensuremath{\mathcal W^{#1}}}
\newcommand{\Wm}[1][m]{\ensuremath{\mathcal W^{#1}}}


\newcommand{\EI}{\ensuremath{{E_\bullet}}}


%%%%Gradings
\newcommand{\vH}[1][v]{\sfrac{H}{#1}}
\newcommand{\vE}[1][v]{\sfrac{E}{#1}}
\newcommand{\nV}[1][n]{V_{#1}}
\newcommand{\nH}[1][n]{H_{#1}}
\newcommand{\nE}[1][n]{E_{#1}}

%1. Graph with index
\newcommand{\Gn}[1]{\ensuremath{\mathcal G^{#1}}}
\newcommand{\En}[1]{\ensuremath{E^{#1}}}
\newcommand{\Hn}[1]{\ensuremath{H^{#1}}}
\newcommand{\Vn}[1]{\ensuremath{V^{#1}}}
\newcommand{\sn}[1]{\ensuremath{s^{#1}}}
\newcommand{\tn}[1]{\ensuremath{t^{#1}}}
\newcommand{\taun}[1]{\ensuremath{\tau^{#1}}}

%1. Component of a graph
\newcommand{\Gc}[1][c]{\ensuremath{\mathcal G^{#1}}}
\newcommand{\Ec}[1][c]{\ensuremath{E^{#1}}}
\newcommand{\Hc}[1][c]{\ensuremath{H^{#1}}}
\newcommand{\Vc}[1]{\ensuremath{V^{#1}}}
%\newcommand{\sn}[1]{\ensuremath{s^{#1}}}
%\newcommand{\tn}[1]{\ensuremath{t^{#1}}}
%\newcommand{\taun}[1]{\ensuremath{\tau^{#1}}}

% 2. Graph associated to set $W \subset V$
\newcommand{\GWbot}[1][W]{\ensuremath{\mathcal G^{\bot(#1)}}}
\newcommand{\GW}[1][W]{\ensuremath{\mathcal G^{(#1)}}}
\newcommand{\XW}[1][W]{\ensuremath{X^{(#1)}}}
\newcommand{\XWbot}[1][W]{\ensuremath{X^{\bot(#1)}}}
\newcommand{\EW}[1][W]{\ensuremath{E^{(#1)}}}
\newcommand{\EWbot}[1][W]{\ensuremath{E^{\bot(#1)}}}
\newcommand{\HW}[1][W]{\ensuremath{H^{(#1)}}}
\newcommand{\HWbot}[1][W]{\ensuremath{H^{\bot(#1)}}}
\newcommand{\VWbot}[1][W]{\ensuremath{V^{\bot(#1)}}}
\newcommand{\VW}[1][W]{\ensuremath{V^{(#1)}}} % = W
\newcommand{\sW}[1][W]{\ensuremath{s^{(#1)}}}
\newcommand{\tW}[1][W]{\ensuremath{t^{(#1)}}}
\newcommand{\tauW}[1][W]{\ensuremath{\tau^{(#1)}}}

% 3. Corolla associated to a set

\newcommand\CX[1][X]{{\mathcal C_{#1}}}
%\newcommand{\Gn}[1]{\ensuremath{\mathcal G^{#1}}}
\newcommand{\EX}[1][X]{\ensuremath{E^{#1}}}
\newcommand{\HX}[1][X]{\ensuremath{H^{#1}}}
\newcommand{\VX}[1][X]{\ensuremath{V^{#1}}}
\newcommand{\sX}[1][X]{\ensuremath{s_{#1}}}
%\newcommand{\tX}[1]{\ensuremath{t^{#1}}}
\newcommand{\tauX}[1][X]{\ensuremath{\tau_{#1}}}

% 4. Corolla associated to a vertex
\newcommand\Cv[1][v]{{\mathcal C_{\mathbf{#1}}}}
%\newcommand{\Gn}[1]{\ensuremath{\mathcal G^{#1}}}
%\newcommand{\En}[1]{\ensuremath{E^{#1}}}%\newcommand{\Hn}[1]{\ensuremath{H^{#1}}}
%\newcommand{\Vn}[1]{\ensuremath{V^{#1}}}
\newcommand{\sv}[1][v]{\ensuremath{s_{(#1)}}}
%\newcommand{\tX}[1]{\ensuremath{t^{#1}}}
\newcommand{\tauv}[1][v]{\ensuremath{\tau_{(#1)}}}

% 5. stick associated to an edge orbit
\newcommand\shorte[1][\tilde e]{{\shortmid_{#1}}}
\newcommand{\taue}[1][\tilde e]{\ensuremath{\tau_{(#1)}}}


%5. maps associated to a graph
%\newcommand{\Gn}[1]{\ensuremath{\mathcal G^{#1}}}
\newcommand{\EG}[1][\shortmid]{\ensuremath{E^{(#1)}}}
%\newcommand{\Hn}[1]{\ensuremath{H^{#1}}}
%\newcommand{\Vn}[1]{\ensuremath{V^{#1}}}
\newcommand{\sG}[1]{\ensuremath{s^{(#1)}}}
\newcommand{\tG}[1]{\ensuremath{t^{#1}}}
\newcommand{\tauG}[1][\shortmid]{\ensuremath{\tau_{#1}}}
\newcommand{\qG}[1]{\ensuremath{q^{(#1)}}}

%%%%CATEGORIES OF GRAPHS
%%category associated to a graph
\newcommand\cat[1][\G]{\ensuremath{\ldbrack #1\rdbrack}}




%%%graph morphisms and components of natural transformations $in_x^{\CX}$.
\newcommand{\xin}[2][x]{\ensuremath{ch_{#1}^{#2}}} % e.g. ip_x^\G$
\newcommand{\xout}[2][x]{\ensuremath{ch_{#1}^{#2}}\circ \taue}

%Monads and free and forgetful functors
%% Review monad noation to reflect base category....
\newcommand{\OOO}{\mathbb {O}}
\newcommand{\MM}{\mathbb {M}}
\newcommand{\MMop}{\MM_{\mathsf{Op}}}%^\mathrm{OP}}
\newcommand{\Mop}{ M_{\mathsf{Op}}}
\newcommand{\Fop}{ {F}_{\mathsf{Op}}}
\newcommand{\Uop}{ {U}_{\mathsf{Op}}}
\newcommand{\MMcat}{\mathbb {M}_{\mathsf{Cat}}}
\newcommand{\Mcat}{ {M}_{\mathsf{Cat}}}
\newcommand{\Fcat}{ {F}_{\mathsf{Cat}}}
\newcommand{\Ucat}{ {U}_{\mathsf{Cat}}}

%categories
%%slice
\newcommand{\ov }{/}

%%%%% SECTION 2 ESSENTIAL
% essential category of $\G$. Contained in $\el$
\newcommand{\esG}[1][\mathcal{G}]{\ensuremath{\mathsf{es}{(#1)}}}
\newcommand{\esx}[1][x]{\ensuremath{\iota_{#1}}}
\newcommand{\esv}[1][v]{\ensuremath{\iota_{{#1}}}}
\newcommand{\ese}[1][e]{\ensuremath{\iota_{\tilde{#1}}}}%{\ensuremath{\mathbf{\tilde{#1}}}}
\newcommand{\esh}[1][h]{\ensuremath{\delta_{{#1}}}} %WARN: Is $\kappa$ a good choice?
\newcommand{\esH}[1]{\ensuremath{\delta_{#1}}}
\newcommand{\iG}[2][]{\ensuremath{i_{#1}^{#2}}}

%%%%% CATEGORIES OF ELEMENTS
% category of elements of $\G$
\newcommand{\elG}[1][\mathcal{G}]{\ensuremath{\mathsf{el}{(#1)}}}
\newcommand{\ElP}[2]{\ensuremath{\mathsf{El}_{#1}{(#2)}}}
% canonical functor $\cat[\G] \to \el$
\newcommand{\esdownG}[1][\mathcal{G}]{\ensuremath{{es}^(\downarrow){(#1)}}}

%%%% FUNCTORS DEFINING EQUIVALENCES.
\newcommand{\yet}{\Upsilon}
\newcommand{\yetp}{{\yet_*}}
% $\elG \to \esG$
\newcommand{\res}[2][\mathcal{G}]{\ensuremath{\lfloor #2\rfloor}^{#1}}
\newcommand{\fres}[1][\mathcal{G}]{\ensuremath{r^{f\ es}_{#1}}}
%%POINTED
\newcommand{\resp}[2][\mathcal{G}]{\ensuremath{\lfloor #2\rfloor}^{#1}_*}

%%%%%%SECTION 3 GLUING%%%%%%%%%%
%1. $\G$-indexed graph of graphs
\newcommand\Gg{\mathbf \Gamma}
\newcommand\Gdg{\mathbf \Lambda}
%%colimit of $\Gg$
\newcommand\coGg[1][\G]{{\Gg}({#1})}%{\overline{\Gg}}
\newcommand\coGgvar[2][\G]{\overline{\Gg^{#2}}} %% \Gg^1(\G)
\newcommand\GSg[1][S]{\mathbf \Gamma_{#1}}
%\newcommand\coGSg[1][\G]{{#1}^{\Gg}}

%%%%%%%
%core inclusion
\newcommand{\corei}[1][\G]{\ensuremath{ i^\bullet_{#1}}}


%%%%%%%%%%%SECTION 4 SPECIES
\newcommand{\CGS}[1][(\CCC,\omega)]{{\GS^{#1}}}

\newcommand{\Comm}{{K}}
\newcommand{\CComm}[2][(C,\omega)]{{{\Comm}^{#1}_{#2}}}

%%%%%%%%%%%
%GRAPHS OF GRAPHS
%%%%%%%%%%%

%%S-graph of graphs $\Gg_S$ NOTHING MORE COMPLICATED\
%%%%colimits of S-graph of graphs
\newcommand{\coGgS}[1][\G]{\overline{\Gg_S}}
\newcommand{\coGgSvar}[2][\G]{\overline{\Gg_{#2}}}


\newcommand{\comC}{\mathsf{comp}}
%%%%%%
\newcommand{\CMO}[1][(C,\omega)]{{\MO^{#1}}}
\newcommand{\CCSM}[1][(C,\omega)]{{^{#1}MO}}
\newcommand{\CCat}{ \mathsf{C}}
\newcommand{\DCat}[1][D]{ \mathsf{#1}}
\newcommand{\Op}{ \mathsf{Op}}
\newcommand{\boffcat}[1][\MM, \DCat]{ \Theta_{#1}}

%\newcommand{\CGSp}[1][C^\omega][1][C^\omega]{(#1)\GS_*}

%%%2.3
\newcommand{\CEl}[1][(C,\omega)]{{^{#1}El}}

%listed \underline c C,\omega graphs




%%%%%
%degnerate $\W$-shaped graph of $S$-graphs $\mathbf O_S^c$
\newcommand{\TJK}{T^{{(\shortmid)}}}
\newcommand{\muJK}{\mu^{(\shortmid)}}
\newcommand{\etaJK}{\eta^{(\shortmid)}}
\newcommand{\XGrJK}[1][X]{{#1}\Griso^{(\shortmid)}}

%%%SECTION 2%%%%%%%%%%%
\newcommand{\CGSp}[1][(C,\omega)]{{\GSp^{#1}}}
%\newcommand{\CCommp}[1][C^\omega]{(#1)Comm}

%%%%Section 3
\newcommand{\uG}[2][]{\ensuremath{ch_{#2} \circ u}}
\newcommand{\zG}[2][]{\ensuremath{ch_{#2} \circ z}}
\newcommand{\kappaG}[2][]{\ensuremath{ch_{#2} \circ \kappa}}
%%vertexdeletion stuff

%%%pointed graph of graphs 
%\newcommand{\Ggp}{\Gg_*}
%\newcommand{\coGgp}[1][\G]{\Ggp(\G)}

%%%vertex deletion
%6. deleting a vertex
\newcommand{\Gnov}[1][W]{\ensuremath{\mathcal G_{/#1}}}
\newcommand{\Enov}[1][W]{\ensuremath{E_{/#1}}}
\newcommand{\Hnov}[1][W]{\ensuremath{H_{/#1}}}
\newcommand{\Vnov}[1][W]{\ensuremath{V_{/#1}}}
\newcommand{\snov}[1][W]{\ensuremath{s_{/#1}}}
\newcommand{\tnov}[1][W]{\ensuremath{t_{/#1}}}
\newcommand{\taunov}[1][W]{\ensuremath{\tau_{/#1}}}
\newcommand{\delW}[1][W]{\mathsf{del}_{/#1}}



%%%%1. $\G$-indexed graph of pointed graphs
\newcommand\Gpg[1][]{{\Gg_*^{#1}}} % e.g. \Gpg[1], etc
%\newcommand\coGpg[1][\G]{\Gg_*(\G)}
%\newcommand\coGpgvar[2][\G]{\Gg_{*#2}(#1)} %% \Gg^1(\G)
%\newcommand{\GpgS}[
%\newcommand{\coGpgS}[1][\G]{\Gg_{*S}(#1)}
%\newcommand{\coGpgSvar}[2][S]{\Gg_{*#1}^{#2}}



%%%% Special constructions

\newcommand{\elup}{\el^{\uparrow}}

\newcommand{\DiGSD}[1][D]{\DiGS^{#1}}
\newcommand{\Tdloop}{T^\circlearrowleft}
\newcommand{\mudloop}{\mu^\circlearrowleft}
\newcommand{\etadloop}{\eta^\circlearrowleft}

%\newcommand\Ggv[2][\G]{\mathbf {G}_{#1, #2}}

%\newcommand\iGg[2][{\Gg{\G}}]{u_{#1}^{#2}}
%%%Category of non-deg $\G$-ind graphs of connected graphs
\newcommand{\GrG}[1][\G]{\ensuremath{\Gr^{(#1)}}}

%%%4. Graphs of structured graphs REWORK THIS...
%\newcommand\GSgj[2][S]{\mathbf {G}^{#1}_{(#2)}}
%%\newcommand\GSg[2][\G]{{\mathbf {G}_{#1}^{#2}}}
%%%CHECK THROUGH FOR ALL CHANGES....
%\newcommand\GSg[2][\G]{{\Xi^{#2}}}
%%%Category of non-deg $\G$-ind graphs of connected graphs
\newcommand{\GrSG}[1][\G]{\ensuremath{\Gr^{(#1)}(S)}}
\newcommand{\GrSGvar}[2][\G]{\ensuremath{\Gr^{(#1)}(#2)}}

%%%%%GROTHENDIECK TOPOLGIES
\newcommand{\sieve}[1][\elG]{\ensuremath{\langle #1 \rangle}}

%%%%Symmetric collections
\newcommand{\Coll}[1][(\CCC, \omega)]{\mathsf{Coll}^{#1}}
\newcommand{\DiColl}[1][D]{\mathsf{DiColl}^{#1}}
\newcommand{\DProp}[1][D]{\mathsf{Prop}_\circlearrowleft^{ #1}}
%%%%%Totally labelled graphs
%\newcommand{\Tl}{\mathsf{Tl}\Gr_{iso}}
%\newcommand{\voTl}[1][k]{\mathsf{Tl}\Gr^{\mathbf{#1}vo}_{iso}}
%\newcommand{\Td}{\mathsf{Di}\Gr^D_{iso}}
% \newcommand{\DiGr}[1][(\ccc;\ddd)]{{#1}\mathsf{DiGr}_{iso}^D}
%  \newcommand{\DiGrloop}[1][(\ccc;\ddd)]{{#1}\mathsf{DiGr}_{iso}^{\circlearrowleft D}}
%  \newcommand{\Wloop}[1][D]{ W^{\circlearrowleft{#1}}}
%    \newcommand{\muloop}[1][D]{ \mu^{\circlearrowleft{#1}}}
%        \newcommand{\etaloop}[1][D]{ \eta^{\circlearrowleft{#1}}}
%            \newcommand{\hloop}{ h^{\circlearrowleft}}
% \newcommand{\DiGrvar}[2]{{#1}\mathsf{DiGr}_{iso}^{#2}}
% \newcommand{\DiGS}{\mathsf{DiGS}}

%%%%%%%%strictly undirected things%%%%%%
% \newcommand{\Tud}{T_{ud}}
% \newcommand{\muud}{\mu_{ud}}
% \newcommand{\etaud}{\eta_{ud}}
% \newcommand{\hud}{h_{ud}}
%%%%%%%%%%%%%%%%%%
%%%POINTED GRAPHS
%%%%%%%%%%%%%%%%%%
\newcommand{\elp}{\ensuremath{\mathsf{elGr}_*}}
\newcommand{\Grp}{\ensuremath{\mathsf{\Gr}_*}}
\newcommand{\GSp}{\ensuremath{\mathsf{\GS}_*}}
\newcommand{\Gretp}{\ensuremath{\Gret_{*}}}
\newcommand{\fisinvp}{\ensuremath{\fisinv_*}}



% category of pointed elements of $\G$
\newcommand{\elpG}[1][\mathcal{G}]{\ensuremath{\mathsf{el}_*{(#1)}}}
% essential pointed category of $\G$. Contained in $\elp$
\newcommand{\espG}[1][\mathcal{G}]{\ensuremath{\mathsf{es}_*{(#1)}}}
% Category of essential pointed elements of $\G$. canonically iso to $\espG$
\newcommand{\esdownpG}[1][\mathcal{G}]{\ensuremath{\mathsf{es}_*^(\downarrow){(#1)}}}

\newcommand{\sievep}[1][\elpG]{\ensuremath{\langle #1 \rangle}}
\newcommand{\sieveG}[1][\G]{\mathcal {El}(#1)}

\newcommand{\mup}{\ensuremath{\mu^{\TTp}}}
\newcommand{\etap}{\ensuremath{\eta^{\TTp}}}
\newcommand{\Tp}{\ensuremath{T_*}}
%\newcommand{\Tpo}{\ensuremath{T_{p.o.}}}

\newcommand{\EsdownpG}[1][\mathcal{G}]{\ensuremath{Es^(\downarrow)_{#1*}}}


%Category of locally linear/minimal graphs
\newcommand{\Grll}{\ensuremath{\Gr_*^{0,2}}}
%1. pointed $\G$-indexed graph of graphs
%\newcommand{\Gpg}[1][\mathcal G]{\mathbf {G}_{#1*}}


%%%%%%%%%%%%
%%natural transformation $C9-,c) \Rightarrow F$ associated with an element $x \in F(c)$ #1 is x
\newcommand{\nt}[1][\alpha]{(#1)^{(\downarrow)}}


\newcommand{\In}{{\mathrm{ in }}}
\newcommand{\Out}{{\mathrm{ out }}}
%%%%%%%%%%%
%POINTED GRAPHS OF GRAPHS
%%%%%%%%%%%
%%1. $\G$-indexed graph of graphs
%\newcommand\Gpg[1][\mathcal G]{\mathbf {G}_{#1*}}
%%2. $\esG$ component of a $\G$-indexed graph of graphs
%\newcommand\Gpgv[2][\overline{\Gg{\G}}]{(\overline{#1})_{#2}}
%%3.canonical map from $\esG$ component  to colimit
%%notice that this is closely related to $\iG$. Why is this justified?
%\newcommand\iGpg[2][\overline{\Gg{\G}}]{i_{#1}^{#2}}
%%%%category of $\G$-indexed non-deg pointed graphs of graphs
\newcommand{\GrpG}[1][\G]{\ensuremath{\Grp^{(#1)}}}

%%4. Graphs of structured graphs 
%\newcommand\GSpgj[2][S]{\mathbf {G}^{#1}_{(#2)}}

%2. $\esG$ component of a $\G$-indexed graph of graphs
%\newcommand\Ggv[2][\overline{\Gg{\G}}]{(\overline{#1})_{#2}}
%3.canonical map from $\esG$ component  to colimit
%notice that this is closely related to $\iG$. Why is this justified?
%\newcommand\iGg[2][\overline{\Gg{\G}}]{i_{#1}^{#2}}

%%%Category of non-deg $\G$-ind pointed graphs of connected graphs
\newcommand{\GrpSG}[1][\G]{\ensuremath{\Grp^{(#1)}(S)}}
\newcommand{\GrpSGvar}[2][\G]{\ensuremath{\Gr^{(#1)}(#2)}}


%%%^%normal form
\newcommand{\nor}[1][f]{{#1}_{\text{nor}}}
\newcommand{\esb}[1][f]{{#1}_{\text{es}}}

%%%NERVE THEOREM
%%Factorisation category
%\newcommand{\fact}[1][\beta]{\ensuremath{\text{fact}_{\Grp, \Tp}(#1)}}
\newcommand{\factcat}[1][\beta]{\ensuremath{\mathsf{fact}(#1)}}
\newcommand{\factel}[1][\phi]{\ensuremath{\text{fact}_{\elp, \Tp}(#1)}}
% %%%DIRECTED STUFF
% \newcommand{\eldG}[1][\G, \xi]{\mathsf{el}^\uparrow(#1)}

% %%%%OPERADS STUFF. TO CHANGE
% \newcommand{\UU}{\mathcal {U}}


% %%%%OPERADS
% \newcommand{\Op}[1][(C, \omega)]{\mathcal O^{#1}}
% \newcommand{\OP}[1][(C, \omega)]{\mathcal P^{#1}}

% %domain and target of a morphism
% \newcommand{\sfs}{\mathsf{s}}
% \newcommand{\sft}{\mathsf{t}}

% %%%4. Graphs of structured graphs 
% %\newcommand\GSpgj[2][S]{\mathbf {G}^{#1}_{(#2)}}
% %\newcommand\GSpg[2][S]{\mathbf {G}^{#1}_{#2}}
% %







%\newcommand\GU{\mathcal{G}_\mathcal{U}}
%\newcommand\C{\mathcal{C}}
%\newcommand\D{\mathcal{D}}
%\newcommand\up{\uparrow}
%\newcommand\down{(\downarrow)}
%\newcommand\esdown{es^(\downarrow)}
%\newcommand\eldown{el^(\downarrow)}
%
%\newcommand\PC{\mathcal P (\mathcal C)}
%\newcommand\Open{\mathcal{O}}
%\newcommand\E{\mathcal{E}}
%\newcommand\bcd{B(\underline c, \underline d)}
%\newcommand\g{\tilde {\mathcal G}_0^-}
%\newcommand{\defeq}{\overset{\textup{def}}{=}}
%\newcommand\0{\bm 0}
%\newcommand\U{\mathcal U}
%\newcommand\X{\mathcal X}
%\newcommand\Y{\mathcal Y}
%%\newcommand\{\mathcal{L} }
%\newcommand\lt{\mathcal{L} \mathcal{T}}
%\newcommand\CC{\textswab C}
%%\newcommand\DD{\textswab D}
%\newcommand\II{\textswab I}
%\newcommand\OO{\textswab O}
%\newcommand\whe{\circlearrowleft}
%\newcommand\PP{\mathcal {P}}
%\newcommand\tm{\mathcal{T}}
%\newcommand\GS{\mathsf {GS}}
%\newcommand\GG{\mathbf {GG}}
%
%
%\newcommand\Grsim{\mathsf{Gr}_{sim}}
%\newcommand\Tsim{T_{sim}}
%\newcommand\Grsimp{\mathsf{Gr}_{sim_*}}
%\newcommand\Graug{\mathsf{Gr}^\bot_{sim*}}
%\newcommand\Mod{\mathbf {Mod}}
%%\newcommand\MO{\mathsf {MO}}
%\newcommand\CSM{\mathsf {MO}}
%%\newcommand\MO{\mathsf {MO}}
%\newcommand\CO{\mathsf {CO}}
%\newcommand{\Comp}{\mathsf{Comp}}
%\newcommand\nuCSM{\mathsf {MO}^-}
%\newcommand\Klgr{\Xi}%{\widetilde{\mathsf{\Gr}_*}}
%\newcommand\trdown{\mathsf {Tr}^{(\downarrow)}}
%\newcommand\trds{\mathsf {Tr}^{(\downarrow), *}}
%
%
%\newcommand\modx{\mathcal {\mathbf {X}}}
%%%%%TIKX
%	\tikzset{->-/.style={decoration={
%			markings,
%			mark=at position #1 with {\arrow{>}}},postaction={decorate}}}
%			\tikzset{-<-/.style={decoration={
%					markings,
%					mark=at position #1 with {\arrow{<}}},postaction={decorate}}}
%				
%				
%				\newcommand{\multiplication}{ \draw[thick](0,0)--(0,-2)
%					(0,0)--(-1.5,2)
%					(0,0) --( 0,2)
%					(0,0)--(1.5,2)
%					(0,2)--(-1,4)
%					(0,2)--(-.5,4)
%					(0,2)--(1,4)
%					;
%					
%					\node at (.3,1){\tiny{c}};
%					
%					\draw[dashed]
%					(-.3,4)--(.8,4);
%					
%					\draw[decoration={brace, raise=5pt},decorate]
%					(-1,4) -- node[above=6pt] {\small{$X$}} (1,4);
%%					
%					
%					%\draw[decoration={brace,raise=5pt},decorate]
%					%  (-1.5,2.1) -- node[above=6pt] {\small{$n$ inputs}} (1.5,2.1);
%					
%					\draw  [ draw=red,   fill=white]
%					(0,2)circle (15pt)
%					(0,-0) circle (15pt);
%					
%					\node at(0,0) {\small{$\phi_1 $}};
%					\node at(0,2) {\small{$\phi_2 $}};
%					
%				}
%			
%			
%			\newcommand{\product}{ \draw[thick](0,0)--(0,-2)
%				(0,0)--(-1.5,2)
%				%(0,0) --( 0,2)
%				(0,0)--(1.5,2)
%				(0,0)--(-1,2.2)
%				(0,0)--(-.5,2.2)
%				(0,0)--(1,2.2);
%				
%				\draw[dashed]
%				(-.3,2.2)--(.8,2.2);
%				
%				\draw[decoration={brace, raise=5pt},decorate]
%				(-1.5,2.5) -- node[above=6pt] {\small{$n\amalgm-1$}} (1.5,2.5);
%				
%				
%				%\draw[decoration={brace,raise=5pt},decorate]
%				%  (-1.5,2.1) -- node[above=6pt] {\small{$n$ inputs}} (1.5,2.1);
%				
%				\draw  [ draw=red,   fill=white]
%				(0,0) ellipse (30pt and 15 pt);
%				
%				\node at(0,0) {\small{$\phi_1 \square_2 \phi_2 $}};
%			}
%
%%%FRONTMATTER
%%%%%%NOTATION SECTION
%%%%SETS
%\newcommand\CCC{\mathfrak{C}}
%\newcommand\DDD[1][D]{\mathfrak{#1}}
%%%%Directed stuff
%%\newcommand{\Cor}{\mathcal{Cor}}% For directed rooted corollas for rooted trees.. 
%\newcommand\Di{\mathfrak{Di}}% \{\In, \Out\}
%\newcommand\DiD[1][\mathfrak D]{{{#1}^{Di}}}%\DDD \times \Di
%\newcommand{\Disig}{\sigma_{\Di}}% involution on \Di
%\newcommand{\DisigD}[1][\DDD]{\sigma^{#1}_{\Di}}% involution on \DiD
%\newcommand{\Dipal}{(\Di, \sigma_{\Di})}%
%\newcommand{\DipalD}[1][\DDD]{({#1} \times \Di,\sigma^{#1}_{\Di})}%
%\newcommand{\DiGS}{\overrightarrow{\GS}}% Directed species
%\newcommand{\DDiGS}[1][\mathfrak D]{{\overrightarrow{\GS}}^{#1}}%\DDD coloured directed
%
%
%
%\newcommand{\mm}[1][m]{\mathbf{#1}}
%\newcommand{\nul}{\mathbf{0}}
%\newcommand{\one}{\mathbf{1}}
%\newcommand{\two}{\mathbf{2}}
%\newcommand{\nn}{\mathbf{n}}
%
%%%CATEGORIES 
%\newcommand\Set{\mathsf{Set}}
%\newcommand\Cat{\mathsf {Cat}}
%\newcommand\fin{\mathsf{Set_f}}
%\newcommand\sSet{\mathsf{sSet}}
%\newcommand{\prs}[1]{\mathsf{ps_{\sSet}}(#1)}
%\newcommand{\fiso}{\mathbb {P}}%NEED BETTER NOTATION HERE...
%\newcommand{\fisinv}{\mathbb{P}^\circlearrowleft}
%\newcommand{\Bifiso}{{\fiso}^{(\downarrow) }}
%
%
%%%Rooted trees
%\newcommand{\Tr}[1][T]{\mathbf{#1}}
%
%%%Monads 
%\newcommand{\TT}{\mathbb T}
%\newcommand{\TTp}{\mathbb T_*}
%\newcommand{\DD}{\mathbb D}
%\newcommand{\LL}{\mathbb L}
%%\newcommand{\PProd}{\mathbb P}
%\newcommand{\Sbold}{{\mathbf{S}}}
%\newcommand{\GSbold}[1]{{\mathbf{#1}}}
%
%%%partial maps
%\newcommand\pto{\mathrel{\ooalign{\hfil$\mapstochar$\hfil\cr$\to$\cr}}}
%
%%%%prehseaf category $\mathsf C^{op} \to \Set$
%\newcommand{\pr}[1]{\mathsf{ps}(#1)}
%\newcommand{\sh}[1]{\mathsf{sh}(#1)}
%%maximal subgroupoid
%\newcommand{\iso}[1]{{#1}_{iso}}
%
%%%Functor category
%\newcommand{\Fun}[1][\mathsf C, \mathsf D]{\mathsf{Fun}(#1)}
%
%%%%Curve arrows
%\newcommand{\CricArrowRight}[1]{%
%	\setlength{\@Si(\Di, \sigma_{\Di})eOfCirc}{\maxof{\widthof{#1}}{\heightof{#1}}}%
%	\tikz [x=1.0ex,y=1.0ex,line width=.15ex, draw=black]%
%	\draw [->,anchor=center]%
%	node (0,0) {#1}%
%	(0,1.2\@SizeOfCirc) arc (-90:180:1.2\@SizeOfCirc);%
%}%
%\newcommand \inv{%
%	\tikz{ [x=1.0ex,y=1.0ex,line width=.15ex, draw=black]%
%	\draw [<->,anchor=center]%
%	node (0,0)%
%	(0,1.2) arc (-90:180:1.2);}%
%}%
%
%
%%%%Profunctor notation (from nlab)
%\makeatletter
%\def\slashedarrowfill@#1#2#3#4#5{%
%  $\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
%\relax#5#1\mkern-7mu%
%\cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
%\mathclap{#3}\mathclap{#2}%
%\cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
%\mkern-7mu#4$%
%}
%\def\rightslashedarrowfill@{%
%  \slashedarrowfill@\relbar\relbar\mapstochar\rightarrow}
%\newcommand\xslashedrightarrow[2][]{%
%  \ext@arrow 0055{\rightslashedarrowfill@}{#1}{#2}}
%\makeatother
%
%\def\proarrow{\xslashedrightarrow{}}
%
%
%
%%%quotient notation
%  \newcommand\quotient[2]{
%	\mathchoice
%	{% \displaystyle
%		\text{\raise1ex\hbox{$#1$}\Big/\lower1ex\hbox{$#2$}}%
%	}
%	{% \textstyle
%		#1\,/\,#2
%	}
%	{% \scriptstyle
%		#1\,/\,#2
%	}
%	{% \scriptscriptstyle  
%		#1\,/\,#2
%	}
%}
%
%
%
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%\newcommand\alert[1]{\marginpar{\warn{\scriptsize{#1}}}}
%%%GRAPH CATEGORIES
%\newcommand\Gr{\mathsf{etGr}}
%\newcommand\el{\mathsf{elGr}}
%\newcommand{\Grbig}{\mathsf{Graph}}
%\newcommand{\Gret}{\mathsf{etGraph}}
%\newcommand{\Griso}{\mathsf{Gr_{iso}}}
%
%%%% GRAPH NOTATION
%%$$$GRAPH NOTATION
%\newcommand\G{\mathcal{G}}
%\renewcommand\H{\mathcal{H}}
%\newcommand\W{\mathcal W}
%\newcommand\I{\mathcal{I}}
%%%%line and wheel graphs
%\newcommand{\Lk}[1][k]{\ensuremath{\mathcal L^{#1}}}
%\newcommand{\Wl}[1][m]{\ensuremath{\mathcal W^{#1}}}
%\newcommand{\Wm}[1][m]{\ensuremath{\mathcal W^{#1}}}
%
%
%\newcommand{\EI}{\ensuremath{{E_\bullet}}}
%
%
%%%%%Gradings
%\newcommand{\vH}[1][v]{\sfrac{H}{#1}}
%\newcommand{\vE}[1][v]{\sfrac{E}{#1}}
%\newcommand{\nV}[1][n]{V_{#1}}
%\newcommand{\nH}[1][n]{H_{#1}}
%\newcommand{\nE}[1][n]{E_{#1}}
%
%%1. Graph with index
%\newcommand{\Gn}[1]{\ensuremath{\mathcal G^{#1}}}
%\newcommand{\En}[1]{\ensuremath{E^{#1}}}
%\newcommand{\Hn}[1]{\ensuremath{H^{#1}}}
%\newcommand{\Vn}[1]{\ensuremath{V^{#1}}}
%\newcommand{\sn}[1]{\ensuremath{s^{#1}}}
%\newcommand{\tn}[1]{\ensuremath{t^{#1}}}
%\newcommand{\taun}[1]{\ensuremath{\tau^{#1}}}
%
%%1. Component of a graph
%\newcommand{\Gc}[1][c]{\ensuremath{\mathcal G^{#1}}}
%\newcommand{\Ec}[1][c]{\ensuremath{E^{#1}}}
%\newcommand{\Hc}[1][c]{\ensuremath{H^{#1}}}
%\newcommand{\Vc}[1]{\ensuremath{V^{#1}}}
%%\newcommand{\sn}[1]{\ensuremath{s^{#1}}}
%%\newcommand{\tn}[1]{\ensuremath{t^{#1}}}
%%\newcommand{\taun}[1]{\ensuremath{\tau^{#1}}}
%
%% 2. Graph associated to set $W \subset V$
%\newcommand{\GWbot}[1][W]{\ensuremath{\mathcal G^{\bot(#1)}}}
%\newcommand{\GW}[1][W]{\ensuremath{\mathcal G^{(#1)}}}
%\newcommand{\XW}[1][W]{\ensuremath{X^{(#1)}}}
%\newcommand{\XWbot}[1][W]{\ensuremath{X^{\bot(#1)}}}
%\newcommand{\EW}[1][W]{\ensuremath{E^{(#1)}}}
%\newcommand{\EWbot}[1][W]{\ensuremath{E^{\bot(#1)}}}
%\newcommand{\HW}[1][W]{\ensuremath{H^{(#1)}}}
%\newcommand{\HWbot}[1][W]{\ensuremath{H^{\bot(#1)}}}
%\newcommand{\VWbot}[1][W]{\ensuremath{V^{\bot(#1)}}}
%\newcommand{\VW}[1][W]{\ensuremath{V^{(#1)}}} % = W
%\newcommand{\sW}[1][W]{\ensuremath{s^{(#1)}}}
%\newcommand{\tW}[1][W]{\ensuremath{t^{(#1)}}}
%\newcommand{\tauW}[1][W]{\ensuremath{\tau^{(#1)}}}
%
%% 3. Corolla associated to a set
%
%\newcommand\CX[1][X]{{\mathcal C_{#1}}}
%%\newcommand{\Gn}[1]{\ensuremath{\mathcal G^{#1}}}
%\newcommand{\EX}[1][X]{\ensuremath{E^{#1}}}
%\newcommand{\HX}[1][X]{\ensuremath{H^{#1}}}
%\newcommand{\VX}[1][X]{\ensuremath{V^{#1}}}
%\newcommand{\sX}[1][X]{\ensuremath{s_{#1}}}
%%\newcommand{\tX}[1]{\ensuremath{t^{#1}}}
%\newcommand{\tauX}[1][X]{\ensuremath{\tau_{#1}}}
%
%% 4. Corolla associated to a vertex
%\newcommand\Cv[1][v]{{\mathcal C_{\mathbf{#1}}}}
%%\newcommand{\Gn}[1]{\ensuremath{\mathcal G^{#1}}}
%%\newcommand{\En}[1]{\ensuremath{E^{#1}}}%\newcommand{\Hn}[1]{\ensuremath{H^{#1}}}
%%\newcommand{\Vn}[1]{\ensuremath{V^{#1}}}
%\newcommand{\sv}[1][v]{\ensuremath{s_{(#1)}}}
%%\newcommand{\tX}[1]{\ensuremath{t^{#1}}}
%\newcommand{\tauv}[1][v]{\ensuremath{\tau_{(#1)}}}
%
%% 5. stick associated to an edge orbit
%\newcommand\shorte[1][\tilde e]{{\shortmid_{#1}}}
%\newcommand{\taue}[1][\tilde e]{\ensuremath{\tau_{(#1)}}}
%
%
%%5. maps associated to a graph
%%\newcommand{\Gn}[1]{\ensuremath{\mathcal G^{#1}}}
%\newcommand{\EG}[1][\shortmid]{\ensuremath{E^{(#1)}}}
%%\newcommand{\Hn}[1]{\ensuremath{H^{#1}}}
%%\newcommand{\Vn}[1]{\ensuremath{V^{#1}}}
%\newcommand{\sG}[1]{\ensuremath{s^{(#1)}}}
%\newcommand{\tG}[1]{\ensuremath{t^{#1}}}
%\newcommand{\tauG}[1][\shortmid]{\ensuremath{\tau_{#1}}}
%\newcommand{\qG}[1]{\ensuremath{q^{(#1)}}}
%
%%%%%CATEGORIES OF GRAPHS
%%%category associated to a graph
%\newcommand\cat[1][\G]{\ensuremath{\ldbrack #1\rdbrack}}
%
%
%%%%%Defining connectedness and establishing universal properties
%\newcommand{\diag}{\mathsf{\mathtt D}}
%\newcommand{\GrShape}{\mathsf{ps_f}(\mathtt D)}
%
%%%%graph morphisms and components of natural transformations $in_x^{\CX}$.
%\newcommand{\xin}[2][x]{\ensuremath{ch_{#1}^{#2}}} % e.g. ip_x^\G$
%\newcommand{\xout}[2][x]{\ensuremath{ch_{#1}^{#2}}\circ \taue}
%
%%Monads and free and forgetful functors
%\newcommand{\OOO}{\mathbb {O}}
%\newcommand{\MM}{\mathbb {M}}
%\newcommand{\MMop}{\mathbb {M}^{Op}}
%\newcommand{\Mop}{ {M}^{Op}}
%\newcommand{\Fop}{ {F}^{Op}}
%\newcommand{\Uop}{ {U}^{Op}}
%\newcommand{\MMcat}{\mathbb {M}^{Cat}}
%\newcommand{\Mcat}{ {M}^{Cat}}
%\newcommand{\Fcat}{ {F}^{Cat}}
%\newcommand{\Ucat}{ {U}^{Cat}}
%
%%categories
%%%slice
%\newcommand{\ov }{/}
%
%%%%%% SECTION 2 ESSENTIAL
%% essential category of $\G$. Contained in $\el$
%\newcommand{\esG}[1][\mathcal{G}]{\ensuremath{\mathsf{es}{(#1)}}}
%\newcommand{\esx}[1][x]{\ensuremath{\iota_{#1}}}
%\newcommand{\esv}[1][v]{\ensuremath{\iota_{{#1}}}}
%\newcommand{\ese}[1][e]{\ensuremath{\iota_{\tilde{#1}}}}%{\ensuremath{\mathbf{\tilde{#1}}}}
%\newcommand{\esh}[1][h]{\ensuremath{\delta_{{#1}}}} %WARN: Is $\kappa$ a good choice?
% \newcommand{\esH}[1]{\ensuremath{\delta_{#1}}}
%\newcommand{\iG}[2][]{\ensuremath{i_{#1}^{#2}}}
%
%%%%%% CATEGORIES OF ELEMENTS
%% category of elements of $\G$
%\newcommand{\elG}[1][\mathcal{G}]{\ensuremath{\mathsf{el}{(#1)}}}
%% canonical functor $\cat[\G] \to \el$
%\newcommand{\esdownG}[1][\mathcal{G}]{\ensuremath{{es}^(\downarrow){(#1)}}}
%
%%%%% FUNCTORS DEFINING EQUIVALENCES.
%\newcommand{\yet}{Y}
%% $\elG \to \esG$
%\newcommand{\res}[2][\mathcal{G}]{\ensuremath{\lfloor #2\rfloor}^{#1}}
%\newcommand{\fres}[1][\mathcal{G}]{\ensuremath{r^{f\ es}_{#1}}}
%%%POINTED
%\newcommand{\resp}[2][\mathcal{G}]{\ensuremath{\lfloor #2\rfloor}^{#1}_*}
%
%%%%%%%SECTION 3 GLUING%%%%%%%%%%
%%1. $\G$-indexed graph of graphs
%\newcommand\Gg{\mathbf \Gamma}
%\newcommand\Gdg{\mathbf \Lambda}
%%%colimit of $\Gg$
%\newcommand\coGg[1][\G]{{\Gg}({#1})}%{\overline{\Gg}}
%\newcommand\coGgvar[2][\G]{\overline{\Gg^{#2}}} %% \Gg^1(\G)
%\newcommand\GSg[1][S]{\mathbf \Gamma_{#1}}
%%\newcommand\coGSg[1][\G]{{#1}^{\Gg}}
%
%%%%%%%%
%%core inclusion
%\newcommand{\corei}[1][\G]{\ensuremath{ i^\bullet_{#1}}}
%
%
%
%%%%%%%%%%%%SECTION 4 SPECIES
%\newcommand{\CGS}[1][(C,\omega)]{{\GS^{#1}}}
%
%\newcommand{\Comm}{{Z}}
%\newcommand{\CComm}[2][(C,\omega)]{{{\Comm}^{#1}_{#2}}}
%
%%%%%%%%%%%%
%%GRAPHS OF GRAPHS
%%%%%%%%%%%%
%
%
%%%S-graph of graphs $\Gg_S$ NOTHING MORE COMPLICATED\
%%%%%colimits of S-graph of graphs
%\newcommand{\coGgS}[1][\G]{\overline{\Gg_S}}
%\newcommand{\coGgSvar}[2][\G]{\overline{\Gg_{#2}}}
%
%
%\newcommand{\comC}{\mathsf{CCC}}
%%%%%%%
%\newcommand{\CMO}[1][(C,\omega)]{{\MO^{#1}}}
%\newcommand{\CCSM}[1][(C,\omega)]{{^{#1}MO}}
%\newcommand{\CCat}{ \mathsf{C}}
%\newcommand{\DCat}[1][D]{ \mathsf{#1}}
%\newcommand{\Op}{ \mathsf{Op}}
%\newcommand{\boffcat}[1][\MM]{ \Theta_{#1}}
%
%%\newcommand{\CGSp}[1][C^\omega][1][C^\omega]{(#1)\GS_*}
%
%%%%2.3
%\newcommand{\CEl}[1][(C,\omega)]{{^{#1}El}}
%
%%listed \underline c C,\omega graphs
%
%
%
%
%
%%%%%%
%%degnerate $\W$-shaped graph of $S$-graphs $\mathbf O_S^c$
%\newcommand{\TJK}{T^{{(\shortmid)}}}
%\newcommand{\muJK}{\mu^{(\shortmid)}}
%\newcommand{\etaJK}{\eta^{(\shortmid)}}
%\newcommand{\XGrJK}[1][X]{{#1}\Griso^{(\shortmid)}}
%
%%%%SECTION 2%%%%%%%%%%%
%\newcommand{\CGSp}[1][(C,\omega)]{{\GSp^{#1}}}
%%\newcommand{\CCommp}[1][C^\omega]{(#1)Comm}
%
%
%%%%%Section 3
%\newcommand{\uG}[2][]{\ensuremath{ch_{#2} \circ u}}
%\newcommand{\zG}[2][]{\ensuremath{ch_{#2} \circ z}}
%\newcommand{\kappaG}[2][]{\ensuremath{ch_{#2} \circ \kappa}}
%%%vertexdeletion stuff
%
%%%%pointed graph of graphs 
%%\newcommand{\Ggp}{\Gg_*}
%%\newcommand{\coGgp}[1][\G]{\Ggp(\G)}
%
%%%%vertex deletion
%%6. deleting a vertex
%\newcommand{\Gnov}[1][W]{\ensuremath{\mathcal G_{/#1}}}
%\newcommand{\Enov}[1][W]{\ensuremath{E_{/#1}}}
%\newcommand{\Hnov}[1][W]{\ensuremath{H_{/#1}}}
%\newcommand{\Vnov}[1][W]{\ensuremath{V_{/#1}}}
%\newcommand{\snov}[1][W]{\ensuremath{s_{/#1}}}
%\newcommand{\tnov}[1][W]{\ensuremath{t_{/#1}}}
%\newcommand{\taunov}[1][W]{\ensuremath{\tau_{/#1}}}
%\newcommand{\delW}[1][W]{\mathsf{del}_{/#1}}
%
%
%
%%%%%1. $\G$-indexed graph of pointed graphs
%\newcommand\Gpg[1][]{{\Gg_*^{#1}}} % e.g. \Gpg[1], etc
%%\newcommand\coGpg[1][\G]{\Gg_*(\G)}
%%\newcommand\coGpgvar[2][\G]{\Gg_{*#2}(#1)} %% \Gg^1(\G)
%%\newcommand{\GpgS}[
%%\newcommand{\coGpgS}[1][\G]{\Gg_{*S}(#1)}
%%\newcommand{\coGpgSvar}[2][S]{\Gg_{*#1}^{#2}}
%
%
%
%%%%% Special constructions
%
%\newcommand{\elup}{\el^{\uparrow}}
%
%\newcommand{\DiGSD}[1][D]{\DiGS^{#1}}
%\newcommand{\Tdloop}{T^\circlearrowleft}
%\newcommand{\mudloop}{\mu^\circlearrowleft}
%\newcommand{\etadloop}{\eta^\circlearrowleft}
%
%%\newcommand\Ggv[2][\G]{\mathbf {G}_{#1, #2}}
%
%%\newcommand\iGg[2][{\Gg{\G}}]{u_{#1}^{#2}}
%%%%Category of non-deg $\G$-ind graphs of connected graphs
%\newcommand{\GrG}[1][\G]{\ensuremath{\Gr^{(#1)}}}
%
%%%%4. Graphs of structured graphs REWORK THIS...
%%\newcommand\GSgj[2][S]{\mathbf {G}^{#1}_{(#2)}}
%%%\newcommand\GSg[2][\G]{{\mathbf {G}_{#1}^{#2}}}
%%%%CHECK THROUGH FOR ALL CHANGES....
%%\newcommand\GSg[2][\G]{{\Xi^{#2}}}
%%%%Category of non-deg $\G$-ind graphs of connected graphs
%\newcommand{\GrSG}[1][\G]{\ensuremath{\Gr^{(#1)}(S)}}
%\newcommand{\GrSGvar}[2][\G]{\ensuremath{\Gr^{(#1)}(#2)}}
%
%%%%%%GROTHENDIECK TOPOLGIES
%\newcommand{\sieve}[1][\elG]{\ensuremath{\langle #1 \rangle}}
%
%%%%%Symmetric collections
%\newcommand{\Coll}[1][(C, \omega)]{\mathsf{Coll}^{#1}}
%\newcommand{\DiColl}[1][D]{\mathsf{DiColl}^{#1}}
%\newcommand{\DProp}[1][D]{\mathsf{Prop}_\circlearrowleft^{ #1}}
%%%%%%Totally labelled graphs
%%\newcommand{\Tl}{\mathsf{Tl}\Gr_{iso}}
%%\newcommand{\voTl}[1][k]{\mathsf{Tl}\Gr^{\mathbf{#1}vo}_{iso}}
%%\newcommand{\Td}{\mathsf{Di}\Gr^D_{iso}}
%% \newcommand{\DiGr}[1][(\ccc;\ddd)]{{#1}\mathsf{DiGr}_{iso}^D}
%%  \newcommand{\DiGrloop}[1][( ;\ddd)]{{#1}\mathsf{DiGr}_{iso}^{\circlearrowleft D}}
%%  \newcommand{\Wloop}[1][D]{ W^{\circlearrowleft{#1}}}
%%    \newcommand{\muloop}[1][D]{ \mu^{\circlearrowleft{#1}}}
%%        \newcommand{\etaloop}[1][D]{ \eta^{\circlearrowleft{#1}}}
%%            \newcommand{\hloop}{ h^{\circlearrowleft}}
%% \newcommand{\DiGrvar}[2]{{#1}\mathsf{DiGr}_{iso}^{#2}}
%% \newcommand{\DiGS}{\mathsf{DiGS}}
% 
%%%%%%%%%strictly undirected things%%%%%%
%% \newcommand{\Tud}{T_{ud}}
%% \newcommand{\muud}{\mu_{ud}}
%% \newcommand{\etaud}{\eta_{ud}}
%% \newcommand{\hud}{h_{ud}}
%%%%%%%%%%%%%%%%%%%
%%%%POINTED GRAPHS
%%%%%%%%%%%%%%%%%%%
%\newcommand{\elp}{\ensuremath{\mathsf{elGr}_*}}
%\newcommand{\Grp}{\ensuremath{\mathsf{\Gr}_*}}
%\newcommand{\GSp}{\ensuremath{\mathsf{\GS}_*}}
%\newcommand{\Gretp}{\ensuremath{\Gret_{*}}}
%\newcommand{\fisinvp}{\ensuremath{\fisinv_*}}
%
%%\newcommand\Gr{\mathsf{etGr}}
%%\newcommand\el{\mathsf{elGr}}
%%\newcommand{\Grbig}{\mathsf{Graph}}
%%\newcommand{\Gret}{\mathsf{etGraph}}
%
%
%% category of pointed elements of $\G$
%\newcommand{\elpG}[1][\mathcal{G}]{\ensuremath{\mathsf{el}_*{(#1)}}}
%% essential pointed category of $\G$. Contained in $\elp$
%\newcommand{\espG}[1][\mathcal{G}]{\ensuremath{\mathsf{es}_*{(#1)}}}
%% Category of essential pointed elements of $\G$. canonically iso to $\espG$
%\newcommand{\esdownpG}[1][\mathcal{G}]{\ensuremath{\mathsf{es}_*^(\downarrow){(#1)}}}
%
%\newcommand{\sievep}[1][\elpG]{\ensuremath{\langle #1 \rangle}}
%\newcommand{\sieveG}[1][\G]{\mathcal {El}(#1)}
%
%\newcommand{\mup}{\ensuremath{\mu_*}}
%\newcommand{\etap}{\ensuremath{\eta_*}}
%\newcommand{\Tp}{\ensuremath{T_*}}
%\newcommand{\Tpo}{\ensuremath{T_{p.o.}}}
%
%\newcommand{\EsdownpG}[1][\mathcal{G}]{\ensuremath{Es^(\downarrow)_{#1*}}}
%
%
%%Category of locally linear/minimal graphs
%\newcommand{\Grll}{\ensuremath{\Gr_*^{0,2}}}
%%1. pointed $\G$-indexed graph of graphs
%%\newcommand{\Gpg}[1][\mathcal G]{\mathbf {G}_{#1*}}
%
%
%%%%%%%%%%%%%
%%%natural transformation $C9-,c) \Rightarrow F$ associated with an element $x \in F(c)$ #1 is x
%\newcommand{\nt}[1][\alpha]{(#1)^{(\downarrow)}}
%
%
%\newcommand{\In}{{\mathrm{ in }}}
%\newcommand{\Out}{{\mathrm{ out }}}
%%%%%%%%%%%%
%%POINTED GRAPHS OF GRAPHS
%%%%%%%%%%%%
%%%1. $\G$-indexed graph of graphs
%%\newcommand\Gpg[1][\mathcal G]{\mathbf {G}_{#1*}}
%%%2. $\esG$ component of a $\G$-indexed graph of graphs
%%\newcommand\Gpgv[2][\overline{\Gg{\G}}]{(\overline{#1})_{#2}}
%%%3.canonical map from $\esG$ component  to colimit
%%%notice that this is closely related to $\iG$. Why is this justified?
%%\newcommand\iGpg[2][\overline{\Gg{\G}}]{i_{#1}^{#2}}
%%%%%category of $\G$-indexed non-deg pointed graphs of graphs
%\newcommand{\GrpG}[1][\G]{\ensuremath{\Grp^{(#1)}}}
%
%%%4. Graphs of structured graphs 
%%\newcommand\GSpgj[2][S]{\mathbf {G}^{#1}_{(#2)}}
%
%%2. $\esG$ component of a $\G$-indexed graph of graphs
%%\newcommand\Ggv[2][\overline{\Gg{\G}}]{(\overline{#1})_{#2}}
%%3.canonical map from $\esG$ component  to colimit
%%notice that this is closely related to $\iG$. Why is this justified?
%%\newcommand\iGg[2][\overline{\Gg{\G}}]{i_{#1}^{#2}}
%
%%%%Category of non-deg $\G$-ind pointed graphs of connected graphs
%\newcommand{\GrpSG}[1][\G]{\ensuremath{\Grp^{(#1)}(S)}}
%\newcommand{\GrpSGvar}[2][\G]{\ensuremath{\Gr^{(#1)}(#2)}}












==> 0401Definitions.tex <==

%\subsection{Graphical species}
\section{Definitions and examples}

\label{sec: definitions}


The goal of this section is to give an axiomatic definition of modular operads (\cref{defn: Modular operad}), and to provide some motivating examples. As mentioned in the introduction, the term `modular operad' refers here to what are called `compact symmetric multicategories (CSMs)' in \cite{JK11}. 

After establishing some basic notional conventions, the section begins with a discussion of Joyal and Kock's category $\GS$ of graphical species \cite{JK11} which generalises various notions of coloured collection used in the study of operads. 

\subsection{Graphical species}
\label{ssec: graphical species}
%\subsection{General notation}
%\srnote{0403 - some rejigging, also in response to R16}


A \emph{presheaf} on a category $\CCat$ is a functor $ P\colon \CCat^\mathrm{op} \to \Set$. The corresponding functor category %or \emph{presheaf category} 
is denoted $\pr{\CCat}$. 

The notion of elements of a presheaf will be used extensively in what follows:%A presheaf $P$ on $\CCat$ describes a category $\mathsf{el}_{\CCat}(P)$:

\begin{defn}%\srnote{R16}
	\label{defn: general element} An \textit{element} of a presheaf $P \colon \CCat^{\mathrm{op}} \to \Set$ is a pair $(c, x)$ where $c$ is an object of $\CCat$ and $x \in P(c)$. The elements of $P$ are the objects of a category $\ElP{P}{\CCat}$ whose morphisms $(c,x) \to (d,y)$ are given by morphisms $f \in \CCat (c,d)$ such that $P(f)(y) = x$. 

\end{defn}
%
%
%
%
%
%Let $F\colon \DCat \to \CCat$ and $G\colon \DCat[E] \to \CCat$ be functors. Objects of the \textit{comma category} $F \ov G$ (or $F_{\DCat}\ov G_{\DCat[E]}$) are triples $ ( d, \gamma, e)$ with $d \in \DCat, e \in \DCat[E]$ and $\gamma \in \CCat(F(d), G(e))$. Morphisms in $F\ov G((d, \gamma, e), (d',\gamma',e'))$ are pairs of morphisms $f \in \DCat (d,d')$ and $g \in \DCat[E](e,e')$ such that 
%\[ \xymatrix{ F(d) \ar[rr]^-{F(f)} \ar[d]_{\gamma}&& F(d') \ar[d]^{\gamma'}\\
%G(e) \ar[rr]_-{G(g)} && G(e')}\] commutes in $\CCat$.
If a presheaf $P $ on $\CCat$ is of the form $ \CCat(-, c)$, then $\ElP{P}{\CCat}$ is the \textit{slice category} $\CCat\ov c$ whose objects are pairs $(d,f)$ where $f \in \CCat (d,c)$, and morphisms $(d,f) \to (d', f')$ are given by %$g \in \CCat (d, d')$ such that $f = f' \circ g$. 
 by commuting triangles in $\CCat$:
\[ \xymatrix{ d \ar[rr]^-g \ar[dr]_{f} && d' \ar[dl]^-{f'}\\&c.&}\] 

Given a functor $\iota\colon\DCat \rightarrow \CCat$, and an object $c$ of $\CCat$, the pullback $\iota^* \CCat(-,c)$, $d \mapsto \CCat(\iota (d),c)$ defines a presheaf on $\DCat$, and $ \iota \ov c \defeq\ElP{\iota^*\CCat(-, c) }{\DCat}$ is called the \emph{slice category of $\iota$ {over} $c$}. % is defined as $ \iota \ov c \defeq\ElP{\CCat(-, c) \circ \iota}{\DCat}$. So, its %morphisms 
% in $\CCat$, has 
%Its objects are pairs $(d,f)$ with $d \in \DCat$ and $f \in \CCat(\iota (d),c)$, and its morphisms 
%$(d, f) \to (d', f')$ are given by those $g \in \DCat (d, d')$ such that $ \iota (g)$ describes a morphism in $ \CCat \ov c$. If $\iota$ is an inclusion of subcategories $\DCat \hookrightarrow \CCat$, then we write $\DCat \ov c \defeq \iota \ov c$.  
%The categories $ c \ov \iota $ and $c \ov \DCat$ are defined similarly. %\srnote{2603 - do I use?}

%For $n \in \N$, the set $ \{1,\dots, n\}$ is denoted by $\nn$, so $\nul $ denotes the empty set $\emptyset$.  
%Let $\Sigma$ denote 
 The groupoid of finite sets and bijections is denoted by $\fiso$.  For $n \in \N$, the set $ \{1,\dots, n\}$ is denoted by $\nn$. So $\nul  = \emptyset$ is the empty set.% $\emptyset$.  

%I denote the category of finite sets by $\fin$.



\begin{rmk}
	
%The permutation groupoid $\Sigma$ -- with objects $n \in \N$ and morphisms 
%$\Sigma (m, n) =  Aut(\nn) $ if $ m = n$, and $ \Sigma(m,n) = \emptyset$  if $m \neq n$ -- is skeletal in $\fiso$. 
Let $\Sigma\subset \fiso$ denote the skeletal subgroupoid on the objects $\nn$, for $n \in \N$. A presheaf $P\colon \fiso^\mathrm{op} \to \Set$ on $\fiso$, also called a \emph{(monochrome} or \emph{single-sorted) species} \cite{Joy81},  determines a presheaf on $\Sigma$ by restriction. %, or \emph{symmetric sequence}, 
	 Conversely, a $\Sigma$-presheaf $Q$ may always be extended to a $\fiso$-presheaf $Q_{\fiso}$, by setting
	\[ Q_{\fiso}(X) \defeq \mathrm{lim}_{(\nn,f) \in \Sigma \ov X}  Q(\nn) \  \text{ for all } n \in \N.\]% if $\nn \defeq \{ 1,\dots, n\}.$
%%\srnote{got rid of convenience remark...}	
%For convenience, we work with presheaves over (categories containing) $\fiso$ instead of $\Sigma$.
 %\warn{However, in some contexts, $\Sigma$ will be used, particularly for examples where the reader is likely to be more familiar with a grading by $\N$.}
%	\warn{21.5do briefly consider what actually happens in the paper..}}
 \end{rmk}

%\begin{ex}%\srnote{R.11 -example added?}
%	An uncoloured symmetric operad in $\Set$ is described, up to equivalence, by a species $O \colon \fiso^{\mathrm{op}}\to \Set$, together with the data of a unital operadic composition. 
%	
%	However, more is required to specify
%
%\end{ex}
 

%\subsection{Graphical species}

%\warn{REV. 11. Question - what type of intuition here?  Operad example above? Usual problems ASK RICHARD} %\srnote{R11. recall previous versions...}
Graphical species, defined in \cite[Section~4]{JK11}, are a \textit{coloured} or \textit{multi-sorted} version of species. 

Let the category $\fisinv$ be obtained from $\fiso $ by adjoining a distinguished object $\S$ that satisfies %according to% such that 
%%\srnote{change ok? should I reorder and include equivariance...?
%Also, single and multi-shorted}
\begin{itemize}
	\item $\fisinv (\S, \S) = \{ id, \tau \} $ with $\tau^2 = id$,
	%	\item for all finite sets $X$ and $Y$, $\fisinv(X,Y) = \fiso  (X,Y)$,
	\item for each finite set $X$ and each element $x \in X$, there is a morphism $ch_x \in \fisinv (\S, X)$ that `chooses' $x$, and $\fisinv(\S, X)=  \{ch_x\ ,\ ch_x \circ \tau \}_{x \in X}$, % \amalg \{ch_x \circ \tau \}_{x \in X}
	\item for all finite sets $X$ and $Y$, $\fisinv(X,Y) = \fiso  (X,Y)$, and morphisms are equivariant with respect to the action of $\fiso$: $ ch_{f(x)} = f \circ ch_x  \in \fisinv (\S, Y)$ for all $ x \in X$ and all bijections $f\colon X \xrightarrow {\cong} Y$.
\end{itemize}
% \[
%\begin{array}{lll} \fisinv (\S, \S) &=& \{ id, \tau \} \ \text{ with } \tau^2 = id,\\ 
%\fisinv(\S, X)&=&  \{ch_x\}_{x \in X}  \amalg \{ch_x \circ \tau \}_{x \in X}  \\
%\fisinv(X,Y)& = &\fiso  (X,Y), \ \text{ where } X \text{ and } Y \text{ are finite sets.}\end{array}\] 


\begin{defn}\label{defn: graphical species}
 A \emph{graphical species} is a presheaf $S\colon {\fisinv}^\mathrm{op} \to \Set$. The category of graphical species is denoted $\GS\defeq\pr{\fisinv}$.
 
\end{defn}





% An \emph{involutive set} is a set $\CCC$ equipped with an involution $\omega\colon \CCC \to \CCC$, $\omega^2 = id$. Given an involutive set $(\CCC, \omega)$, the set of $\omega$-orbits in $\CCC$ is denoted by $\widetilde \CCC$, and $\tilde c \in \widetilde \CCC$ is the orbit of $c \in \CCC$.

%\srnote{consistency in using $S_\tau$...}
Hence, a graphical species $S$ is described by a species $(S_X)_{X \in \fiso}$, and a set $S_\S$ with involution $S_\tau \colon S_\S \to S_\S$, % an involutive set $(\CCC, \omega)  = (S_\S, S_\tau)$ called the \emph{palette} of $S$, % and involution $\omega = {S_{\tau}}\colon \CCC \to \CCC$, 
together with, for each finite set $X$, and $x \in X$ a $\fiso$-equivariant {projection} $S(ch_x)\colon S_X \to S_\S$. 


\begin{defn}\label{c arity}%\srnote{1503 - R11 amalgamated definitions}
	Given a graphical species $S$, the pair $(S_\S, S_\tau)$ is called the \emph{(involutive) palette} of $S$ and elements $c \in S_\S$ are \textit{colours of $S$}.  If $S_\S$ is trivial then $S$ is a \emph{monochrome graphical species}.
%\end{defn}
%
%\begin{defn}

	For each element $ \underline c = (c_x)_{x \in X} \in {S_\S}^{X}$, the \emph{$\underline c$-(coloured) arity $ {S_{\underline c}}$} is the fibre above $ \underline c \in {S_\S}^{X}$ of the map $(S(ch_x))_{x \in X}\colon  {S_X} \to{S_\S}^{X}$.
	
	
	%	\warn{check notation for this map}
	
\end{defn}

%\warn{R11. tie in with intuition}


% In this case $S$ is called a \emph{$(\CCC, \omega)$-coloured graphical species} and elements $c \in \CCC$ are \textit{colours of $S$}. If $(\CCC, \omega)\cong \{*\}$ is trivial then $S$ is a \emph{monochrome graphical species}.

	%\footnote{In this work, the singular term `palette' replaces the more standard multi-word `colour set'. } 
%\end{defn}


\begin{rmk}%\srnote{R 13}
The involution $\tau$ on $\S$ is responsible for much of the heavy lifting in the constructions that follow. Initially however, its role may seem obscure. I mention two key features here. First, the involution provides the expressive power necessary to describe composition rules involving colours, such as particle spin, that may have an orientation, or direction. %encode structure such as (topological) type of boundary components, or particle spin, that may, or may not have an orientation. % thereby bolstering the expressive power of graphical species. 
(Directed graphical species are discussed in \cref{ex:direction}.)

The second is more fundamental. The involution enables us to encode formal compositions in graphical species -- described in terms of graphs -- as categorical limits, and thereby derive the results of this paper % our results %, and the Segal condition for \cref{thm: nerve intro} (\cref{nerve theorem}), in particular, using 
by purely abstract methods. For example, the involution underlies a well-defined notion of graph nesting, or substitution, in terms of diagram colimits, without the need to specify extra data (see Sections \ref{sec: non-unital} and \ref{degenerate}, and compare with, e.g.\ \cite{JY15,HRY15}).

\end{rmk}



\begin{ex}\label{Comm}
	The terminal graphical species $\Comm$ has trivial palette and $ \Comm_X = \{*\}$ for all finite sets $X$.
\end{ex}



\begin{defn}\label{def: palette preserving]}

	A morphism $ \gamma \in \GS(S, S' )$ is \emph{palette-preserving} if its component $\gamma_\S$ at $\S$ is the identity on ${S_\S}$. For a fixed palette $(\CCC, \omega)$, $\CGS$ is the subcategory of $\GS$ on the $(\CCC, \omega)$-coloured graphical species and palette-preserving morphisms.% is denoted $\CGS$.
	
	\end{defn}




%\srnote{2803 - sentence deleted. Obvious}
%If $ \gamma \in \GS(S, S' )$ is a palette-preserving morphism of $(\CCC, \omega)$-coloured graphical species, 
%$\gamma_X ( {S_{\underline c}}) \subset  {S' _{\underline c}} $ for all finite sets $X$ and all $ \underline c \in \CCC^X$.
%\srnote{0203 - slight notation change.}

%\srnote{0203 - slight order change}
\begin{ex}\label{Comm c}
	For any palette $(\CCC, \omega)$, the terminal $(\CCC, \omega)$-coloured graphical species $\CComm{}$ in $\CGS$ is described by
	\[ \CComm{X}= \CCC^X, \text{ with } \CComm{\underline c} = \{*\}, \text { for all finite sets } X \text{ and all } \underline c \in \CCC^X.\]	
	
	
	In particular, let $\Disig$ be the unique non-identity involution on the set $\Di \defeq \{\In, \Out\}$. A \textit{monochrome directed graphical species} is a graphical species with palette $\Dipal$. The terminal monochrome directed graphical species is denoted by $Di \defeq\CComm[\Dipal]{}$. See also \cref{ex:direction}. % be the terminal $\Dipal$-coloured graphical species. 
\end{ex}

\begin{rmk} \label{rmk: visualise} %(This remark is made precise in \cref{subs. sheaves}.) 
	As will be explained in \cref{ex: embedding fin}, $\fisinv$ embeds in a certain category of graphs. Under this embedding, the distinguished object $\S$ and the involution $\tau$ on $\S$, are represented, as in \cref{fig. lim and colim}, as the exceptional edge with no vertices and two endpoints, and the map that flips the edge. 
	  %labelled by $1$ and $2$. The involution $\tau$ on $\S$ is the map is represented by the map $1 \leftrightarrow 2$, that flips the edge.  
	A finite set $X$ is represented by a \textit{corolla} or \textit{star graph} $\CX$ with legs in bijection with $X$ (\cref{fig. species vis} left side). For each $x \in X$, the map $ch_x \colon \S \to X$ corresponds to the inclusion $1 \mapsto x $, of the exceptional edge as an edge of the corolla.
	
	If $S$ is a graphical species, an element $ \phi \in S_X$ is represented graphically as a labelling or \textit{decoration} of the unique vertex of $\CX$, and a \textit{colouring} of the legs of $\CX$ by $S_\S$ according to $S(ch_x)$ for $x \in X$. %
%	
%	%\srnote{Refers to R18. 24.2 This is tricky...}
%	
%Given a graphical species $S$ and $ \underline c = (c_x)_{x \in X}, \ c_x \in S_\S$, % is a $(\CCC, \omega)$-coloured graphical species, 
%an element $\phi \in S_{\underline c} $ % for some $ \underline c = (c_x)_{x \in X} \in \CCC^X$ for some finite set $X$. An element $\phi \in S_{\underline c} \subset S_X$ 
%may be visualised, as in the right hand side of \cref{fig. species vis}, as a corolla with vertex \textit{decorated by $\phi$}  and legs bijectively \textit{coloured} by $(c_x)_{ x \in X}$. %A colour $c \in  S_\S$ may then be visualised as a line with ends labelled by $c$ and $S_\tau c$ 
(See, for example \cref{fig: directed elements}.)
	
	\begin{figure}[htb!]
	\[	\begin{tikzpicture}[scale = 0.55]
	\node at(0,0){\begin{tikzpicture}[scale = 0.55]
		\draw [thick] (-8.5,3.5) --(-6.5,3.5);
	%	\node at (-5.8, -0.5) {\tiny {$(x)$}};
	\node at (-8.3, 3.1) {\tiny{ $1$}};
	\node at (-6.7, 3.1) {\tiny{ $2$}};
	

	\node at (-7.5,1.7){$\S$};
	\node at (0,1.7){$X = \{x,y,z\}$};
	
	\draw[->] (-5.5,3.5)--( -3.5,3.5);
	\node at (-4.5,3.1){\scriptsize{$1 \mapsto x$}};
		\node at (-4.5,3.9){\scriptsize{$ch_x$}};
	\draw [  ultra thick] (0,3.5) -- (-2.25,3.5);
	\draw (0,3.5)--(1.8,4.5)
	(0,3.5) --(1.8,2.5);
\filldraw (0,3.5) circle (3pt);	
	\node at (-1, 3.2) {};
	\node at (0.3, 4.5) {};
	\node at (-2.2, 3) {\scriptsize {$x$}};
%	\node at (1.7, 4.05) {\tiny {$y$}};
%	\node at (1.7, 2.75) {\tiny{ $z$}};
	\node at (0.3,2.5) {}; 
	
		\draw [gray, decorate,decoration={brace,amplitude=5pt, raise=4pt},yshift=0pt]
	(-9,2) -- (-9,5) %node [black,midway,xshift=0.8cm] {\footnotesize
	%	$P_2$}
	;
	\draw [gray,decorate,decoration={brace,amplitude=5pt,mirror,raise=4pt},yshift=0pt]
(2.5,2) -- (2.5,5)% node [black,midway,xshift=0.8cm] {\footnotesize
%		$P_2$}
	;
	
	\end{tikzpicture}};
	
	\draw[gray, thick, ->] (7.5,0)--(9.5,0);
	\node at (8.5,.5) {$S$};
	\node at(17, 0){\begin{tikzpicture}[scale = 0.55]
	

	%\node at(0,-2) {\small{$\phi_2 $}};
%%%%%%%%%%%%%%%
	\draw [blue, thick] (-8.5,0) --(-6.5,0);
	%	\node at (-5.8, -0.5) {\tiny {$(x)$}};
	\node at (-8.3, 0.3) {\tiny{ $c_x$}};
	\node at (-6.7, 0.3) {\tiny{ $\omega c_x$}};
	
	
	\draw[<-] (-5.5,0)--( -3.5,0);
	\node at (-4.5,.4){\scriptsize{$S(ch_{x})$}};
	
	\draw [  blue, ultra thick] (0,0) -- (-2.25,0);
	\draw (0,0)--(1.8,1)
	(0,0) --(1.8,-1);
	
	\node at (-1, -0.3) {};
	\node at (0.3, 1) {};
	\node at (-2.2, -0.5) {\tiny {$(x)$}};
	\node at (-2.2, 0.3) {\tiny{ $c_{x}$}};
%		\node at (-.85, 0.3) {\tiny{ $\omega c_{x}$}};
		\node at (1.7, .55) {\tiny {$(y)$}};
	\node at (1.7, 1.2) {\tiny{ $c_{y}$}};
		\node at (1.7, -.6) {\tiny {$c_{z}$}};
	\node at (1.7, -1.25) {\tiny{ $(z)$}};
	\node at (0.3,-1) {};
	
	\draw  [ draw=red,   fill=white]
	(0,0) circle (15pt);
	
	\node at(0,0) {\small{$\phi $}};
	%\node at(0,-2) {\small{$\phi_2 $}};
		\draw [gray, decorate,decoration={brace,amplitude=5pt, raise=4pt},yshift=0pt]
	(-9,-1.5) -- (-9,1.5) %node [black,midway,xshift=0.8cm] {\footnotesize
	%	$P_2$}
	;
	\draw [gray, decorate,decoration={brace,amplitude=5pt,mirror,raise=4pt},yshift=0pt]
	(2.5,-1.5) -- (2.5,1.5)% node [black,midway,xshift=0.8cm] {\footnotesize
	%		$P_2$}
	;
		\node at (-7.5,-1.8){\small{${\color{blue}{c_x}} \in S_\S$}};
	\node at (-.6,-1.8){\small{$\phi \in S_{X}$}};
	\end{tikzpicture}
		};
		\end{tikzpicture}
	\]
	\caption{%Visualising $\S$ as a loose edge and finite sets as corollas. 
	Graphical species may be represented graphically: % by decorations of Morphisms in $\fisinv$ may be represented graphically (left), and 
		$\phi \in S_{X}$ is represented as a $X$-corolla $\CX$ with vertex decorated by $\phi$ and $x$-leg coloured by ${\color{blue}c_x =  S(ch_{x})}$.}\label{fig. species vis}
		\end{figure}
\end{rmk}







%\begin{rmk}
%	Let $P\colon \CCat^\mathrm{op} \to \Set$ be any presheaf and $ *\colon \CCat^\mathrm{op} \to \Set$ the terminal presheaf on $\CCat$. So, objects of the category $(* \ov P)^\mathrm{op}$ (often called the \textit{element category of $P$}) are determined by pairs $(c, \alpha)$ $c \in \CCat, \alpha \in P(c)$, and morphisms $(c, \alpha) \to (c', \alpha')$ are morphisms $f \in \CCat (c, c')$ such that $P(f)(\alpha') = \alpha$. 
%\end{rmk}

 %Let $ *\colon \CCat^\mathrm{op} \to \Set$ denote the terminal presheaf on a category $\CCat$. 
 %%\srnote{RG? This feels inefficient. How would he do it?}
 \srnote{3103}
For any graphical species $S$, the Yoneda embedding $\fisinv \hookrightarrow \GS$ induces a canonical isomorphism $\ElP{S}{\fisinv} \cong \fisinv \ov S$ between the the slice category $\fisinv \ov S$ and the category $\ElP{S}{\fisinv}$ of elements of $S$ (see \cref{defn: general element}). These categories will be identified in what follows, and called the \textit{category of elements of $S$}, denoted by $\fisinv \ov S$.

%\begin{defn}\label{elS} %For any category $\CCat$ and presheaf $P\colon \CCat^\mathrm{op} \to \Set$, the \emph{element category of $P$} is the given by $(* \ov P)^\mathrm{op}$, where $*$ denotes the terminal presheaf on $\CCat$.
%	
%The category $\ElS[S]$ of \emph{elements of a graphical species $S$} is defined as $\ElS[S] \defeq \ElP{S}{\fisinv}$.
%%(\cref{defn: general element}) .%$(\Comm \ov S)^\mathrm{op}$.
%%	\[\ElS[S] \defeq \int_{\fisinv} S.\] 
%\end{defn}
%So, objects of $\ElS[S]$ are pairs $(\C, \phi)$ where $\C$ is an object of $\fisinv$ and $\phi \in S(\C)$, and morphisms $(\C, \phi) \to (\C', \phi')$ are given by those morphisms $g \in \fisinv (\C, \C')$ such that $S(g)(\phi') = \phi$. 
%%\srnote{description deleted R.16}
%the category $(* \ov P)^\mathrm{op}$ (often called the \textit{element category of $P$}) are determined by pairs $(c, \alpha)$ $c \in \CCat, \alpha \in P(c)$, and morphisms $(c, \alpha) \to (c', \alpha')$ are morphisms $f \in \CCat (c, c')$ such that $P(f)(\alpha') = \alpha$. 

%\begin{rmk}
%	\label{rmk: elements of presheaf} 
% I only use the term `category of elements' specifically to refer to categories of the form $(\Comm_{\fisinv} \ov S_{\fisinv})^\mathrm{op}$. In \cref{subs. sheaves}, we see that graphical species may be extended to presheaves on a larger category $\Gr \supset \fisinv$ of graphs. To distinguish the two viewpoints, objects in $ (\Comm_{\Gr} \ov S_{\Gr})^\mathrm{op}$ will be called `$S$-structured graphs'.
%\end{rmk}
%%\srnote{R. 16,17}

%%\srnote{slight formatting change, deletion of last sentence. RG?}

\srnote{3103 - check brackets around element categories.}
For any graphical species $R$, there is a canonical isomorphism $\GS \ov R \cong \pr{\ElS[R]}$ given by:
\[ (S, \gamma\colon S \to R) \ \longleftrightarrow \ S^\gamma\colon \ElS[R]^\mathrm{op} \to \Set, \ % \quad S^\gamma\colon 
\left \{\begin{array}{ll} (\S, c) \mapsto \gamma_\S^{-1} (c), & c \in {R} _{\S}\\
(X, \phi) \mapsto \gamma_X^{-1}(\phi), & \phi \in R_X, \ X \in \fiso.
\end{array} \right. \]
%where, for each object $\C$ of $\fisinv$, $\gamma_{\C}$ denotes the component of $\gamma$ at $\C$ .

%%\srnote{0403 - could say something about operads for modular operads..} 

\begin{ex}\label{ex:direction}%\srnote{R18. better lay out with example} %The combinatorics of PROPs \cite{MacL65}  may be descri
	 	A \textit{PROP} \cite{MacL65} is a strict symmetric monoidal category $(\DCat[E], + , 0)$ whose objects are natural numbers and whose monoidal product $+$ is addition on objects. Equivalently, $\DCat[E]$ is described by a presheaf $P = P_{\DCat[E]} \colon \left(\fiso \times \fiso^{\mathrm{op}}\right)^{\mathrm{op}} \to \Set$ with $P(X;Y) = \DCat[E](|X|, |Y|)$, together with the distinguished element $id_1 \in P(\one;\one) = \DCat[E](1,1)$, and maps defining the composition and monoidal product. 
	 	
	 	More generally, for any set $\DDD$, a $\DDD$-\textit{coloured PROP} is a strict symmetric monoidal category whose monoid of objects is freely generated by $\DDD$. %(Coloured) PROPs admit a description in terms of graphical species.
	
Let $\fisinvdi$ be obtained from $\fiso\times \fiso^{\mathrm{op}} $ by adjoining a distinguished object $(\downarrow)$ with
	%\begin{itemize} \item
	trivial endomorphism group, % $\fisinvdi(\downarrow, \downarrow) = \{id_\downarrow\}$,
	%\item 
	and, for all pairs $(X, Y)$ of finite sets, and all elements $x \in X$ and $y \in Y$, \textit{input} morphisms $i_x\colon(\downarrow) \to (X,Y)$, and \textit{output} morphisms $o_y\colon(\downarrow) \to (X,Y)$ that are compatible with the action of $\fiso\times \fiso^{\mathrm{op}} $ (see \cref{fig: directed elements}(d)). 

Then, a $\DDD$-coloured PROP 
$(\DCat[E]^{\DDD}, \oplus , \emptyset)$ is equivalently a presheaf $P^{\DDD}$ on $\fisinvdi$ with $P^{\DDD}(\downarrow) = \DDD$ and, for all pairs $(X,Y)$ of finite sets, 
\[P^{\DDD}(X;Y) = \coprod_{(\underline c, \underline d) \in \DDD^{|X|} \times \DDD^{|Y|} } \DCat[E]^{\DDD}(\underline c, \underline d),\]
together with composition and monoidal product maps, and an injection $P^{\DDD}(\downarrow ) \hookrightarrow P^{\DDD}(\one;\one)$ that induces the identities for composition.	

% 
%%takes each finite set $Z$ to the set $\{\In, \Out\}^Z$ of ordered partitions $Z = Z_{\In}\amalg Z_{\Out}$ of $Z$ into \textit{input} and \textit{output} sets. % and $\ElS[Di]((X, (X_{\In}, X_{\Out})), (Y, (Y_{\In}, Y_{\Out})))$ is precisely the set of bijections $g \colon Y \to X$ that preserve the partitions. 
%%\srnote{double use of $Y,Z$ throughout.}
%%A \textit{directed } \warn{R 18. This is where I'm up to.... I don't know how to do this!!} 
%So $\ElS[Di]$ is equivalent to the category $\fisinvdi$ obtained from $\fiso\times \fiso^{\mathrm{op}} $ by adjoining a distinguished element $(\downarrow)$ with
%%\begin{itemize} \item
% trivial endomorphism group, % $\fisinvdi(\downarrow, \downarrow) = \{id_\downarrow\}$,
%%\item 
%and, for all pairs $(X, Y)$ of finite sets, and all $x \in X$ and $y \in Y$, \textit{input} morphisms $i_x\colon(\downarrow) \to (X,Y)$ and \textit{output} morphisms $o_y\colon(\downarrow) \to (X,Y)$ that are compatible with the action of $\fiso\times \fiso^{\mathrm{op}} $ (see \cref{fig: directed elements}(d)). 
%%\end{itemize} 

Following \cref{rmk: visualise}, the objects $(X,Y)$ of $\fisinvdi$ may be visualised, %of \textit{directed corollas} whose objects are either \textit{directed corollas} $ C_{X;Y}$ , 
as in \cref{fig: directed elements}(b), as \textit{directed corollas} %$ C_{X;Y}$, 
and the distinguished object $(\downarrow) $ as a %directed loose edge %. for all pairs $(X, Y)$ of finite sets, or, the distinguished 
\textit{directed exceptional edge} %$(\downarrow)$
 (\cref{fig: directed elements}(a)). %Elements $d \in \DDD$ and $\phi \in P_{X;Y}$ of a directed graphical species $P$ are visualised as decorated directed exceptional edges and corollas (compare \cref{fig. species vis}).
 
 
 If $Y = \{r\}$ is a singleton, then the object $(X, \{*\})$ describes a %directed corolla $C_{X;\{r\}}$ is called a 
 \emph{rooted corolla} % and denoted by $t_X \defeq C_{X;\{*\}}$  
 as in \cref{fig: directed elements}(c). See also Examples \ref{ex: operad}, \ref{ex: dendroidal}, \ref{ex: operad endo} on operads.
 %\srnote{0203 shortened sentence}

%Morphisms or directed corollas are in $\ElS[Di]$ are equivalent to morphisms  $i_x, o_y\colon(\downarrow) \to C_{X, Y}$ (induced by $Di(ch_x)$ and $Di(ch_y \circ \tau)$ in $\fisinv(\S, X \amalg Y))$)all $x \in X$ and $y \in Y$, there are morphisms $i_x, o_y\colon(\downarrow) \to (X,Y)$ in $\ElS[Di]$ (induced by $Di(ch_x)$ and $Di(ch_y \circ \tau)$ in $\fisinv(\S, X \amalg Y))$). (See \cref{fig: directed elements}.) 
% 
  %Note that $(\downarrow)$ has no non-trivial endomorphisms in $\ElS[Di]$. 
%  So
%  So, $\ElS[Di]$ is equivalent to the category $\Bifiso$, obtained from $\fiso \times \fiso ^\mathrm{op}$ by adjoining a distinguished element $\downarrow$ and, for all $x \in X$ and $y \in Y$, morphisms $i_x, o_y\colon(\downarrow) \to (X,Y)$ (induced by $Di(ch_x)$ and $Di(ch_y \circ \tau)$ in $\fisinv(\S, X \amalg Y))$).


\begin{figure}[htb!]
	\[	\begin{tikzpicture}
	
	\node at (1.4,-2.3) {(a)};
	\node at (1,0){\begin{tikzpicture}[scale = .6]
		
		\draw[thick]%(0,0)--(0,2)
		%(0,0)--(-1.5,-2)
		%	(0,0) --( 0,2)
		(0,1)--(0,3);
		
		
		
		
		\node at (-.5, 1.3) {\tiny{$\Out$}};
		\node at (-.5, 2.7) {\tiny{$\In$}};
		
		
		
		\end{tikzpicture}};

	\node at (1.8,0){\begin{tikzpicture}[scale = .6]
		
		\draw[ -<-=.5]%(0,0)--(0,2)
		%(0,0)--(-1.5,-2)
		%	(0,0) --( 0,2)
		(0,1)--(0,3);
		
		\end{tikzpicture}};
	
			\node at (5.3, -2.3) {(b)};
	\node at (4,0){\begin{tikzpicture}[scale = .55]
		\draw[thick]%(0,0)--(0,2)
		%(0,0)--(-1.5,-2)
		%	(0,0) --( 0,2)
		(-1.5,0)--(0,2)
		(-1,0)--(0,2)
		(1,0)--(0,2)
		(1.5,0)--(0,2)
		%(0,0)--(1.5,-2)
		(0,2)--(-1,4)
		(0,2)--(-.5,4)
		(0,2)--(1,4);
		
		\draw[dashed]
		(-. 8, 0)--(0.8,0)
		(-.3,4)--(.8,4);
		
		\draw[decoration={brace, raise=5pt},decorate]
		(-1,4) -- node[above=6pt] {\small{$X$}} (1,4);
		\draw[decoration={brace,mirror, raise=5pt},decorate]
		(-1.5,0) -- node[below=6pt] {\small{$Y$}} (1.5,0);
		
		\node at (-1.9, .2) {\tiny{$\Out$}};
		\node at (1.9, .2) {\tiny{$\Out$}};
		\node at (.8, 1.6) {\tiny{$(\In)$}};
		%	\node at (0, -.3){$x_0$};
		\node at (-1.4,3.8) {\tiny{$\In$}};
		\node at (-.8,2.4) {\tiny{$(\Out)$}};
		\node at (1.4, 3.8) {\tiny{$\In$}};
		
		
		
		
		
		
		
		
		%\draw[decoration={brace,raise=5pt},decorate]
		%  (-1.5,2.1) -- node[above=6pt] {\small{$n$ inputs}} (1.5,2.1);
		
		\draw  [ draw=black,   fill=white]
		(0,2)circle (8pt);
		%(0,-0) circle (15pt);
		
		%\node at(0,0) {\small{$\iota $}};
		%	\node at(0,2) {\small{$\phi $}};
		
		\end{tikzpicture}};
	
	\node at (6.6,0){\begin{tikzpicture}[scale = .55]
		\draw[-<-=.3]%(0,0)--(0,2)
		%(0,0)--(-1.5,-2)
		%	(0,0) --( 0,2)
		(-1.5,0)--(0,2);
		\draw[-<-=.3]	(-1,0)--(0,2);
		\draw[-<-=.3]	(1,0)--(0,2);
		\draw[-<-=.3]	(1.5,0)--(0,2);
		%(0,0)--(1.5,-2)
		\draw[-<-=.7](0,2)--(-1,4);
		\draw[-<-=.7](0,2)--(-.5,4);
		\draw[-<-=.7]	(0,2)--(1,4);
		
		\draw[dashed]
		(-. 8, 0)--(0.8,0)
		(-.3,4)--(.8,4);
		
		\draw[decoration={brace, raise=5pt},decorate]
		(-1,4) -- node[above=6pt] {\small{$X$}} (1,4);
		\draw[decoration={brace,mirror, raise=5pt},decorate]
		(-1.5,0) -- node[below=6pt] {\small{$Y$}} (1.5,0);
		
		
		\draw  [ draw=black,   fill=white]
		(0,2)circle (8pt);
		
		\end{tikzpicture}};
		\node at (10,0.1){	\begin{tikzpicture}
		
		\node at (2,0){\begin{tikzpicture}[scale = .6]
			\draw[ultra thick]%(0,0)--(0,2)
			%(0,0)--(-1.5,-2)
			(0,0) --( 0,2);
			%(0,0)--(1.5,-2)
			\draw
			(0,2)--(-1,4)
			(0,2)--(-.5,4)
			(0,2)--(1,4);
			
			\draw[dashed]
			(-.3,4)--(.8,4);
			
			\draw[decoration={brace, raise=5pt},decorate]
			(-1,4) -- node[above=6pt] {\small{$X$}} (1,4);
			
			\draw  [ draw=black,   fill=white]
			(0,2)circle (8pt);
			%(0,-0) circle (15pt);
			\node at (0, -.3){$*$};
			%\node at(0,0) {\small{$\iota $}};
			%	\node at(0,2) {\small{$\phi $}};
			
			\end{tikzpicture}};
		\end{tikzpicture}
	};
		\node at (10,-2.3) {(c)};
	
	\node at (14.5,0){\begin{tikzpicture}[scale = .6]
		\draw[red,thick, -<-=.5]
		(-2.5, 2)--(-2.5,4);
		\draw [red, ->]
		(-1.8,3)--(-1,3);
		\node at (-1.4,3.3) {\tiny{$i_x$}};
		\draw[blue,thick, ->-=.5]
		(3, 2)--(3,0);
		\draw [blue, ->]
		(2.5,1)--(1.7,1);
		\node at (2.2,.7) {\tiny{$o_y$}};
		\draw[-<-=.3]%(0,0)--(0,2)
		%(0,0)--(-1.5,-2)
		%	(0,0) --( 0,2)
		(-1.5,0)--(0,2);
		\draw[ -<-=.3]	(-1,0)--(0,2);
		\draw[blue, thick,-<-=.3]	(1,0)--(0,2);
		\node at (.55, .3){\scriptsize{$y$}};
		\draw[ -<-=.3]	(1.5,0)--(0,2);
		
		
		%(0,0)--(1.5,-2)
		\draw[-<-=.7](0,2)--(-1,4);
		\draw[red, thick,-<-=.7](0,2)--(-.5,4);
		
		\node at (-.2,3.6){\scriptsize{$x$}};
		\draw[-<-=.7]	(0,2)--(1,4);
		
		\draw[dashed]
		(-. 8, 0)--(0.8,0)
		(-.3,4)--(.8,4);
		
		\draw[decoration={brace, raise=5pt},decorate]
		(-1,4) -- node[above=6pt] {\small{$X$}} (1,4);
		\draw[decoration={brace,mirror, raise=5pt},decorate]
		(-1.5,0) -- node[below=6pt] {\small{$Y$}} (1.5,0);
		
		
		\draw  [ draw=black,   fill=white]
		(0,2)circle (8pt);
		
		\end{tikzpicture}};

		\node at (14.5,-2.3) {(d)};
	

	\end{tikzpicture}\]
	\caption{(a) the directed exceptional edge $(\downarrow)$, (b) the pair $(X,Y) \in \fisinvdi$ describes a directed corolla, (c) $(X, \{*\})$ describes a  rooted corolla, (d) input and output morphisms in $\fisinvdi$.}
	\label{fig: directed elements}
\end{figure}




%\srnote{1503 -careful with the unit}


%More generally, for any set $\DDD$, a $\DDD$-\textit{coloured PROP} is a strict symmetric monoidal category whose monoid of objects is freely generated by $\DDD$, and a 


%In particular, PROPs admit an equivalent description in terms of graphical species: For, 
Let $Di$ be the terminal $\Dipal$-coloured graphical species defined in \cref{Comm c}. Then, %let $\Disig$ be the unique non-identity involution on the set $\Di \defeq \{\In, \Out\}$ and let $Di \defeq\CComm[\Dipal]{}$ be the terminal $\Dipal$-coloured graphical species. 
for each finite set $X$, $Di_X  =\{\In, \Out\}^X$ is the set of partitions $X = X_{\In}\amalg X_{\Out}$ of $X$ into \textit{input} and \textit{output} sets, with blockwise action of the partition-preserving isomorphisms in $\ElS[Di]$. Hence, $\ElS[Di] \simeq \fisinvdi$ canonically and so $ \GS \ov Di \cong \pr{\ElS[Di]}$ is equivalent to the category $\pr{\fisinvdi}$ of \textit{directed graphical species}. The subcategory $\CGS[\Dipal] \ov Di $ of  \textit{monochrome directed graphical species} is equivalent to $ \pr{\fiso \times \fiso^{\mathrm{op}}}$. In particular, PROPs may be described in terms of graphical species. % of monochrome directed graphical species. 

%%\srnote{0203 removed unused notation (slash)DiGS. Something about monochrome directed graphical species... }

%
%Namely, for any set $\DDD$, the pairing $ (d, \In) \leftrightarrow (d, \Out)$ defines a canonical involution $\DisigD$ on $\DDD \times \Di$.
%
%If a graphical species $S$ has palette $(\CCC, \omega)$ and is equipped with an {`orientation'} $\gamma\colon S \to Di$, then $\gamma$ induces an involution preserving isomorphism
%$(\CCC, \omega) \cong \DipalD[\widetilde \CCC]$ where, for any set $\DDD$, $\DisigD$ is the canonical involution $ (d, \In) \leftrightarrow (d, \Out)$ on $\DDD \times \Di$. 
%
%Therefore, a directed graphical species $(S, \gamma)$ is equivalently an object in $\CGS[\DipalD]$ for some set $\DDD$.
%As such, the extra structure of orientation actually simplifies the combinatorics of graphical species in $\GS \ov Di$. 
%%%\srnote{got rid of stuff here... check I don't use it} 
\end{ex}

\subsection{Multiplication and contraction on graphical species}

Intuitively, a multiplication $\diamond$ on a graphical species $S$ is a rule for combining (gluing) distinct elements of $S$ along pairs of legs (called `ports') with dual colouring as in \cref{multiplication}: %whose colours are matched by the involution. 
 \begin{figure}[htb!]
	
	%\begin{figure}[H] 
	%\centering{
	\begin{tikzpicture}
	\node at (0,0){\begin{tikzpicture}[scale = 0.5]
		%\filldraw(0,0) circle(3pt);
		\foreach \angle in {-0,90,180,270} 
		{
			\draw(\angle:0cm) -- (\angle:1.5cm);
			
			
		}
		\draw [  thick] (0,0) -- (1.5,0);
		
		\node at (-1, -0.3) {};
		\node at (0.3, 1) {};
		\node at (1, -0.5) {\tiny {$(x)$}};
		\node at (1, 0.3) {\tiny c};
		\node at (0.3,-1) {};
		
		\draw  [ draw=red,   fill=white]
		(0,0) circle (15pt);
		
		\node at(0,0) {\small{$\phi $}};
		%\node at(0,-2) {\small{$\phi_2 $}};
		\end{tikzpicture}
	};
	
	
	
	\node at (2,0){\begin{tikzpicture}[scale = 0.5]
		%\filldraw(0,0) circle(3pt);
		\foreach \angle in {60,180, 300} 
		{
			\draw(\angle:0cm) -- (\angle:1.5cm);
			
			
			
		}
		\draw [  thick] (0,0) -- (-1.5,0);
		\node at (-1, 0.3) {\tiny {$\omega c$}};
		\node at (-1, -0.5) { \tiny{$(y)$} };
		\node at (1, 0.8) {};
		\node at (1, -0.8) {};
		\draw  [ draw=red,   fill=white]
		(0,0) circle (15pt);
		
		\node at(0,0) {\small{$\psi $}};
		
		
		\end{tikzpicture}};
	
	% \node at (2,-1.5){$\CX[Y]$};
	
	\node at (4,0){\large $\longrightarrow$};
	
	\node at (6,0) 
	{\begin{tikzpicture}[scale = 0.5]
		%\filldraw(0,0) circle(3pt);
		\foreach \angle in {-0,90,180,270} 
		{
			\draw(\angle:0cm) -- (\angle:1.5cm);
			\draw[thick]
			(0,0)--(2.1,0);
			\draw  [ draw=red,   fill=white]
			(0,0) circle (15pt);
			
			\node at(0,0) {\small{$\phi  $}};
			
			
			
		}
		
		\end{tikzpicture}};
	
	\node at (7,0){\begin{tikzpicture}[scale = 0.5]
		%\filldraw(0,0) circle(3pt);
		\foreach \angle in {60,180, 300} 
		{
			\draw(\angle:0cm) -- (\angle:1.5cm);
			
			
			
		}
		\draw [  thick] (0,0) -- (-1.5,0);
		\draw  [ draw=red,   fill=white]
		(0,0) circle (15pt);
		
		\node at(0,0) {\small{$ \psi $}};
		
		\end{tikzpicture}};
	
	\draw  [ draw=blue]
	(6.5,0) ellipse (30pt and 14 pt);
%	\node at (6.25,0.1){\tiny{$\omega c$}};
	
	\node at (6.5,-1.5){ $\phi \diamond_{x,y} \psi$};
	
\end{tikzpicture}

\caption{Multiplication}
\label{multiplication} 	
\end{figure}


The notation `$\pto$' denotes a partial map of sets: $f \colon A \pto B$ is given by a function $A' \to B$ with $A' \subset A$.
 
\begin{defn}\label{defn: multiplication}\label{coloured mult cont} %Let $S$ be a $(\CCC, \omega)$- coloured graphical species. 
	A \emph{multiplication} $\diamond$ on a graphical species $S$ is given by a family of partial maps %%\srnote{RG? in terms of limits?}
	\begin{equation} \label{eq: mult def} - \diamond^{X,Y}_{x,y} - \colon S_{X \amalg \{x\}} \times S_{Y \amalg \{y\}} \pto S_{X \amalg Y},\end{equation} 
	defined (for all $X,Y$) when %for all pairs $X, Y$ of finite sets and all pairs 
	$\phi \in S_{X \amalg \{x\}}, \psi \in  S_{Y \amalg \{y\}}$ satisfy $S(ch_x)(\phi) = S(ch_y \circ \tau)(\psi)$. 

The multiplication $\diamond$ satisfies the following conditions:
  \begin{enumerate}[(m1)]%%\srnote{Do I use the commutativity axiom anywhere? Iso follows from equivariance. Remove axiom? Possibly use in uniqueness of unit. leave as is..}
 	\item \emph{(Commutativity axiom.)}\\
 	Wherever $\diamond^{X,Y}_{x,y}$ is defined, %\srnote{R20}
 	\[\psi \diamond^{Y,X}_{y,x} \phi =  \phi \diamond^{X,Y}_{x,y} \psi \] %for all finite sets $X,Y$ and all pairs $\phi \in S_{X \amalg \{x\}}$, $\psi \in S_{Y \amalg \{y \}}$ for which the map is defined.
 	\item \emph{(Equivariance axiom.)}\\
 	%The multiplication $\diamond$ respects the action of $\fiso$ on $S$:
 	For all bijections $ \sigma\colon X \xrightarrow{\cong} W$ and $\rho\colon Y \xrightarrow{\cong} Z$ that extend to bijections $\hat \sigma \colon X \amalg \{x\} \xrightarrow{\cong} W \amalg \{w\}$ and $\hat \rho \colon Y \amalg \{y\} \xrightarrow{\cong} Z \amalg \{z\}$,
 		\[ S( \sigma \sqcup  \rho )(\phi \diamond ^{W,Z}_{w,z} \psi) = S(\hat \sigma)(\phi) \diamond^{X,Y}_{x,y} S(\hat \rho)(\psi),\]
 	(where $ \sigma \sqcup  \rho\colon X \amalg Y \xrightarrow{\cong} W \amalg Z$ is the block permutation).
 	
 \end{enumerate}
 
 A \emph{unit for the multiplication $\diamond$} is a map 
 $\epsilon\colon S_\S \to S_\two $, $c \mapsto \epsilon_c$ such that, for all $X$ and all $\phi \in S_{X \amalg \{x\}}$ with $S(ch_x) = c \in S_\S$, 
 \[ \phi \diamond^{X, \{1\}}_{x,2} \epsilon_c = \epsilon_c \diamond^{\{1\},X}_{2,x} \phi = \phi.\]
A multiplication $\diamond$ is called \emph{unital} if it has a unit $\epsilon$. In this case 
% If $\epsilon$ is a unit for $\diamond$ then $\diamond$ is said to be \emph{unital} and 
 %The map $\epsilon$ is called a \emph{unit} for $\diamond$, and, 
$ \epsilon _c$ is a \emph{$c$-coloured unit for $\diamond$}. 

\end{defn}


If $(\diamond,\epsilon\colon \CCC \to S_\two)$ is a unital multiplication on a $(\CCC, \omega)$-coloured graphical species $S$, then $\epsilon_c \in S_{(c, \omega c)}$ for all $c \in \CCC$. So a unit map $\epsilon\colon \CCC \to S_\two$ is injective. %Observe that there is an involution $ S(\sigma_\two) $ on $S_\two$ induced by the unique non-identity endomorphism in 
Let $\sigma_\two\in \fisinv (\two, \two) $ be the unique non-identity endomorphism. %\srnote{shortened sentence}

%Let $S$ be a $(\CCC, \omega)$-coloured graphical species with multiplication $\diamond$.
\begin{lem} \label{lem: unique and equivariant}If $\diamond$ admits a unit $\epsilon: \CCC \to S_\two$, it is unique. Moreover, $\epsilon$ is compatible with the involutions $\omega = S_\tau$ on $\CCC$ and $S(\sigma_\two)$ in that %\srnote{removed incorrect set membership}
	\begin{equation}
	\label{eq: unit compatible with involution}
	\epsilon \circ  \omega  = \epsilon \circ S_\tau  = S(\sigma_\two)  \circ \epsilon\colon \ \CCC \to S_\two.
	\end{equation}
	%	
	%	, for each $c \in \CCC$, the $c$-coloured unit $\epsilon_c$  is unique, and commutes with the involutions $\omega\colon \CCC\to \CCC$ and the non-identity automorphism $\sigma_\two \in \fisinv(\two, \two)$. That is
\end{lem}
\begin{proof}
	
	Let $\lambda\colon \CCC \to S_\two$, $c \mapsto \lambda_c$ be another unit for $\diamond$. Then, for all $c \in \CCC$,
	\[ \epsilon_c = \epsilon_c \diamond^{\{1\},\{1\}}_{2,2} \lambda_c = \lambda_c  \diamond^{\{1\},\{1\}}_{2,2} \epsilon_c = \lambda_c, \] whence $\epsilon$ is unique. The second statement follows from the defining properties of multiplication. Namely,
		\[\begin{array}{c}
	S(\sigma_\two)  (\epsilon_c )  =  S(\sigma_\two)(\epsilon_{ c} )\diamond^{\{1\}, \{1\}}_{2,2}\epsilon_{\omega c} =  S(\hat \sigma_\two \sqcup id_{\{1\}})( \epsilon_c \diamond^{\{2\}, \{1\}}_{1,2} \epsilon_{\omega c}) %&\ \text{ by equivariance of $\diamond$,}\\
	 =  \epsilon_c \diamond^{\{2\}, \{1\}}_{1,2} \epsilon_{\omega c} %\ \text{ since $\hat{\sigma _\two}$ is a bijection of singleton sets,}\\
	 = \epsilon_{\omega c} \diamond^{\{2\}, \{1\}}_{1,2}\epsilon_c%&\  \text{ by commutativity of $\diamond$,}
 =  \epsilon_{\omega c}.%&\ \text{ by definition of the unit.}
	\end{array}\]
\end{proof}

\begin{rmk}	\label{rmk: mult notation}
%	(See also \cref{rmk: cont notation}.)%\srnote{0203 - I hate these remarks}
Equivalently, a multiplication $\diamond$ on $ (\CCC, \omega)$-coloured graphical species $S $ is a family of maps 
 	\begin{equation}\label{eq. coloured mult}- \diamond^{\underline c, \underline d}_{c} - \colon S_{(\underline c, c) } \times S_{(\underline d, \omega c)} \to S_{(\underline c \underline d)}, \ \text{ for } c \in \CCC,\  \underline c \in \CCC^X, \  \underline d \in \CCC^ Y,\end{equation}
 % for $c \in \CCC$, $\underline c \in \CCC^X$, $\underline d \in \CCC^ Y$.
Both (\ref{eq: mult def}) and (\ref{eq. coloured mult}) are used in what follows. Where the context is clear, the superscripts may be dropped altogether.
  
%  The notation $\diamond^{X,Y}_{x,y}$ introduced in \cref{defn: multiplication} is clumsier but has the advantage of greater precision, particularly in describing the symmetry actions. 
 

\end{rmk}



As one would expect, a multiplication $\diamond$ on a graphical species $S$ is called `associative' if the result of several consecutive multiplications does not depend on their order. This is stated precisely in condition (C1) of \cref{defn: Modular operad}, and visualised in the figure therein.% (See also the figure therein, for a visualisation of the associativity axiom.)
%\srnote{0203 - sentence made more compact}


\begin{ex}\label{cyclic}
	
	A graphical species $O$ equipped with a unital, associative multiplication $(\diamond , \epsilon)$ is a cyclic operad in the sense of \cite{DCH19}. When the involution is trivial, these are the \textit{entries-only} cyclic operads of \cite{CO20} (see there for a comparison with cyclic operads as introduced in \cite{GK95}).
	
	
		Some advantages of the involutive, graphical species approach to cyclic operads are discussed in \cite{DCH19} and \cite[Introduction]{HRY19b}.%\srnote{0303 small change, added the comparison to classical defn}
\end{ex}

\begin{ex}
	\label{ex: operad}%\srnote{RG?? 2602 some changes} 
	To describe operads in terms of graphical species, recall
the graphical species $Di$ introduced in \cref{Comm c}, and that $\ElS[Di]\simeq \fisinvdi$ by \cref{ex:direction}, where objects of $\fisinvdi$ are either the exceptional directed edge $(\downarrow)$, or pairs $(X, Y)$ of finite sets. 

If $Y \cong \{*\}$ is a singleton, then $(X, \{*\})$ is called a rooted corolla, and denoted by $t_X$. Let $\Bifiso \subset \fisinvdi$ be the full subcategory on $(\downarrow)$ and the rooted corollas $t_X$ (for all finite sets $X$).


%tion in terms of directed graphical species equipped with a unital multiplication. 

%The $\Dipal$-coloured graphical species $Di$ was introduced in \cref{comm c}, and the category $\fisinvdi$ such that $\ElS[Di ] \cong \fisinvdi$ was described in \cref{ex:direction}. Objects of $\fisinvdi$ are either the exceptional directed edge $(\downarrow)$, or pairs $(X, Y)$ of finite sets. When $Y \cong \{*\}$ is a singleton, $(X, \{*\})$ is called a rooted corolla, and denoted by $t_X$.% that, $\ElS[Di ] \cong \fisinvdi$,for a finite set $X$
%	
%Objects of the form $(X, \{*\})$ in $\fisinvdi$ Recall from \cref{ex:direction} that, for a finite set $X$, the rooted corolla $t_X$ is an object of the form $(X, \{*\})$ in $\fisinvdi$, and that $(\downarrow) \in \fisinvdi$ denotes the exceptional directed edge.  %the , and the definition of rooted corollas $t_X$ in terms of objects $(X, \{*\})$ of $\fisinvdi$, where $X$ is a finite set. 

 Presheaves $O \colon{ \Bifiso }^{\mathrm{op}}$ are described by a set $\DDD = O(\downarrow)$ and sets $O(\underline c;d)$, defined for all $d \in \DDD$ and $\underline c \in \DDD^X$ (for all finite sets $X$). The action of $\fiso$ on $O$ induces isomorphisms $O((c_x)_x; d) \cong O((c_{f(x)})_x;d)$ for all $f \colon X \xrightarrow {\cong} Y$. So, a $\DDD$- coloured operad is a $\Bifiso$ presheaf $O$, together with an operadic composition, and unit elements $1_d \in O(d;d)$ for all $d \in \DDD  = O(\downarrow)$.

The graphical species $RC \subset Di$  is %$\Dipal$-coloured 
 given by essential image of $\Bifiso \subset \fisinvdi$ under the equivalence $\fisinvdi \simeq \ElS[Di]$. So, $RC_\S = Di_\S = \{\In, \Out\}$, $RC_\nul = \emptyset$ and, for all finite sets $X$, $RC_{X \amalg \{*\}}$ consists of those $\phi \in Di_{x \amalg \{*\}}$ such that 
\[ Di (ch_x)(\phi) = (\In) \text { for all } x \in X, \text { and } Di (ch_{*}) (\phi) =( \Out). \]

Clearly, $RC$ inherits the trivial unital multiplication from $Di$. Moreover, a presheaf $O \colon {\Bifiso}^{\mathrm{op}} \to \Set$ has the structure of an operad precisely when the corresponding graphical species $O^{\GS} \in \GS \ov RC$ is equipped with an associative unital multiplication. %precisely when the corresponding presheaf $O \colon {\Bifiso}^{\mathrm{op}} \to \Set$ has the structure of an operad. 
% There is a graphical species $RC \subset Di$ such that 
Hence, the category $\Op$ of (symmetric) operads %(see e.g.\ \cite{BM07}) 
 is equivalent to the category whose objects are objects of $\GS \ov RC $ %(or\textit{ species of rooted corollas}) 
 equipped with an associative unital multiplication,
%\[ \diamond^{X,(Y \amalg \{r_y\})\setminus \{y\}}_{r, x} \colon S(X;\{r_x\})\times S(Y; \{r_y\}) \to S(X \amalg Y\setminus \{y\}; \{r_y\})\],
and whose morphisms are morphisms in $ \GS \ov RC$ that preserve the multiplication and units.

%Recall from \cref{ex:direction} that $\ElS[Di ] \cong \fisinvdi$, where objects of $\fisinvdi$ are either the exceptional directed edge $(\downarrow)$, or pairs $(X, Y)$ of finite sets. When $Y \cong \{*\}$ is a singleton, $(X, \{*\})$ is called a rooted corolla, and denoted by $t_X$. 

%\[   \phi \in RC_{X \amalg \{x'}} \text { if and only if } Di (ch_x')(\phi) = Di (ch_{x'}) \colon RC_{X \amalg \{*\}} \mapsto \Out \in \Di$ if and only if $x'  = *$. 

%  for all finite sets $X$, $\underline c \in \DDD^X$ and $d \in \DDD$, sets $O(\underline c;d)$, together with isomorphisms induced by the action of $\fiso$. 

%The $\Dipal$-coloured graphical species $Di$ was introduced in \cref{comm c}. By \cref{ex:direction}, $\ElS[RC] \simeq \Bifiso$, where $RC \subset Di$ is the $\Dipal$-coloured (directed) \emph{graphical species of rooted corollas} defined by $ch_{x'} \colon RC_{X \amalg \{*\}} \mapsto \Out \in \Di$ if and only if $x'  = *$. %, then $\ElS[RC] \simeq \Bifiso$ by \cref{ex:direction}. %Given a presheaf $O$ on $\Bifiso$
%%Objects of the category $\Op$ of (symmetric) coloured operads in $\Set$ (see e.g.\ \cite{BM07}) are presheaves $O \colon \Bifiso^{\mathrm{op}} \to \Set$ together wi

%$(X; \{*\})$ and $(\downarrow)$ $ \fiso  \cong \fiso \times \{*\} \hookrightarrow \fiso \times \fiso$Let $RC \subset Di$ be the $\Dipal$-coloured (directed) \emph{graphical species of rooted corollas}: elements are rooted trees $t_X = C_{X;{r}}$ with leaves decorated by finite sets $X$, or the distinguished directed edge $(\downarrow)$. So, $RC$ is equivalent to the category obtained from the full subcategory of $ \fisinvdi$ on the objects $(\downarrow)$ and $(X, \{r\})$, for all finite sets $X$. 



%In particular, a $\Dipal$-coloured species of rooted corollas $(S, \gamma)$ is described by a collection of sets $S_X = S(X; \{r\})$ for all finite sets $X$, together with an action by $\fiso$: in other words, $S$ is a species. If $S$ is equipped with an associative, unital multiplication $(\diamond, \epsilon)$, then the operad structure is given by
%\[\circ_i \colon S^O(n) \times S^O(m) \to S^O(n + m -1), \ \text{ for all } m, n \in \N, \ 1 \leq i \leq n,\] where $S(k) \defeq S_{\mathbf k; \{*\}}$ for all $k \in \N$ and 
%\[\circ_i \defeq \diamond^{\mm,(\nn \amalg \{r_n\})\setminus \{i\}}_{r_m, i} \colon S(\mm;\{r_m\})\times S(\nn; \{r_n\}) \to S((\mm  \amalg \nn)\setminus \{i\}; \{r_n\}).\]
%\warn{Notation not consistent here... depends on notation in \cref{ex:direction}}
%%\[\circ_i \colon S^O(n) \times S^O(m) \to S^O(n + m -1), \ \text{ for all } m, n \in \N, \ 1 \leq i \leq n,\] where $S(k) \defeq S_{\mathbf k; \{*\}}$ for all $k \in \N$ and $\circ_i$ by an assos
% %Though the symmetric sequence 
%
%
\end{ex}

\begin{rmk}
	Examples \ref{cyclic} and \ref{ex: operad} highlight the expressive power of graphical species. The involution $\tau$ on $\S$ means that (undirected) cyclic operads and (directed) operads may be expressed in terms of presheaves on the same underlying category. (See also Examples \ref{ex:direction} and \ref{ex: wheeled prop}.)
\end{rmk}

%Just as a while loop in a simple piece of code creates the possibility of infinite runtime, 

%\srnote{0203 slight reordering}
Intuitively, a contraction $\zeta$ on a graphical species $S$ may be thought of as a rule for `self-gluing' single elements of $S$ along pairs of ports with dual colouring (\cref{contraction}). The presence of a contraction operation enables modular operads to encode algebraic structures -- such as those involving trace -- that ordinary operads cannot \cite{MMS09, Mer10}.
%%\srnote{R21 - Merkulov.... I would like to add a nice physical example here...}
\begin{figure}[htb!] %\label{multiplication}
	
	\begin{tikzpicture}
	
	\node at (0,0){\begin{tikzpicture}[scale = 0.5]
		%\filldraw(0,0) circle(3pt);
		\foreach \angle in {-0,90,180,270} 
		{
			\draw(\angle:0cm) -- (\angle:1.5cm);
			
			
		}
		\draw [  thick] (0,0) -- (1.5,0);
		\draw [  thick] (0,0) -- (-1.5,0);
		\node at (-1, 0.3) {\tiny c};
		\node at (-1, -0.3) {\tiny (x)};
		%  \node at (0.3, 1) {};
		\node at (1, -0.3) {\tiny (y)};
		\node at (1, 0.3) {\tiny {$\omega c$}};
		
		\draw  [ draw=red,   fill=white]
		(0,0) circle (15pt);
		
		\node at(0,0) {\small{$ \phi $}};
		%\node at (0.3,-1) {\tiny 4};
		\end{tikzpicture}};

	
	
	\node at (2.5,0){\large $\longrightarrow$};
	
	\node at (5,0) 
	{\begin{tikzpicture}[scale = 0.5]
		%\filldraw(0,0) circle(3pt);
		\draw (0,-1.5)--(0,3.5);
		\draw[ thick] 
		(0,0)..controls (3,3) and (-3,3)..(0,0);
		\node at (-1.5,1) {\tiny {$(y)$}};
		% \node at (0.3, 1) {\tiny 2};
		\node at (1.5, 1) {\tiny {$(x)$}};
		%\node at (0.3,-1) {\tiny 2};
		
		
		\draw  [ draw=red,   fill=white]
		(0,0) circle (15pt);
		
		\node at(0,0) {\tiny{$\phi $}};
		\draw  [ draw=blue]
		(0,1) ellipse (30pt and 60 pt);   
		\end{tikzpicture}};
	
	
	
	\node at (5,-2){ $ \zeta_{x,y} (\phi )$};
	
\end{tikzpicture}
\caption{ Contraction}\label{contraction}


\end{figure}


\begin{defn}\label{defn: contraction}


A \emph{contraction} $\zeta$ on $ S$ is given by a family of partial maps 
\begin{equation}\label{eq: cont def} \zeta^X_{x,y}\colon S_{X \amalg \{x,y\}} \pto S_{X}\end{equation}
defined for all finite sets $X$ and all $\phi \in S_{X \amalg \{x, y\}},$ such that $ S(ch_x)(\phi) = S(ch_y\circ \tau)(\phi)$, and {equivariant} with respect to the action of $\fiso $ on $S$: 
If $\hat \sigma\colon X \amalg \{x,y\} \xrightarrow{\cong} Z \amalg\{w,z\}$ extends the bijection $ \sigma\colon X \xrightarrow{\cong} Z$ by $\hat\sigma(x) = w,\hat \sigma(y) = z$, then for any $\phi \in S_{Z \amalg \{w,z\}}$, we have
\[ S( \sigma) \left( \zeta^Z_{w,z}(\phi) \right ) = \zeta^X_{x,y}\left (S(\hat \sigma)(\phi) \right ).\]
 \end{defn}


If $\zeta$ is a contraction on $S$, then by, equivariance, $\zeta^X_{x,y}( \phi )= \zeta^X_{y,x} (\phi)$ wherever defined. 

\begin{rmk}\label{rmk: cont notation}%(See also \cref{rmk: mult notation}.) %\srnote{limits?}
		 A contraction $\zeta$ on a $(\CCC, \omega)$-coloured graphical species $S$ is equivalently a family of maps 
		\[ \zeta ^{\underline c}_c\colon S_{(\underline c, c, \omega c)}  \to S_{\underline c }\]
for $c \in \CCC$, and $\underline c \in \CCC^X$. Depending on context, both $\zeta ^{\underline c}_c$ (and even $\zeta_{c}$%, where the context is clear
) and $\zeta^X_{x,y}$ will be used. % will often be used in place of the more precise, but clunkier $\zeta^X_{x,y}$.

\end{rmk}


Let $S$ be a $(\CCC, \omega)$-coloured graphical species equipped with a unital multiplication $(\diamond, \epsilon)$ and contraction $\zeta$. By \cref{lem: unique and equivariant}, there is a \emph{contracted unit} map%%\srnote{dimension? RG?}
%\[ o \defeq \zeta \epsilon\colon \CCC \to S_\nul,  \] such that,  for all $c \in \CCC$, by \cref{lem\colon unique and equivariant} 
\begin{equation}\label{eq: unit contraction} o \defeq \zeta \epsilon: \CCC \to S_\nul, \text{ satisfying } \zeta_c (\epsilon_c) = \zeta_{\omega c} (\epsilon_{\omega c}) \text{ for all } c \in \CCC. \end{equation}

%\begin{rmk}
%We shall see 
As will be explained in Sections \ref{degenerate} and \ref{s. Unital}, the contracted units $o\colon {S_\S}\to S_\nul$  present the main challenge for describing the combinatorics of modular operads.
%\end{rmk}


\subsection{Modular operads: definition and examples}
Modular operads are graphical species with multiplication and contraction operations that satisfy the nicest possible (mutual) coherence axioms.% \warn{These axioms are visualised in Figure \ref{fig: coherence}. }

\begin{defn}\label{defn: Modular operad}
A \emph{modular operad} is a graphical species $S$, with palette $(\CCC, \omega)$, say, together with a unital multiplication $(\diamond,\epsilon)$, % with unit $\epsilon\colon {S_\S}\to S_{\two}$,
 and a contraction $\zeta$, satisfying the following four \emph{coherence axioms}  %-- (C1)-(C4) in the statement of \cref{unpointed modular operad} -- 
governing their composition:

%%T\warn{make text in diagrams larger and add mapsto arrows to the grey arrows.}
%
%%\begin{itemize}
%%\item 
%%Let $S$ have palette $(\CCC, \omega)$.
%%\srnote{1703 these equals signs  in diagrams}
%%\hspace{-10pt}
\begin{minipage}{.55\textwidth}
\emph{(C1)}	\emph{Multiplication is associative.}\\
For all $\underline b \in \CCC^{X_1}, \underline c \in \CCC^{X_2}, \underline d\in \CCC^{X_3}$ and all  $c, d \in \CCC$, the following square commutes:
%\begin{equation}\label{eq: C1}
\[
\xymatrix{
	S_{(\underline b, c)} \times S_{(\underline c, \omega c, d)} \times S_{(\underline d, \omega d)} 
	\ar[rr]^-{\diamond_c \times id}
	\ar[dd]_{id \times \diamond_d} &&
	S_{(\underline b \underline c, d)}\times S_{(\underline d, \omega d)} 
	\ar[dd]^{\diamond_d  }\\
	&{}&\\
	S_{(\underline b, c)}\times  S_{( \underline c,  \omega c, \underline d)}
	\ar[rr]_-{\diamond_c} &&
	S_{\underline b\underline c\underline d}. }%\end{equation}
\]

\end{minipage}
\begin{minipage}{.45\textwidth}
	\begin{figure}[H]
	\includestandalone[width = \textwidth]{standalones/axiom1}
%	\caption{Associativity}
\end{figure}
\end{minipage}

\begin{minipage}{.55\textwidth}
	\emph{(C2)} \emph{Order of contraction does not matter.} \\For all $\underline c \in \CCC^X$ and $c, d \in \CCC$, the following square commutes:%  the following diagram commutes:
	 	 \[\xymatrix{
	S_{(\underline c, c, \omega c, d, \omega d)} \ar[rr]^-{\zeta_c }\ar[dd]_{\zeta_d} && 
	S_{(\underline c, d, \omega d) }\ar[dd]^{\zeta_d}\\
	&{}&\\\
	S_{(\underline c, c, \omega c)}\ar[rr]_-{\zeta_c} &&S_{\underline c}.}\]

	
\end{minipage}
\begin{minipage}{.45\textwidth}
	\begin{figure}[H]
		\includestandalone[width = \textwidth]{standalones/axiom2}
		%	\caption{Associativity}
	\end{figure}
\end{minipage}

\begin{minipage}{.5\textwidth}
	\emph{(C3)}\emph{ Multiplication and contraction commute.} \\For all $\underline c \in \CCC^{X_1}$, $\underline d \in \CCC^{X_2}$ and $c, d \in \CCC$, the following square commutes.
	\[
	\xymatrix{
	S_{(\underline c, c, \omega c, d) } \times S_{(\underline d, \omega d)}
	\ar[rr]^-{\zeta_c \times id}
	\ar[dd]_ {\diamond_d} &&
	S_{(\underline c, d)} \times S_{(\underline d, \omega d)} 
	\ar[dd]^{\diamond_d}\\
	&{}&\\
	S_{(\underline c,c,\omega c,\underline d )}
	\ar[rr]_-{\zeta_c} &&
	S_{\underline c\underline d}}\]
\end{minipage}
\begin{minipage}{.48\textwidth}
	\begin{figure}[H]
		\includestandalone[width = \textwidth]{standalones/axiom3}
		%	\caption{Associativity}
	\end{figure}
\end{minipage}

\begin{minipage}{.55\textwidth}
	\emph{(C4)} \emph{`Parallel multiplication' of pairs.}\\For all $\underline c \in \CCC^{X_1}$, $\underline d \in \CCC^{X_2}$, and $c, d \in \CCC$, the following square commutes:
%	\includestandalone[width = 1\textwidth]{axiom4}
	\[
	\xymatrix{
	S_{(\underline c,  c, d)} \times S_{(\underline d, \omega c, \omega d)}
	\ar[rr]^-{ \diamond_c}
	\ar[dd]_{ \diamond_d}&&
	S_{(\underline c, d,  \underline d, \omega d)}
	\ar[dd]^{\zeta_d}\\&{}&\\
	S_{(\underline c,c, \underline d, \omega c)}\ar[rr]_-{\zeta_c}&&
	S_{\underline c  \underline d}}\]

\end{minipage}
\begin{minipage}{.45\textwidth}
	\begin{figure}[H]
		\includestandalone[width = \textwidth]{standalones/axiom4}
		%	\caption{Associativity}
	\end{figure}
\end{minipage}

%
%%\end{itemize}
%%
%%the following diagram commutes.
%%\[
%%\xymatrix{
%%S_{(\underline b, c)} \times S_{(\underline c, \omega c, d)} \times S_{(\underline d, \omega d)} 
%%\ar[rrr]^-{\diamond_c \times id}
%%\ar[dd]_{id \times \diamond_d} &&&
%%S_{(\underline b \underline c, d)}\times S_{(\underline d, \omega d)} 
%%\ar[dd]^{\diamond_d  }\\
%%&&&\\
%%S_{(\underline b, c)}\times  S_{( \underline c,  \omega c, \underline d)}
%%\ar[rrr]_-{\diamond_c} &&&
%%S_{\underline b\underline c\underline d} }\]
%
%
%
%%\item [(C2)] 
%
%
% 	For a finite set $X$, $\underline c \in C^X$ and $c, d \in C$,  the following diagram commutes
%% 	 \[\xymatrix{
%%S_{(\underline c, c, \omega c, d, \omega d)} \ar[rrr]^-{\zeta_c }\ar[dd]_{\zeta_d} &&& 
%%S_{(\underline c, d, \omega d) }\ar[dd]^{\zeta_d}\\
%%&&&\\\
%%S_{(\underline c, c, \omega c)}\ar[rrr]_-{\zeta_c} &&&S_{\underline c}}\]
%%commutes.
%
%
%%	\begin{figure}[H]
%\includestandalone[width = 1\textwidth]{axiom2}
%%	\end{figure}
%
%
%
%
%%The second pair of coherence conditions relate the multiplication $\diamond$ and the contraction $\zeta$ to each other.
%%\begin{itemize}
%%\item [(C3)]
%For finite sets $X_1$ and $X_2$, $\underline c \in C^{X_1}$, $\underline d \in C^{X_2}$ and $c, d \in C$, the following diagram commutes.
%\includestandalone[width = 1\textwidth]{axiom3}
%%\[
%%\xymatrix{
%%S_{(\underline c, c, \omega c, d) } \times S_{(\underline d, \omega d)}
%%\ar[rrr]^-{\zeta_c \times id}
%%\ar[dd]_ {\diamond_d} &&&
%%S_{(\underline c, d)} \times S_{(\underline d, \omega d)} 
%%\ar[dd]^{\diamond_d}\\
%%&&&\\
%%S_{(\underline c,c,\omega c,\underline d )}
%%\ar[rrr]_-{\zeta_c} &&&
%%S_{\underline c\underline d}}\]
%
%%\item [(C4)] For finite sets $X_1, {X_2}$, $\underline c \in C^{X_1}$, $\underline d \in C^{X_2}$, and $c, d \in C$, the following digram commutes.
%\includestandalone[width = 1\textwidth]{axiom4}
%%\[
%%\xymatrix{
%%S_{(\underline c,  c, d)} \times S_{(\underline d, \omega c, \omega d)}
%%\ar[rrr]^-{ \diamond_c}
%%\ar[dd]_{ \diamond_d}&&&
%%S_{(\underline c, d,  \underline d, \omega d)}
%%\ar[dd]^{\zeta_d}\\&&&\\
%%S_{(\underline c,c, \underline d, \omega c)}\ar[rrr]_-{\zeta_c}&&&
%%S_{\underline c  \underline d}}\]
%%commutes.
%
%
%%\end{itemize}
%
%
%
%%The multiplication $\diamond$ on $S$ is \emph{unital}: If $S$ has palette $(\CCC, \omega)$, then, for each $ c \in C$ of $S$, there is a unique element $ \epsilon_c $ of $ S_\two $ that acts a \emph{$c$-coloured unit} for $\diamond$.
%%
%%That is 
%%
%%\warn(Write out unit equations)

Modular operads form a category $\CSM$ whose morphisms are morphisms of the underlying graphical species that preserve multiplication, contraction and multiplicative units. 

\end{defn}

 Informally, the multiplication and contraction operations describe rules for \textit{collapsing} edges of graphs that represent formal compositions of elements. %contraction and multiplication. 
 The coherence axioms (C1)-(C4) say that this is independent of the order in which the edges are collapsed. %%\srnote{small change to this sentence}% does not matter.

%\begin{figure}[!htb]
%	{
%		\begin{tabular}{ll}
%			
%			
%			\includestandalone[width = .5\textwidth]{axiom1}
%			&
%			\includestandalone[width = .5\textwidth]{axiom2}\\
%			
%			\includestandalone[width = .5\textwidth]{axiom3}
%			&
%			\includestandalone[width = .5\textwidth]{axiom4}
%			
%		\end{tabular}
%	}\label{fig: coherence}
%	\caption{Visualising the coherence axioms (C1)-(C4).} 
%	\end{figure}
%\warn{add labels for the figures..}


\begin{rmk} \label{rmk:non-unital}
 A \emph{non-unital modular operad} $(S, \diamond, \zeta)$ is a graphical species $S$ equipped with a multiplication $\diamond$ and contraction $\zeta$ satisfying (C1)-(C4), but without the requirement of a multiplicative unit. These form a category $\nuCSM$ whose morphisms are morphisms in $\GS$ that preserve the multiplication and contraction operations. Non-unital modular operads are the subject of \cref{sec: non-unital}.
\end{rmk}
%
%%\begin{ex}\label{ex:cyclic}
%%	(See also \cref{ex: general cyclic}.)
%%A \emph{cyclic operad} in the sense of \cite{DCH19}	is a graphical species  $S$ equipped with a \emph{unital} multiplication satisfying condition (C1), but with no contraction. As mentioned in \cref{ex: general cyclic}, if $S$ has palette $(\DDD \times \{\In, \Out\}, s)$ \warn{notation for this involution}, and 
%%\[ S(c_1, \dots...)  = \emptyset
%%\]
%%\warn{NOTATION}
%%unless..., then $S$ describes a $\DDD$ coloured operad. Say more.
%%
%%
%%%graphical species $S$ admitting a multiplication and contraction that satisfy conditions (C1)-(C4) of \cref{defn: Modular operad} but without a distinguished multiplicative unit.
%%\end{ex}
%
%
% 
%% \subsection{Examples of modular operads} 
% \label{subs: mo examples}
% 
% %\srnote{0203 GO THROUGH EXAMPLES}
 To provide context and motivation for the constructions that follow, the remainder of this section is devoted to examples. 
%	In the next subsection, review the abstract nerve theorem of Weber and motivate the graphical approach to modular operads.}
%\warn{2.6 - reconsider examples in light of reading.. So compact closed categories should be based on Ross's book and kelly's article. Others based on closer consideration. But this section is nice.}
\begin{ex}\label{ex: gk mod op}%\srnote{1703 - work on this example}
\label{cob} {\textbf{Getzler-Kapranov modular operads.}}
We may equip the monochrome graphical species $M : M_{X} = \N$ (for all $X$), with a unital multiplication $(+, 0 \in M_\two)$ induced by addition in $\N$:
\[ +\colon M_{\mm} \times M_\nn \to M_{\mathbf{m + n - 2}}, \ (g_m, g_n) \mapsto g_m+g_n  \text{ for } m,n \geq 1, \] and a contraction $t$ induced by the successor operation:
	\[ t\colon M_\nn \to M_{\mathbf{n - 2}} , \ g_n \mapsto g_n+1 \text{ for } n \geq 2.\]
%\warn{I don't like term multiplication since it is symmetric...}

Since a compact oriented surface with boundary is determined, up to homeomorphism, by its genus and number of boundary components, $(M, + , s)$ models gluing of topological surfaces along boundary components. Monochrome objects $(S, \gamma)$ of the slice category $\CSM\ov M$ describe a bigraded set $S^\gamma(g,n)$ with operations
\[ +^S \colon S^\gamma(g_1, n_1) \times S^\gamma(g_2, n_2) \to S^\gamma (g_1 + g_2, n_1 + n_2 -2)  \text { for } n_1, n_2 \geq 1, \]  \[
t^S\colon S^\gamma(g, n) \to S^\gamma(g+1, n-2) \text { for } n \geq 2,\]
and may encode (moduli spaces) of geometric structures on surfaces. For example, % $S^\gamma(g,n)$ could be the %compactified moduli space of compact genus $g$ Riemann surfaces with $n$ boundary components, that  %compactified moduli space of genus $g$ Riemann surfaces with $n$ boundary components, or, equivalently, the 
the Deligne-Mumford compactification $\overline {\mathcal M}_{g,n}$ of the moduli space of genus $g$ smooth algebraic curves with $n$ marked points, may be described, via Belyi's Theorem, in terms of the space of genus $g$ Riemann surfaces with $n$ nodes, and the spaces $\overline {\mathcal M}_n \defeq \coprod_{g \in \N} \overline {\mathcal M}_{g,n}$ form a monochrome modular operad. (See also \cite[Example~6.2]{GK98}.) %\srnote{1703 - check} %the space of conformal structures on a genus $g$ surface $\Gamma$ with $n$ boundary components.
%
%\warn{may then describe extra geometric structure on surfaces}. %\warn{Careful - need to add in colour. Restricting to monochrome modular oeprads...} may be viewed as describing extra structure \warn{what what what} on surfaces. 
%%%\srnote{Chose examples: Is this the same as the modular operads in \emph{operads revisited}?}
%
%
%A pair $(S, \gamma)$ of a monochrome species, and a morphism $\gamma \in (S, M)$ 

%%\srnote{question on stability.. is this correct?}
Getzler and Kapranov \cite{GK98} originally defined modular operads in terms of the restriction to the \emph{stable part} $M^{st} \subset M$ of the graphical species $M$.  An oriented surface $\Gamma$ is stable %\footnote{This corresponds to stability of algebraic curves. An algebraic curve is stable if its automorphism group is finite.} 
if and only if $2g + n -2 > 0$. So $M^{st}_\nn = M_\nn$ for $n >2$ but $M^{st}_\nul = \{ 2, 3, 4, \dots\}$ and $M^{st}_{\mathbf{1}} = M^{st}_{\two} = \{1, 2, 3, 4, \dots\}.$

In particular, since $0 \not \in M^{st}_{\two}$, %\warn{cylinder has infinite which automorphism group...See Birman etc.\. to work this out}, 
modular operads in the original sense of \cite{GK98} are non-unital. %(A number of examples are provided in \cite[Section~???]{GK98}.)


These ideas may be extended to many-coloured cases: for example, one can describe a 2-coloured modular operad for gluing surfaces along %-coloured stable modular operads arising from gluing of surfaces along 
{open and closed} subsets of their boundaries. (See, e.g.~\cite{Gia13}.)% describes 2-coloured modular operads 
%This is discussed in, e.g.\ \cite{Gia13}.
%Open-closed modular operads are considered in \cite{DJM15}, and a sequel paper \cite{DJP17} gives many of the same constructions, but this time in terms of open-closed 2-cobordism categories (see \cref{ex: compact closed} below).
%\srnote{deleted reference}
\end{ex}


\begin{ex}\label{ex: compact closed} {\textbf{Compact closed categories}}, introduced in \cite{Kel72}, are symmetric monoidal categories $(\CCat, \otimes, e)$ for which every object $c \in \CCat$ has a symmetric \textit{categorical dual} (see \cite{BG99,KL80}): there is an object $c^* \in \CCat$, and morphisms $\cap_c \colon e \to c^* \otimes c $ and $ \cup_c\colon c \otimes c^* \to e $ such that
	\[(\cup_c \otimes id_c) \circ(id_c \otimes \cap_c) = id_c = (\cap_{c^*}\otimes id_c)\circ (id_c \otimes \cup_{c^*}).\]
	
	%This implies also that they are equipped with a trace operation.\cite{SV92}
	Examples of compact closed categories include categories of finite dimensional vector spaces over a given field, or, more generally, finite dimensional projective modules over a commutative ring. Cobordism categories provide other important examples. %Other important compact closed categories include, for example, cobordism categories. % provide more examples. %\footnote{Though some treatments of cobordisms of manifolds exclude certain cases --for example by insisting that cobordisms have non-empty outgoing boundary -- to avoid technical difficulties, thereby breaking the compact closed structure. One of the hopes for this work is that it will provide insights into some of these cases.}, and they appear in many other contexts (see \cite{KL80} for a nice list from 1980 - of course much more work has been done since!).
	
%There is a canonical monadic adjunction $\CSM \leftrightarrows \comC$, where $\comC$	
The category of small compact closed categories contains an equivalent full subcategory $\comC$ of those categories $\CCat$ such that $c = c^{**}$ for all objects, and there is a canonical monadic adjunction $\CSM \leftrightarrows \comC$. 
	The right adjoint takes a small compact closed category $(\CCat, \otimes, e,*)$ with object set $\CCat_0$ to a $(\CCat_0, *)$-coloured modular operad $S^\CCat$ with coloured arities
\[  S^\CCat_{(c_1, \dots,c_m, d_1^*,\dots, d_n^*)} =\CCat(c_1 \otimes \dots \otimes c_m, d_1 \otimes \dots \otimes d_n)\] and the modular operad structure on $S^\CCat$ is induced by composition in $\CCat$ together with $\cup$ and $\cap$. The left adjoint $\CSM \to \comC$ is induced by the free monoid functor on palettes and arities. 

These observations underly the proof, in \cite{Ray21b}, of an `operadic' nerve theorem for compact closed categories in the style of \cref{s. nerve}. %This has a left adjoint.

\end{ex}

\begin{ex}%\srnote{0403 new example}%\textbf{Circuits in low dimensional topology.}
	\label{ex: circuits} \textbf{Circuit algebras} -- so named because of their resemblance to electronic circuits -- are a symmetric version of Jones's planar algebras, introduced to study finite-type invariants in low-dimensional topology \cite{BND17, DHR20}. 
	
	Objects of the category $\CO$ of \textit{circuit operads} \cite{Ray21a} are modular operads equipped, via a monadic adjunction $\CSM \leftrightarrows \CO$, with an extra `external product' operation. Circuit operads in a linear category $\E$ are precisely the circuit algebras in $\E$.
	
The adjunction between modular operads and compact closed categories in \cref{ex: compact closed} factors though the adjunction $\CSM \leftrightarrows \CO$. %as $\CSM \leftrightarrows \CO\leftrightarrows \comC$, 
Moreover, every compact closed category in $\comC$ is equivalent to the free compact closed category on a circuit operad. 
	

%	
%	\warn{Any small compact closed category $\CCat$ with $c^{**} = c$ for all $c$, is equivalent to a category $\CO^\times$ of modular operads equipped with an extra monoidal structure. These \textit{representable circuit operads} are closely related to circuit algebras studied in low dimensional topology \cite{BND17, DHR20}. This is discussed in \cite{Ray21a}. In \cite{Ray21b}, I prove a Weber style nerve theorem for circuit operads, via an iterated distributive law.}%(Details \cite{Ray20b,Ray20c}.)}
	
	This formal perspective on modular operads, circuit algebras, and compact closed categories leads to interesting questions in a number of directions. For example, we can study the analogous relationships if the definition of modular operads is relaxed by replacing the symmetric action with a braiding, or by considering higher dimensional versions. Related ideas are being explored by Dansco and Robertson in their work on algebraic and categorical structures in low-dimensional topology.
\end{ex}

\begin{ex}\label{ex: wheeled prop}
	\label{wheeled properads intro} {\textbf{Wheeled properads.}} 
		Wheeled properads have been studied extensively in \cite{HRY15} and \cite{JY15}. They describe the \textit{connected part} (c.f.~\cite[Introduction]{Val07}) of wheeled PROPs -- coloured PROPs with a contraction -- that have applications in geometry, deformation theory, and other areas \cite{Mer10, MMS09}. 
	
	The category $\mathsf{WP}$ of ($\Set$-valued) wheeled properads is canonically equivalent to the slice category $\CSM\ov Di$ of \textit{directed modular operads}. This is well-defined since the terminal directed graphical species $Di$ trivially admits the structure of a modular operad (see \cref{ex:direction}).%, the slice category $\CSM\ov Di$ of \textit{directed modular operads} is well-defined. It is canonically equivalent to the category of ($\Set$-valued) wheeled properads, that have been studied extensively in \cite{HRY15}, \cite{JY15}.  
	
An equivalence between wheeled PROPs in linear categories and directed circuit algebras is established in \cite{DHR20}. The equivalence between $\CSM \ov Di$ and $\mathsf{WP}$ is extended to an equivalence between wheeled PROPs and circuit operads in \cite{Ray21a}.
	
%	%\srnote{R 23. The simplest way to say something about wheeled properads is to state the equivalence and give references.}
	
	
	
	
\end{ex}

%%The final example of this section is of a quite different, somewhat silly, flavour, but it is of combinatorial interest. %interesting from a combinatorial point of view.
%%\begin{ex}\label{ex: free tree operad}
%%	
%%		Objects of the dendroidal category $\Omega$  (see \cite{MW07} and \cref{ex: dendroidal}) are the free operads $\Omega(\Tr)$ on symmetric rooted trees, and admit a description as wheeled properads (albeit with a trivially uninteresting contraction). This extends to a fully faithful embedding of $\Omega$ in $\CSM$. %embeds fully faithfully in $\CSM$. 
%%
%%	
%%	Let $E$ be the set of edges, and $V$ the set of vertices of a rooted tree $\Tr$. So, if $\Tr$ is the directed exceptional edge $(\downarrow)$, then $E$ is a singleton and $V $ is empty, and, if $\Tr$ is the rooted corolla $t_X$, then $ E \cong X \amalg \{r\}$, while $V $ is a singleton. %The \emph{leaves} of the tree $\Tr$ are those edges that are not the root of any subtree $\Tr[S] \subset \Tr$ with non-trivial vertex set. %%\srnote{too much information re leaves etc.\..?}
%%\begin{figure}[htb!]	
%%\[	
%%	\begin{tikzpicture}[scale = .9]
%%	
%%		\node at (12,2){(b)};
%%		\node at (14,0){
%%		\begin{tikzpicture}[scale = 0.4]
%%	%	\node at (0,0){\begin{tikzpicture}[scale = .4]
%%	\draw[black, dashed]
%%		(-1,0)--(.5, 1);
%%
%%		\draw[thick, cyan]
%%		(-1.5,-3)--(-1.5, -1)
%%		(-1.5, -1)--(-1,0)
%%		(-3.5,1)--(-1.5, -1);
%%		
%%		\filldraw [cyan]
%%		(-1.5, -1) circle (6pt);
%%
%%		
%%		\draw[thick, blue]
%%		(0,3)--(0,4.5)%not leaves or subtree
%%		
%%		
%%		%(-.5, -1)--(0,0)
%%		(.5, 1)--(1,2)
%%		(1,2)--(3,4)
%%		(1,2)--(-1,4)
%%		(3,4)--(3,5.5)%just subtree
%%				
%%		(-2,5)--(-0,3)
%%		(3,5.5)--(2,7)
%%		(3,5.5)--(4,7)% just leaves
%%		
%%		(3,4)--(1,6)
%%		(3,4)--(4.5,6)
%%		(3,4)--(6,6);% leaves and subtree
%%				
%%		\filldraw [blue]
%%		%(-.5, -1) circle (6pt)
%%		(0,3) circle (6pt)
%%		(0,4.5) circle (6pt)
%%		(3,5.5) circle (6pt)%just main tree
%%		(1,2) circle (6pt)
%%		(3,4) circle (6pt)
%%		;
%%		
%%	\end{tikzpicture}};
%%
%%	\node at (15.5,0){\large{$\longrightarrow$}};
%%	\node at (15.5,.3){\scriptsize{$\circ_{e_0}$}};
%%%	\draw [->](1,0)--(2,0);
%%
%%\node at (18,0){	\begin{tikzpicture}[scale = 0.4]
%%			
%%			\draw[thick]
%%		(0,-2)--(0,0)
%%		(0,3)--(0,4.5)%not leaves or subtree
%%		
%%		
%%		(0,0)--(1,2)
%%		(1,2)--(3,4)
%%		(1,2)--(-1,4)
%%		(3,4)--(3,5.5)%just subtree
%%		;
%%		\draw[thick]
%%		(-2,2)--(0,0)
%%		(-2,5)--(-0,3)
%%		(3,5.5)--(2,7)
%%		(3,5.5)--(4,7)% just leaves
%%		
%%		(3,4)--(1,6)
%%		(3,4)--(4.5,6)
%%		(3,4)--(6,6);% leaves and subtree
%%		
%%		\filldraw 
%%		(0,0) circle (6pt)
%%		(0,3) circle (6pt)
%%		(0,4.5) circle (6pt)
%%		(3,5.5) circle (6pt)%just main tree
%%		(1,2) circle (6pt)
%%		(3,4) circle (6pt)
%%		;
%%		
%%			\end{tikzpicture}
%%
%%};
%%		
%%	%	\end{tikzpicture}};
%%%\node at (-2.5,2){(a)};
%%%	\node at (0,0){
%%%		\begin{tikzpicture}[scale = 0.4]
%%%		
%%%		\draw[thick]
%%%	(0,-2)--(0,0)
%%%	(0,3)--(0,4.5)%not leaves or subtree
%%%	
%%%	
%%%	(0,0)--(1,2)
%%%	(1,2)--(3,4)
%%%	(1,2)--(-1,4)
%%%	(3,4)--(3,5.5)%just subtree
%%%	;
%%%	\draw[red, thick]
%%%	(-2,2)--(0,0)
%%%	(-2,5)--(-0,3)
%%%	(3,5.5)--(2,7)
%%%	(3,5.5)--(4,7)% just leaves
%%%	
%%%	(3,4)--(1,6)
%%%	(3,4)--(4.5,6)
%%%	(3,4)--(6,6);% leaves and subtree
%%%	
%%%	\filldraw 
%%%	(0,0) circle (6pt)
%%%	(0,3) circle (6pt)
%%%	(0,4.5) circle (6pt)
%%%	(3,5.5) circle (6pt)%just main tree
%%%	(1,2) circle (6pt)
%%%	(3,4) circle (6pt)
%%%	;
%%%	
%%%		\end{tikzpicture}};
%%	
%%	\node at (2.5,2){(a)};
%%	
%%	\node at (4.5,0){	\begin{tikzpicture}[scale = 0.4]
%%		
%%		\draw[thick, cyan]
%%%		(0,-2)--(0,0)
%%%		(0,3)--(0,4.5)%not leaves or subtree
%%%		
%%%		
%%		(1,0)--(1,2)
%%		(1,2)--(3,4);
%%		\node at (1.6,.8){\scriptsize{$e_0$}};
%%			\draw[thick,cyan]
%%		
%%		(1,2)--(-.5,3.5)
%%		(3,4)--(3,6)%just subtree
%%%		;
%%%		\draw[cyan, thick]
%%%		(-2,2)--(0,0)
%%%		(-2,5)--(-0,3)
%%%		(3,5.5)--(2,7)
%%%		(3,5.5)--(4,7)% just leaves
%%%		
%%		(3,4)--(1,6)
%%		(3,4)--(4.5,6)
%%		(3,4)--(6,6);% leaves and subtree
%%		
%%		\filldraw [cyan]
%%%		(0,0) circle (6pt)
%%%		(0,3) circle (6pt)
%%%		(0,4.5) circle (6pt)
%%%		(3,5.5) circle (6pt)%just main tree
%%		(1,2) circle (6pt)
%%		(3,4) circle (6pt)
%%		;
%%		
%%		\end{tikzpicture}};
%%	
%%	\node at (5.8,0){\large{$\longrightarrow$}};
%%	
%%	\node at (8.5, 0){	\begin{tikzpicture}[scale = 0.4]
%%		
%%		\draw[thick]
%%		(0,-2)--(0,0)
%%		(0,3)--(0,4.5)%not leaves or subtree
%%		
%%		(-2,2)--(0,0)
%%		(-2,5)--(-0,3)
%%		(3,5.5)--(2,7)
%%		(3,5.5)--(4,7)% just leaves
%%		;
%%		
%%		\draw[thick,cyan]
%%		(0,0)--(1,2)
%%		(1,2)--(3,4);
%%		\draw[thick, cyan]
%%		(1,2)--(0,3)
%%		(3,4)--(3,5.5)%just subtree
%%		
%%		(3,4)--(1,6)
%%		(3,4)--(4.5,6)
%%		(3,4)--(6,6);% leaves and subtree
%%		
%%		\filldraw 
%%		(0,0) circle (6pt)
%%		(0,3) circle (6pt)
%%		(0,4.5) circle (6pt)
%%		(3,5.5) circle (6pt);
%%\filldraw[cyan]
%%		(1,2) circle (6pt)
%%		(3,4) circle (6pt)
%%		;
%%		\node at (1.2, .8){\scriptsize{$e_0$}};
%%		
%%		\end{tikzpicture}};
%%	
%%	\end{tikzpicture}\]
%%	\label{fig: rooted trees}
%%	\caption{%(a) A rooted tree (with leaves in red), 
%%		(a) Subtree inclusion respects vertex valency. (b) Tree grafting along and inner edge.}
%%	\end{figure}
%%	
%%Let $E^\dagger \cong E$ be the formal involution of the set $E$ of edges of $\Tr$. Since $E$ is finite, a subset $E' \subset E$, is precisely an element $\underline e  = (e_x)_x\in E^X$ such that $e_x \neq e_y$ for distinct $x, y \in X$.
%%	The $(E \amalg E^\dagger, \dagger)$-coloured graphical species  $\Omega^{MO}(\Tr)$ is given by
%%	$\Omega^{MO}(\Tr)_{\nul } = \{*\}, $ and
%%	\[\Omega^{MO}(\Tr)_{\underline e, e_0^\dagger } = \left(
%%	\begin{array}{ll}
%%\{\Tr[S]\}& \Tr[S]\subset  \Tr \text{ is a subtree  with leaf set } \underline e \text{ and root } e_0,\\
%%\emptyset & \text{ otherwise,} 	
%%\end{array}\right.
%%	  \] where subtrees $\Tr[S]\subset \Tr$ are required to respect vertex valency.
%%	  
%%	 Grafting of $\Tr$ subtrees as in \cref{fig: rooted trees} (c) (\cite{}) describes a multiplication $\circ$ with unit $(\downarrow)$ on $\Omega^{MO}(\Tr)$ that coincides with the composition in $\Omega(\Tr)$.
%%	 	 
%%	 By definition, $\Omega^{MO}(\Tr)_{e, e^\dagger}  $ is the singleton set whose element $i_e: ((\downarrow) ) \to \Tr$ is the inclusion of the exceptional tree $(\downarrow)$ into the edge $e$ of $\Tr$, and, for all $e \in \underline e \subset E$, $\Omega^{MO}(\Tr)(\underline e, e^\dagger) = \emptyset$ unless $\underline e = \{e\}$. So, $\Omega^{MO}(\Tr)$ admits a completely uninteresting contraction that sends each exceptional subgraph $i_e : (\downarrow) \to  \Tr$, $e \in E$ to a point.
%%	 
%%	 Hence, the free operad $\Omega(\Tr)$ on a symmetric tree $\Tr$ describes, rather trivially, a modular operad. Indeed, there is a fully faithful embedding of $\Omega$ (and, and hence also of) into $\CSM$.
%%
%%\end{ex}
%
%
%


==> 1803Topology.tex <==
\section{The \'etale site of graphs}\label{sec: topology}

By \cref{ex: embedding fin}, there is a canonical embedding $\fisinv \hookrightarrow \Grbig$ whose image consists of the exceptional graph $(\shortmid)$, the corollas $\CX$, and the \'etale (locally bijective) morphisms between them. 

A composition of \'etale morphisms is clearly \'etale by \cref{def: locally inj sur}, and the category all graphs and \'etale morphisms (introduced in \cite[Section~3]{JK11}) will be denoted by $\Gret \subset \Grbig$, and $\Gr \subset \Gret$ is the full subcategory of connected graphs and \'etale morphisms. % is denoted by $\Gr$.

The goal of this section is to describe the categories $\Gr$ and $\Gret$ in detail, and establish a chain 
\[ \xymatrix{ \fisinv \ar@{^{(}->}[r] &\  \Gr \  \ar@{^{(}->}[r]& \GS}\]
	%\hookrightarrow \Gr \hookrightarrow \GS \] 
	of dense fully faithful embeddings as discussed in \cref{sec: Weber}. 

%\warn{ In particular,... sheaves ....this justifies the idea that etale maps are open maps..}

%\begin{rmk}\label{rmk: gret or gr}
%	In this section we will actually work in greater generality and consider the category $\Gret \subset \Grbig$ of \textit{all} graphs and \'etale morphisms, of which $\Gr$ is the full subcategory on the connected graphs. From \cref{subs. unpointed multiplication} onwards it will be assumed that all graphs are connected.
%\end{rmk}
The following is immediate from \cref{def: locally inj sur} and the universal property of pullbacks of sets:
\begin{prop}\label{etale}\label{etale condition}\label{2 out of 3}
	For morphisms $f,g$ in $\Grbig$, if any two of $f, g$ and $g \circ f$ are \'etale, then so is the third. A morphism $f \in \Grbig (\G, \G')$ is \emph{\'etale} if and only if the right-hand square in the defining diagram (\ref{morphism})
%	\begin{equation}\label{etale diagram}\xymatrix{
%		\G\ar[d]_f&&   E \ar@{<->}[rr]^-\tau\ar[d]_{f_E}&&E \ar[d]_{f_E}&& H \ar[ll]_s\ar[d]_{f_H} \ar[rr]^t&& V\ar[d]^{f_V}\\
%		\G'&&  E' \ar@{<->}[rr]_-{\tau'}&&E'&& H' \ar[ll]^{s'} \ar[rr]_{t'}&& V'}\end{equation}
	is a pullback of finite sets. 
	
	
\end{prop}
%\begin{proof}The first statement is immediate from the definition of \'etale morphisms as local bijections,  %Since bijections satisfy a two out of three property, so do local bijections and the first statement 
%	and the second statement follows from \cref{def: locally inj sur} and the universal property of pullbacks of sets. 
%\end{proof}

\srnote{1803 streamlined}
%By the following proposition, which follows directly from \cref{etale}, a graph morphism is \'etale precisely when it is a local bijection: % tells us that the \'etale morphisms are precisely the local bijections:%(See \cref{def: locally inj sur}.)% those that \emph{locally preserve (vertex) valency}.

%\begin{prop}\label{etale condition}\label{2 out of 3}
%	A morphism $ f \in \Grbig(\G, \G')$ is \'etale if and only if it is locally bijective. % for all $v \in V$, the restriction of $f$ to $\vH$ induces an isomorphism $\vH\xrightarrow{\cong}\sfrac{H'}{f(v)}$.
%%	, that is
%%	\[\vH \cong f_H(\vH)  \ \text{ and }  \ f_H(\vH) = \vH[f(v)].\] 
%Hence, for composable morphisms $f,g$ in $\Grbig$, if any two of $f, g$ and $g \circ f$ are \'etale, then so is the third.\end{prop}

\begin{ex}\label{ex: esv ese etale}
%A morphism $f\colon \mathcal S \to \G$ from a shrub $\mathcal S$ is trivially \'etale by definition. %In particular, morphisms from stick graphs are \'etale.
	
	For any graph $\G$ and all $v \in V(\G)$, the essential morphism $\esv\colon \Cv \to \G$ defined in \cref{ex: vertex examples} is \'etale.  Indeed, a morphism $f \in \Grbig(\G, \G')$ is \'etale if and only if $f$ induces an isomorphism $\Cv \cong \Cv[f(v)]$ for all $v \in V$.
	
	\end{ex}



%\begin{ex} Since 
%	In \cref{morphism ex1}, $f_a$ is not \'etale since the unique vertex $v$ of $\C_\two$ has valency $2$ whereas $ f_a(v) = v_1 $ has valency 3. The morphism $f_b$ is \'etale. 
%	
%	The canonical maps $\CX\rightarrow \mathcal M^{X,Y}_{x_0,y_0}\leftarrow \CX[Y]$ and $\CX \to \mathcal N^X_{x_0,y_0}$ in \cref{ex: locally injective MN} are not \'etale, whereas the canonical maps $\CX[X \amalg \{x_0\}] \rightarrow   \mathcal M^{X,Y}_{x_0,y_0}\leftarrow \CX[Y \amalg \{y_0\}]$ and $\CX[X \amalg \{x_0, y_0\}]\to N^{X}$ are \'etale. \end{ex}

\begin{ex}\label{wheels and lines} Though the graphs $\Lk$ and $\Wm$ are bivalent for all $k \geq 0$ and $m \geq 1$, the flattening morphism $q \colon \Wm[2k] \to \Lk[k+1]$ in \cref{ex: flattening} fails to be locally injective (or surjective) at $w_1$ and $w_k$, and is hence not \'etale. 
%	Recall the line and wheel graphs $\Lk$ and $\Wl$, introduced in Examples \ref{def Lk}, and \ref{wheels}.
	
%Morphism in $\Gret(\Lk, \Lk[n])$ (with $k, n \in \N$) are given by a choice of subgraphmay be thought of as an oriented inclusion of $\Lk $ in $\Lk[n]$:
For $k, n \in \N$, 
	\[\Gret(\Lk, \Lk[n]) \cong \left \{
	\begin{array}{ll}
	2(\mathbf{ n-k + 1})& n \geq k\\
\emptyset, & n <k.
	\end{array}
	 \right.\]
	
		A morphism $f \in \Gret(\Lk, \Wl[m])$, $m \geq 1$ is fixed by $f(1_{\Lk}) \in E(\Wl)$. Hence, \[\Gret(\Lk, \Wl[m]) \cong E(\Wl) \cong 2(\mm).\]
	
%	For $k >m$, $\Gr(\Lk, \Lk[k']) = \emptyset$ and, if $k \leq k'$, then $\Gr(\Lk, \Lk[k'])\cong 2(\mathbf{ k'-k})$. 

\'Etale morphisms between wheel graphs are surjective: For $l,m \geq 1$ 
	\[\Gret(\Wl[l], \Wl[m]) \cong \left \{
\begin{array}{ll}
2(\mathbf{m})& \text{ if }\frac{l}{m} = d \in \N\\
\emptyset, & \text{ otherwise.}
\end{array}
\right.\] If $m$ divides $l$, a morphism in $\Gret(\Wl[l], \Wl[m])$ is fixed by $w_1  = f(v_1) \in V(\Wl[m])$, and a choice $f(a_1) \in \vE[w_1]$ of `winding direction'. %$v_1 \in V(\Wl)$ and a choice of winding direction. So,
\end{ex}
\srnote{1803 - check these changes}


\subsection{Pullbacks and monomorphisms in $\Grbig$.}

By \cref{etale condition}, \'etale maps of graphs are local homeomorphisms and, as such, have similar properties to {open maps} of topological spaces. 

\begin{lem}\label{lem: Grbig admits pullbacks}\label{lem: Gret admits pullbacks}
	The graph categories $\Grbig$ and $\Gret$ admit pullbacks. Moreover, \'etale morphisms are preserved under pullbacks in $\Grbig$.
\end{lem}
\begin{proof}
	Recall that graphs are objects of the presheaf category $\GrShape$ of graph-like diagrams in $\fin$. 
	Let $\mathcal P = (\underline E, \underline H, \underline V, \underline s, \underline t, \underline \tau)$ be the pullback in $\GrShape$ of morphisms $f_1 \in \Grbig(\G_1, \G)$ and $f_2 \in \Grbig (\G_2,\G)$. Since pullbacks in $\GrShape$ are computed pointwise, $\underline \tau$ is a fixed-point free involution, and $\underline s$ is injective. So, $\mathcal P$ is a graph, and $\Grbig$ admits pullbacks.	
	
	%	By \cref{lem: Grbig admits pullbacks}, pullbacks of graph maps are graphs. 
	\'Etale morphisms pull back to \'etale morphisms since limits commute with limits. Hence, by symmetry, $\Gret$ admits pullbacks.
\end{proof}



\begin{defn}
	\label{defn: weak subgraph} A \textit{weak subgraph} $w\colon \G {\to} \G'$ is a morphism $w \in \Grbig(\G, \G')$ induced by inclusions $V \hookrightarrow V'$, and $H \hookrightarrow H'$, and such that disjoint components of $\G$ have disjoint images in $\G'$.
\end{defn}

\begin{ex}\label{ex: no orthogonal factorisation}%\warn{23.04-think where to place this.. }
	%Epi-mono factorisation of morphisms is, in general, not unique. For example, 
	Let $\W$ be the wheel graph with vertex $v \in V(\W)$. The essential morphism $ \esv\colon \Cv {\to} \W$ is both surjective and describes a weak subgraph. In general, for all $k \geq 1$, an \'etale morphism $\Lk \to \Wl[k]$ exhibits $\Lk$ as a weak subgraph of $\Wl[k]$ that is surjective and not injective on edges. % and Since $\C_{\two} \cong 
\end{ex}


\begin{defn}\label{defn: etale preimage}
	For any morphism $f \in \Grbig (\G, \G')$, not necessarily \'etale, and any weak subgraph $i\colon\H  \xrightarrow{}\G'$, the \emph{preimage $f^{-1}(\H) \subset \G$ of $\H$ under $f$} is defined as the pullback
	\[
	\xymatrix{
		f^{-1}(\H)  \ar[rr] \ar[d]&& \G\ar[d]^{f}\\
		\H \ar[rr]_-{i}&& \G'.	}\]
	
\end{defn}

In particular, by \cref{lem: Gret admits pullbacks}, the preimage of an \'etale subgraph is an \'etale subgraph. %\warn{check this statement}

\begin{ex}\label{ex: wheel preimage}	 (See also \cref{wheels and lines}.)
	Let $l, m$ and $d$ be positive natural numbers such that $l = dm$. By \cref{wheels and lines},  there exists an \'etale morphism $f \in \Gret (\Wl[l], \Wl[m])$. If $i\colon\Lk \hookrightarrow \Wl[m]$ is a weak \'etale subgraph (so $0 \leq k \leq m$), then the preimage $f^{-1}(\Lk) \hookrightarrow \Wl[m]$ is isomorphic to the disjoint union  $d \Lk$ of $d$ copies of $\Lk$.
	
\end{ex}

%


Any (possibly empty) graph $\H$ has the form $\H' \amalg \mathcal S$ where $\H'$ is a graph without stick components and $\mathcal S$ is a shrub. 

%A monomorphism $f \in \Grbig (\H, \G)$ satisfies the following three conditions\colon 
\begin{lem}\label{lem: weak mono}
	If $f \in \Grbig (\H, \G)$ is a monomorphism, then
		\begin{enumerate}[(i)]
				\item the images $f(\H')$ and $f(\mathcal S)$ are disjoint in $\H'$;
			\item the restriction of $f\colon \mathcal S \to \G$ is injective;
			\item $f$ is injective on $V(\H)$ and $H(\H)$ (but not necessarily on $E(\H))$.
		\end{enumerate}	
\end{lem}

\begin{proof}
Pairs of edges $e' \in E(\H')$ and $l \in E(\mathcal S)$ of $\H$ such that $ f(e') = f(l) \in E(\G)$ correspond to pairs of parallel morphisms $ch_{e'}, ch_{l}\colon (\shortmid) \to \H$ such that $ f\circ ch_l  = f \circ ch_ {e'}$. So monomorphisms in $\Grbig$ satisfy (i). A similar argument shows that conditions (ii) and (iii) are also necessary. 
\end{proof} %, so $f$ is not a monomorphism if $(i)$ does not hold. Conditions (ii) and (iii) are shown to be necessary by similar arguments.
%end{proof}

In \cref{prop: mono}, we see that the converse also holds. So, while epimorphisms in $\Grbig$ are pointwise surjections, monomorphisms in $\Grbig$ are not necessarily pointwise injective.

%The symbol `$  \rightarrowtail $' is used to specify graph morphisms satisfying the conditions of \cref{lem: weak mono}. 
\srnote{0403 notational change}
By \cref{all fE}, any morphism $f\colon \H {\to} \G$ that satisfies the conditions of \cref{lem: weak mono} is either injective on edges or, if not then there exist pairs of ports $e_1, e_2 \in E_0(\H)$ such that  
\begin{itemize}
	\item $\tau_\H e_1, \tau_\H e_2 \in s(H)$, and hence $ e_2 \neq \tau_\H e_1$, and 
	\item $\tau_\G f(e_2) = f(e_1) \in   {\EI '} (\G)$ form a $\tau_\G$-involutive pair of inner edges of $\G$.
\end{itemize} 
In this case we say that $f$ \textit{glues} pairs of ports of $\H$ in $\G$. 



\begin{prop}\label{prop: mono}
	Let  $f \in \Grbig (\H, \G)$ be a morphism. The following are equivalent:
	\begin{enumerate}
		\item $f$ is a monomorphism;
		\item $f$ satisfies the conditions of \cref{lem: weak mono};
		\item for every weak subgraph $i\colon \G' {\to} \G$ where $\G'$ has no inner edges, the induced morphism $f^{-1}(\G') \to \G'$ is a strong inclusion (injective on edges and vertices).
	\end{enumerate}
	
\end{prop}

\begin{proof}
	The implication $(1)\Rightarrow (2)$ follows from \cref{lem: weak mono}.
%	The proof that $f \in \Grbig((\H, \G)$ is a monomorphism implies conditions (ii) and (iii) proceeds along similar lines to the example showing that (i) is necessary given above.
%	If there are distinct vertices $v_1, v_2$ of $\H$ such that $f(v_1)  = f(v_2) = v \in V(\G)$, then there are parallel morphisms $i_{v_1}, i_{v_2}\colon \C_\nul \to \H$, with image $v_1$, respectively $v_2$ such that $f\circ i_{v_1} = f\circ i_{v_2}$. Similarly, if there are distinct $h_1 = (e_1, v_1), h_2 = (e_2, v_2) \in H(\H)$, such that $f(h_1) = f(h_2) = h \in H(\G)$ then $ch_{e_1}\neq ch_{e_2}\colon (\shortmid) \rightrightarrows \H$, but $ch_e =  f \circ ch_{e_1} =  f \circ ch_{e_2}\colon (\shortmid) \to \G$. So, if $f$ is not a weak injection, it is not a monomorphism.
	
For $(2)\Rightarrow (3)$, let $w\colon \G' {\to} \G$ be a weak subgraph such that $\G'$ has no inner edges. Then $f^{-1}(\G') \to \G'$ is a strong injection if $f \in \Grbig(\H, \G)$ satisfies (i)--(iii).	

For	$(3)\Rightarrow (1)$, let $f \in \Grbig (\H, G)$ and let $w\colon \G' {\to} \G$ be any morphism as in (3) so $f^{-1}(\G') \to \G'$ is a strong injection. Let $ g, h\colon \H' \rightrightarrows \H$ be parallel morphisms such that $ f \circ g = f \circ h$. Since $f^{-1}(\G')$ has no inner edges, neither does $(f \circ g)^{-1}(\G')  =  (f \circ h)^{-1}(\G') $ and the induced maps to $f^{-1}(\G')$ agree. By taking $w\colon \G' {\to} \G$ of the form $\C_\nul \xrightarrow{v} \G$ for all $v \in V$, or $\ese\colon (\shorte) {\to} \G$  for $\tilde e \in \tilde E$, we see immediately that $ g = h\colon \H' \to \H$, and hence $f $ is a monomorphism in $\Grbig$.
\end{proof}\srnote{0403 minor change to sentence.}

The following corollary is immediate from the definitions.
\begin{cor}\label{cor: mono covers etale}
	A morphism in $\Grbig$ that is both an epi- and a monomorphism, is \'etale.
\end{cor}



\begin{ex}\label{ex: M and N monos}
	For all finite sets $X$ and $Y$, the canonical \'etale morphisms $ \CX[X \amalg \{x_0\}] \amalg \CX[Y \amalg \{ y_0\}] \to \mathcal M^{X,Y}_{x_0,y_0}$ and $ \CX[X \amalg \{x_0, y_0\}] \to \mathcal N^X_{x_0,y_0}$ are surjective and not pointwise injective. But they are monomorphisms.
\end{ex}

\begin{rmk}\label{rmk: weak injections} 
Monomorphisms of Feynman graphs correspond to pointwise injections in the graphical formalism, outlined in \cref{ex: BM graphs}, of \cite{GK98, BM08} and others.

\end{rmk}


\subsection{Graph neighbourhoods and the essential category $\esG$.}

A  family of morphisms $\mathfrak U = \{f_i \in \Gret (\G_i , \G)\}_{i \in I} $ is \emph{jointly surjective} on $\G$ if $\G = \bigcup_{i \in I} im (f_i)$. %Since $\G$ is finite, we may assume that $I$ is finite. 
By \cref{lem: Gret admits pullbacks}, jointly surjective families of morphisms $\{f_i \in \Gret (\G_i , \G')\}_{i \in I} $, define the {covers at $\G$} for a canonical \emph{\'etale topology} {$J$} on $\Gret$. Sheaves for this topology are those presheaves $P\colon{\Gret}^\mathrm{op}\to \Set$ such that, for all graphs $\G$, and all covers $\mathfrak U = \{f_i \in \Gret (\G_i , \G)\}_{i \in I}$ at $\G$,
\[P(\G) \cong \mathrm{lim}_{f_i \in  \mathfrak U }P(\G_i).\]

\srnote{0503 removed pronouns} In fact, as will be shown in \cref{prop: GS sheaves}, sheaves for the \'etale site $(\Gret,J)$ are canonically equivalent to graphical species (\cref{defn: graphical species}). 

First, we establish more properties of \'etale morphisms. As usual, it is useful to draw on the analogy between \'etale morphisms of graphs and open maps of topological spaces for intuition.
%\warn{just call coverings etale coverings, and decide on notation ...}


\begin{defn}
	A \emph{neighbourhood} of a weak subgraph $w\colon \G' {\to} \G$ is a weak \'etale subgraph $u\colon \mathcal U {\to} \G$ such that $\tilde w\colon \G' {\to} \mathcal U$ is a weak subgraph and $w = u \circ \tilde w\colon \G' {\to} \mathcal U{\to} \G$.
	
	
	
	A neighbourhood $ (\mathcal U, u)$ of $ w\colon \G' {\to} \G$ is \emph{minimal} if every other neighbourhood $ (\mathcal U', u')$ of $ w\colon \G' {\to} \G$ is also a neighbourhood of $(\mathcal U, u)$. 
	
\end{defn}

Since vertices $v$ of $\G$ correspond to subgraphs $v\colon \C_\nul \to \G$,  and edges $e$ of $\G$ are in bijection with subgraphs $ch_e\colon (\shortmid) \hookrightarrow \G$, we may also refer to neighbourhoods of vertices and edges. Moreover, since $u\colon \mathcal U {\to} \G$ is a neighbourhood of $e \in E$ if and only if it is a neighbourhood of $\ese\colon (\shorte)\to \G$, there is no loss of generality in referring to neighbourhoods of $\tau$-orbits $\tilde e \in \tilde E$.


\srnote{0503 - changed stuff around}
%Recall from \cref{ex: first gluing example} that, for all finite sets $X$, the graph $\mathcal N_{x_0, y_0}^X$ is the colimit in $\Gret$ of the parallel morphisms $\ch_{x_0}, ch_{y_0} \circ \tau \colon (\shortmid) \to \CX[X \amalg \{x_0, y_0\}]$. More generally, for any graph $ \G$ with distinct ports $e_1, e_2 \in E_0$, there is a graph $\G_{e_1, e_2}$ that
%Let $\G$ be any graph with $\mathcal S (\EI)  = \coprod_{\tilde e \in \tilde \EI} (\shorte)$ the shrub on the inner edges of $ \G$. The poset of subsets of $\tilde \EI$ is isomorphic to the poset of subgraphs of $\mathcal S(\EI)$:
%\[ \tilde \EI \supset I\ \longleftrightarrow \ \I \defeq \coprod_{ \tilde e \in I } (\shorte) \subset \G.\]
%by $I \mapsto \I$ where 
%\[
%\I \defeq \coprod_{ \tilde e \in I } (\shorte) \subset \G.\]

Let $\mathcal S (\EI)  = \coprod_{\tilde e \in \tilde \EI} (\shorte)$ be the shrub on the inner edges of a graph $ \G$. Given any subgraph $\I \hookrightarrow \mathcal S({\EI})$, there is a graph $\G_{\widehat{\I}}$ and a canonical surjective weak subgraph $i_{\widehat{\I}}\colon\G_{\widehat{\I}}{\to} \G$: % by {`breaking the edges in $\I$'}\colon
\begin{equation}
\label{eq: covering inclusion}
\xymatrix{
	\G_{\widehat{\I}}\ar[d]_{i_{\widehat{\I}}}&&  {E \amalg (E(\I))^\dagger }\ar@{<->}[rr]^-{\tau_{/\I}}\ar@{->>}[d]&& {E \amalg (E(\I))^\dagger }\ar@{->>}[d]&E \ar@{_{(}->}[l]&& H \ar[ll]_-s\ar@{=}[d] \ar[rr]^t&& V\ar@{=}[d]\\
	\G&&  E \ar@{<->}[rr]_-{\tau}&&E&&& H \ar[lll]^{s} \ar[rr]_{t}&& V,}
\end{equation}
where 
\begin{itemize}
	\item $(E(\I))^\dagger$ is the formal involution $e \mapsto e^\dagger$ of the set $E(\I)$ of edges of $\I$ ,
	\item the involution $\tau_{/\I}$ on $E \amalg (E(\I))^\dagger$ is defined by
	\[ e \mapsto \left \{ \begin{array}{ll}
	\tau e, & e \in E \setminus  E(\I)\\
	e^\dagger, & e \in E(\I),
	\end{array} \right . \]
	\item the surjection $E \amalg (E(\I))^\dagger  \twoheadrightarrow  E$ is the identity on $E$ and $e^\dagger \mapsto \tau e$  on $(E(\I))^\dagger$.
\end{itemize} 
 So, $\G_{\widehat{\I}}$ has inner edges $\EI (\G_{\widehat{\I}}) = \EI \setminus  E(\I)$, and boundary $E_0(\G_{\widehat{\I}}) = E_0 \amalg (E(\I))^\dagger$.

Informally, $	\G_{\widehat{\I}}$ is the graph obtained from $\G$ by `breaking the edges' of $\I$, as in \cref{fig: graph covers}.

\begin{figure}
	\begin{tikzpicture}[scale = .3]


\draw[->] (-15,0)--(-11,0);

\node at (-25,0){\begin{tikzpicture}[scale = .25]
	
	\draw [thick]
		(-3,2).. controls (-2.5,1.5) and (-2.5,0.5).. (-3,0)
	(-3,0).. controls (-3.5,-1).. (-5,-1)
	(-5,3)..controls (-2,4) and (1,4) .. (3,3)
	
		(1,-4)..controls (2, -4) and (6,-2).. (5,2)
	
	;
	\filldraw[white] (-3,0) circle (25 pt)
	(-1,3.56) circle (35 pt)
		(4, -2) circle (35 pt);
	
	\draw[ thick] 	
	%cluster 1
	(-6,1).. controls (-6,2).. (-5,3)
	(-5,3).. controls (-4.5,3) and (-3.5,3).. (-3,2)
%	(-3,2).. controls (-2.5,1.5) and (-2.5,0.5).. (-3,0)
%	(-3,0).. controls (-3.5,-1).. (-5,-1)
	(-5,-1).. controls (-6,-0) .. (-6,1)
	(-5,-1)-- (-3,2)
	(-3,2)--(-6,1)
	(-6,1)..controls ( -7.5,1) and (-9, 0.5) ..(-11,0.5)
	%cluster 2
	(-1,-5)..controls (-0.5,-3.5) and ( 0.5, -3.5)..(1,-4)
	(-1,-5)..controls (-0.5,-5) and ( 0.5, -5)..(1,-4)
	(-1,-5) .. controls (-2.5,-5) and (-5, -4.5) ..(-6, -9)
	%cluster 3
	(4,1)--(5,2)
	(5,2)--(3,3)
	(3,3)--(4,1)
	(3,3).. controls (4,3.5) and (5,2.5)..(5,2)
	(3,3).. controls (3,4) and(4,6)  ..(8,6)
	%between clusters
%	(-5,3)..controls (-2,4) and (1,4) .. (3,3)
	(-3,2).. controls (1,-1.5) and (5,-1).. (5,2)
%	(1,-4)..controls (2, -4) and (6,-2).. (5,2)
	;
	
	\filldraw [black]	
	%cluster 1
	(-6,1) circle (8pt)
	(-5,3) circle (8pt)
	(-3,2) circle (8pt)
%	(-3,0) circle (8pt)
	(-5,-1) circle (8pt)
	%cluster 2			
	(1,-4) circle (8pt)
	(-1,-5) circle (8pt)
	%cluster 3			
	(4,1) circle (8pt)
	(5,2) circle (8pt)
	(3,3) circle (8pt);
	
%	\filldraw[white] (-3,0) circle (15pt);
	
	
	
	%\draw [ultra thick] (,0) to [out=87,in=150] (1,1) -- (.85,.15) -- (0,0);
	%\draw [ultra thick, fill=blue] 	(-7.5,0) ..controls ( -6,4) and (-2,6)..(0,6)
	(0,6 ) .. controls (2,6) and (7,4) ..(7,0)
	( 7,0) .. controls (7,-2) and (2,-8) ..(0,-8)--(0,0)--(-7.5,0);
	%\path [fill=blue] (4,0) to [out=87,in=150] (5,1) -- (4.85,.15) -- (4,0);
	\end{tikzpicture}};

\node at (-2,0){\begin{tikzpicture}[scale = .25]
	
	\draw [thick, red]
	(-3,2).. controls (-2.5,1.5) and (-2.5,0.5).. (-3,0)
	(-3,0).. controls (-3.5,-1).. (-5,-1)
	(-5,3)..controls (-2,4) and (1,4) .. (3,3)
	
	(1,-4)..controls (2, -4) and (6,-2).. (5,2)
	
	;
	
	
	\draw[ thick] 	
	%cluster 1
	(-6,1).. controls (-6,2).. (-5,3)
	(-5,3).. controls (-4.5,3) and (-3.5,3).. (-3,2)
	%	(-3,2).. controls (-2.5,1.5) and (-2.5,0.5).. (-3,0)
	%	(-3,0).. controls (-3.5,-1).. (-5,-1)
	(-5,-1).. controls (-6,-0) .. (-6,1)
	(-5,-1)-- (-3,2)
	(-3,2)--(-6,1)
	(-6,1)..controls ( -7.5,1) and (-9, 0.5) ..(-11,0.5)
	%cluster 2
	(-1,-5)..controls (-0.5,-3.5) and ( 0.5, -3.5)..(1,-4)
	(-1,-5)..controls (-0.5,-5) and ( 0.5, -5)..(1,-4)
	(-1,-5) .. controls (-2.5,-5) and (-5, -4.5) ..(-6, -9)
	%cluster 3
	(4,1)--(5,2)
	(5,2)--(3,3)
	(3,3)--(4,1)
	(3,3).. controls (4,3.5) and (5,2.5)..(5,2)
	(3,3).. controls (3,4) and(4,6)  ..(8,6)
	%between clusters
	%	(-5,3)..controls (-2,4) and (1,4) .. (3,3)
	(-3,2).. controls (1,-1.5) and (5,-1).. (5,2)
	%	(1,-4)..controls (2, -4) and (6,-2).. (5,2)
	;
	
	\filldraw [black]	
	%cluster 1
	(-6,1) circle (8pt)
	(-5,3) circle (8pt)
	(-3,2) circle (8pt)
	%	(-3,0) circle (8pt)
	(-5,-1) circle (8pt)
	%cluster 2			
	(1,-4) circle (8pt)
	(-1,-5) circle (8pt)
	%cluster 3			
	(4,1) circle (8pt)
	(5,2) circle (8pt)
	(3,3) circle (8pt);
	
	%	\filldraw[white] (-3,0) circle (15pt);
	
	
	
	%\draw [ultra thick] (,0) to [out=87,in=150] (1,1) -- (.85,.15) -- (0,0);
	%\draw [ultra thick, fill=blue] 	(-7.5,0) ..controls ( -6,4) and (-2,6)..(0,6)
	(0,6 ) .. controls (2,6) and (7,4) ..(7,0)
	( 7,0) .. controls (7,-2) and (2,-8) ..(0,-8)--(0,0)--(-7.5,0);
	%\path [fill=blue] (4,0) to [out=87,in=150] (5,1) -- (4.85,.15) -- (4,0);
	\end{tikzpicture}};
	
	

\end{tikzpicture}
\caption{ Graphs (left) $\G_{\widehat{\I}}$ and, (right) $\G$, with subgraph $\I$ indicated in red.}
\label{fig: graph covers}
\end{figure}

For each $\tilde e\in I$, the essential morphism $\ese\colon (\shorte) \hookrightarrow \G$ (\cref{ex: stick examples}) factors in two ways through $\G_{\widehat{\I}}$:
\begin{equation}\label{eq: parallel maps}
\xymatrix{ (\shorte) \ar@<4pt>[rrr]^{(e, \tau e) \mapsto (e, e^\dagger)}  \ar@<-4pt>[rrr]_{(e, \tau e) \mapsto ((\tau e)^\dagger, \tau e)}  &&&\G_{\widehat{\I}} \ar@{>->}[rr]^{i_{\widehat{\I}}}&& \G.  } \end{equation}
Hence there exist parallel morphisms $\I \rightrightarrows \G_{\widehat{\I}}$ such that the diagram
\begin{equation}\label{eq: general coequaliser}
\xymatrix{ \I \ar@<4pt>[rr]\ar@<-4pt>[rr]&&\G_{\widehat{\I}} \ar[rr]^{i_{\widehat{\I}}}&& \G  } \end{equation}
commutes, and, moreover, describes a coequaliser diagram in $\Grbig$. (Of course the choice of pairs of morphisms $\I \rightrightarrows \G_{\widehat{\I}}$ is not unique -- there are $2^{|I|}$ choices -- but it is unique up to isomorphism.)

For each $\I \subset S(\EI)$, the set of components of $\I \ \amalg  \ \G_{\widehat{\I}} $, together with the canonical monomorphisms to $\G$, defines an \'etale cover at $\G$. % $\mathfrak U_\I = \{(\mathcal U_j,u_j)\}_{j \in J}$ at $\G$, where each $u_j$ is the composition of the inclusion of the component $\mathcal U_j$ in $\I\amalg  \G_{\widehat{\I}} $ with the canonical morphism to $\G$.
\srnote{0503 - much shorter... does next paragraph still work?}

By definition, any surjective weak subgraph $\G' {\to} \G$ is of the form $(\G_{\widehat{\I}},i_{\widehat{\I}})$ for some $I \subset \tilde E$. So the poset of subgraphs of $\mathcal S(\EI)$ defines a poset structure on the collection $\{(\G_{\widehat{\I}}, i_{\widehat{\I}})\}_{\I \hookrightarrow \mathcal S(\EI)} \subset \Gret \ov \G$, for which the graph
%%the relation $i_{\widehat{\I}}\leq i_{/\I'}$ if and only if $i_{\widehat{\I}}$ factors through $i_{/\I'}$ equips 
% the collection $\{(\G_{\widehat{\I}}, i_{\widehat{\I}})\}_{\I \hookrightarrow \mathcal S(\EI)}$ of surjective weak subgraphs of $\G$ has a canonical poset structure, opposite to the poset of $\mathcal S(\EI)$ subgraphs. The graph
 $\G_{\widehat{\mathcal{S}(\EI)}}$ with no inner edges is initial. % obtained by breaking all inner edges of $\G$, is initial. %of surjective 
We have proved the following:
\begin{lem}\label{lem: minimal nbd}\label{cor: minimal nbd of v e}
A neighbourhood $(\mathcal U,u)$  of a weak subgraph $i  \in \Grbig(\G', \G)$ is minimal if and only if each component of $\mathcal U$ intersects non-trivally with $\G'$, and $\EI(\mathcal U) = \EI (\G')$.

For all vertices $v \in V$, and all edges $e \in E$, the essential (weak) subgraphs $\esv$ and $\ese$ describe minimal neighbourhoods of $v$ and $e$ respectively. % $\esv\colon \Cv {\to} \G$ is the minimal neighbourhood of $v$ and $\ese\colon (\shorte) {\to} \G$ is the minimal neighbourhood of $e$. %an edge $ e \in E$.

\end{lem}


In case $\G$ has no stick components, one readily checks that $\G_{\widehat{\mathcal{S}(\EI)}} = \coprod_{v \in V} \Cv.$ In particular, for any graph $\G$, there is a canonical choice of \textit{essential cover} $\mathfrak {Es}_\G $ of $\G$ by essential subgraphs. %\'etale subgraphs $\ese, \tilde e \in \tilde E$, $\esv, v \in V$ of $\G$. The essential category of $\G$ is the full subcategory of the slice category $\Gret \ov \G$ on the objects of $\mathfrak {Es}_\G $.

Note that a graph $\G$ describes a small category with object set $ \tilde E \amalg V$ and non-identity morphisms of the form $h = (e,v) \colon \tilde e \to v$. This is isomorphic to the full subcategory of $\Gret \ov \G$ generated by $\mathfrak {Es}_\G $.
\begin{defn}
	\label{def: essential}
	Let $\G$ be a graph. The \emph{essential category $\esG$ of $\G$} is the full subcategory of $\Gret \ov \G$ on the essential subgraphs
	\[ \ese\colon(\shorte){\to}  \G, \ \tilde e \in \tilde E, \text{ and } \esv\colon \Cv {\to} \G, \ v \in V.\]
	
\end{defn}

%Since $\esG$ has no non-trivial isomorphisms, non-identity morphisms in $\esG$ are of the form $\delta \colon \ese \to v$ described by morphisms
There is a canonical bijection between non-identity morphisms $\delta$ in $\esG$ and half-edges of $\G$ for if $h = (e, v) \in H$, then $ s(h) = e$ is the unique element in the intersection $ E(\shorte) \cap E( \Cv) \cap E$.  So, $\esh$ is the unique morphism in $ \Gret (\shorte, \Cv)$ above $\G$ that fixes $e$. For each $h = (e, v) \in H$, the corresponding morphism in $ \esG(\shorte, \Cv)$ is denoted by $\esh$.
\srnote{0503 - slight reordering to deal with notation}
%Since the objects of $\esG$ are indexed by $\tilde E \amalg V$, there are no other non-identity morphisms in $\esG$.

\begin{lem}\label{lem: essential cover}
	Each graph $\G$ is canonically the colimit of the forgetful functor $\esG \to \Gret$. 
	
	A presheaf $P \in \pr{\Gret}$ is a sheaf for the \'etale site $(\Gret, J)$ if and only if for all $\G$,
	\begin{equation}\label{eq: sheaf condition essential}
	P (\G) \cong \mathrm{lim}_{ (\C,b) \in \esG}P (\C).
	\end{equation}
\end{lem}

\begin{proof}
If $e \in E_0$ is a port of $\G$, then there is, at most, one non-trivial morphism $\esh = \esh[(\tau e,v)]$ in $\esG$ with domain $\shorte$. In this case, $\esh $ has the form $ \esh[(\tau e,v)]$ for some $v \in V$, and $\Cv$ is the colimit of the diagram $\shorte \xrightarrow{\esh} \Cv$. The first statement follows from (\ref{eq: parallel maps}) and (\ref{eq: general coequaliser}). 

The second statement is immediate since, by \cref{lem: minimal nbd}, the essential cover $\mathfrak {Es}_\G $ refines every \'etale cover $\mathfrak U $ of $\G$.
\end{proof}

%he essential cover $\mathfrak {Es}_\G $ refines every \'etale cover $\mathfrak U $ of $\G$,, the essential category $\esG$ refines $\mathfrak U $. Therefore, 
%a presheaf $P \in \pr{\Gret}$ is a sheaf for the \'etale topology on $\Gret$ if and only if for all $\G$,
%\begin{equation}\label{eq: sheaf condition essential}
%P (\G) = \mathrm{lim}_{ (\C,b) \in \esG}P (\C).
%\end{equation}


\cref{lem: essential cover} will be used to prove in \cref{prop: GS sheaves} that the category $\sh{\Gret,J}$ of \'etale sheaves on $\Gret$ is equivalent to the category $\GS$ of graphical species. 

Before doing so, it is worth collecting together a number or results on (\'etale) graph morphisms that will be useful in the rest of this work. 

%To this end, the following subsection is devoted to results about \'etale surjections and a number of useful corollaries of these. 

\subsection{Boundary-preserving \'etale morphisms}%{\'Etale covering maps}
\label{subs. covering}\srnote{Some changes made to this section as a result of changes to the section on paths and cycles}
	
	In general, morphisms $ f \in \Gret(\G', \G)$ do not satisfy $f(E'_0) \subset E_0$. Those that do are componentwise surjective \textit{graphical covering maps} in the sense of \cref{graph cover} below. In particular, monomorphisms $f \in \Gret(\G', \G)$ such that $f(E'_0) = E_0$ are componentwise isomorphisms. 
	

	\begin{prop}\label{graph cover}
		For any \'etale morphism $ f \in \Gret(\G', \G) $, $f (E'_0) \subset E_0$ if and only if there exists an \'etale covering $\mathfrak U = \{ \mathcal U_i, u_i\}_{i \in I}$ of $\G$, such that, for all $i$, $f^{-1}(\mathcal U_i)$ is isomorphic to a disjoint union of $ k(\mathcal U_i, f) \in \N$ copies of $ \mathcal U_i$. 
		
		In this case, $ k(\mathcal U_i,f) = k_f \in \N$  is constant  on connected components of $\G$. 
	\end{prop}

	
	\begin{proof}
	If $u\colon \mathcal U {\to} \G$ is a weak \'etale subgraph for which there is a $k \in \N$ such that $f^{-1}(\mathcal U) \cong k (\mathcal U)$, then also $f^{-1}(\mathcal V) \cong k \mathcal V$ for all weak subgraphs $\mathcal V {\to} \mathcal U$. So, we may assume, without loss of generality, that $\mathfrak U = \mathfrak{Es}_\G$ is the essential covering of $\G$. 
		
	Observe first that, when $f(E'_0) \not \subset E_0$, there exists a $v \in V$ and $e' \in E'_0$ such that $f(e')  \in \vE$. Hence $(\shorte[e'])$ is a connected component of  $ f^{-1}(\Cv)$.%\hookrightarrow \G'$.
		

%		let $(\mathcal U, u)$ be a neighbourhood of $\G$, and consider its preimage $f^{-1}(\mathcal U)$ in $\Gret$.
%	
%	So, 
		For the converse, let $(\mathcal U, u) = (\Cv, \esv)$ for some $v \in V$. Since $f$ is \'etale, $\Cv \cong \Cv[v']$ by \cref{2 out of 3} for all $v' \in V'$ such that $f(v') = v$. The weak \'etale subgraph $\coprod_{ v'\colon f(v') = v}\Cv {\to} \G'$ factors through $f^{-1}(\Cv)\to \G'$ by the universal property of pullbacks. Hence,
	\[ f^{-1}(\Cv) \cong \left (\coprod_{v'\colon f(v') = v} \Cv[v'] \right ) \amalg \mathcal S, \ \text{ where } \mathcal S %\cong \coprod_{i \in I} (\shortmid) 
	\text{ is a shrub. } \]
	
	By construction, a connected component of $\mathcal S$ must be of the form $\ese[e']\colon (\shorte[e']) \to \G'$  for some port $e'$ of $\G'$ satisfying $f(e') = e \in \vE$. But $f(E'_0) \subset E_0$ by assumption, so there is no such port and $\mathcal S = \oslash$ is the empty graph.
	
	 It is immediate that $f^{-1}(\shorte) \cong \coprod_{e' \in E', f(e') = e } (\shorte[e'])$ for all $e \in E$, so $k((\shorte),f) = |f^{-1}(e)| \in \N$. 
%	We prove that $ \mathcal S $ is empty. By construction, a component of $\mathcal S$ corresponds to a neighbourhood of $\G'$ of the form $(\shorte[e']) $ for some port $e' \in E_0'$ such that $f(e') = e \in \vE$. Otherwise, if $e' \in E'$ is not a port, then $(\shorte) \hookrightarrow \Cv[t'(e')]\in f^{-1}(\Cv)$. But, $f(E'_0) \subset E_0$ by assumption so there is no such $e'$ and $\mathcal S = \oslash$ is the empty graph.
	
Hence, the first statement of the proposition is proved.

By condition (3) of \cref{conn 1}, it is sufficient to verify the second part of the proposition componentwise on $\G$. Therefore, we may assume, without loss of generality, that $\G$ is connected. 

Let $f \in \Gret (\G' , \G)$ satisfy $f(E'_0) \subset E_0$. 

If $\G \cong (\shortmid)$ is a stick, there is nothing to prove. Otherwise, the following diagram commutes for all $v \in V$:
	\[
\xymatrix{
	\coprod_{e'\in f^{-1}(e)}(\shorte) \ar[rr] ^- {\coprod_{h' \in f^{-1}(h)} \esh[h']} \ar[d] && \coprod_{v' \in f^{-1}(v)} \Cv \ar[rr] ^- {\coprod_{h} \esv} \ar[d]&& \G' \ar[d]_f
	\\
	(\shorte[\tilde e]) \ar[rr]_-{\esh[h]} && \Cv[v] \ar[rr]_-{\esv[v]}&& \G.}\]

The first part of the proof implies that both squares are pullbacks. In particular, if $ f^{-1} (\Cv)$ is isomorphic to $k_v = k(\Cv, \esv)$ copies of $\Cv$ then $f^{-1}(\shorte) \cong k_v (\shorte) $ for all $e \in \vE$. Hence $\Cv \mapsto k_v$ extends to a functor $K $ from $ \esG$ to the discrete category $\N$. Since $\G$ is connected, $K$ must be constant. 
	\end{proof}

\begin{defn}\label{pp}
	A morphism $ f \in \Gret (\G', \G)$ that restricts to an isomorphism $f_{E_0}\colon E_0 \xrightarrow \cong E'_0$ is called \emph{boundary-preserving}. 
\end{defn}
The following is an immediate corollary of \cref{graph cover}.
\begin{cor}
	\label{cor: coverings}\label{pp iso}
If $\G$ is connected, and $\G'$ is non-empty, then any \'etale morphism $f \in \Gret(\G', \G)$ such that $f(E'_0)\subset E_0$, is surjective. If $ \G'$ is also connected and $E'_0 $ is non-empty, then $f $ is boundary-preserving if and only if it is an isomorphism.


\end{cor}

	\begin{rmk}
		The condition that $ E'_0$ is non-empty is necessary in the statement of \cref{pp iso}. For example, for any $ m > 1$, each of the two \'etale morphisms $\Wl \to \W$ (see \cref{wheels and lines}) is trivially boundary-preserving, but certainly not an isomorphism. 
		
	\end{rmk}


 Recall from \cref{def Lk} that the line graph $\Lk$ has totally ordered edge set $E(\Lk) = (l_j)_{j = 0}^{2k+1}$ with ports $l_0 = 1_{\Lk}$ and $l_{2k+1} = 2_{\Lk}$. For each vertex $w_i \in V(\Lk)$, $ \vE[w_i ]= \{ l_{2i-1}, l_{2i}\}$. %So, $ \tau(2_{\Lk}) = \tau l_{2k+1} = l_{2k}$ (and $\tau 1_{\Lk} = \tau l_0 = l_1$) in $E(\Lk)$.
 
	\begin{prop}\label{bivalent graphs}
		Let $ \G$ be a connected graph with only bivalent vertices. Then $ \G  = \Lk$ or $\G = \Wl$ for some $k \geq 0$ or $m \geq 1$.
	\end{prop}
	
	\begin{proof} \srnote{0103 small changes to proof}
Since $\G$ is bivalent, every monomorphism $\Lk {\to} \G$ from a line graph is \'etale, for all $k \in \N$.
			
		The result holds trivially if $\G \cong \Lk[0]$ is a stick graph. 
			
		Otherwise, if $V = V_2$ is non-empty, then, for each $v \in V$, a choice of isomorphism $\Lk[1] \xrightarrow {\cong } \Cv$ describes a monomorphism $\Lk[1] {\to} \G$.  Since $\G$ is finite, there is a maximum $ M \geq 1$ such that there exists a monomorphism $f\colon \Lk[M] {\to} \G$. 
		
			
				Let $f \in \Gr(\Lk[M], \G)$ be such a map. 	By \cref{prop: mono}, $f$ is either injective on edges, %in which case $f(E_0(\Lk[M])) \subset E_0$, 
				or $f(2_{\Lk[M]}) = \tau f(1_{\Lk[M]}) \subset \EI$. % so $E_0 = \emptyset$ if not.
%				
%			We show first that, if $f$ is injective on edges, then it satisfies $f(E_0(\Lk[M])\subset E_0$: %Since $f$ is injective on edges, it maps the ports $l_0, l_{2M}$
%			
		Let $e_1 =  f(1_{\Lk[M]}), $ and 
			$e_2 =	f(2_{\Lk[M]})$. For $j = 1,2$, if $e_j $ is not a port of $\G$, then $e_j \in \vE$ for some vertex $v \in V_2$. If $f$ is injective on edges then $v$ is not in the image of $f$. But, since $v$ is bivalent, this means that we $f$ factors through monomorphisms $\Lk[M] {\to} \Lk[M+1] {\to} \G$, thereby contradicting maximality of $ M$. So $e_j \in E_0$ for $j = 1, 2$. Hence $f$ is boundary-preserving, and $\G \cong \Lk[M]$ by \cref{cor: coverings}.
	
			Otherwise, if $f$ is not injective on edges then it must be the case that $f(l_0) = f(l_{2M})$, in which case $f$ factors as $ \Lk[M] \to \Wl[M] \to \G$. Since $f$ is an \'etale monomorphism, the second map $\Wl[M] \to \G$ is \'etale, monomorphic and boundary-preserving. Hence, by \cref{cor: coverings}, $\G \cong \Wl[M]$. 
	\end{proof}

\begin{ex}
	\label{covering wheels}(See also Examples \ref{wheels and lines} and \ref{ex: wheel preimage}.)
%	For $m \geq 1$, let $\Wl$ be the wheel graph with $m \geq 1$ vertices. 
	By \cref{bivalent graphs}, if there is a weak \'etale subgraph $w\colon \G {\to} \W$, then $ \G \cong \Wl$ or $\G \cong \Lk$ for some $0 \leq k \leq m$.
	
\end{ex}

\'Etale morphisms of simply connected graphs are easy to describe since they are either (strict) subgraph inclusions or isomorphisms. (This is why the combinatorics of cyclic operads are much simpler than those of modular operads.)  %The extra complexity of the combinatorics of modular operads, compared with cyclic operads is explained by the following corollaries that imply that \'etale morphisms of simply connected graphs are either subgraph inclusions or isomorphisms. 
\cref{prop: dag prop} gives analogous results for directed acyclic graphs (\cref{def: DAG}).% from whence it follows that the combinatorics of props \cite{} and properads \cite{} are also simpler than those of modular operads. (See also \cite{Koc16}.)

\begin{cor}
	\label{cor:simp conn etale}
	If $\G$ is simply connected, and $ \Gret (\G', \G)$ is non-empty, then $\G'$ is simply connected. In particular, any monomorphism of simply connected graphs is a pointwise injection.
\end{cor}

\begin{proof}
	Let $\G, \G'$ be graphs and $f\colon\G'\to \G$ an \'etale morphism. If $\G'$ admits an injective cycle $ c\colon \Wl\to \G'$, then $f \circ c\colon \Wl \to \G$ is locally injective. Hence $f \circ c$ factors as $\Wl \to \Wl[l] \hookrightarrow \G$ where $l$ divides $m$, and $\Wl[l] \hookrightarrow \G$ is injective. So $ \G$ admits a non-trivial cycle.
\end{proof}\srnote{Anything about locally injective cycle -> injective cycle...? in previous section}

\begin{cor}	\label{cor:simp conn iso}\srnote{0103 some changes here}
		Let $\G$ be simply connected and $\G'$ be connected. Any \'etale morphism $f\colon \G' \to \G$ is pointwise injective. 
			In particular, an \'etale morphism $f\colon \G' \to \G$ is boundary preserving %  satisfies  $f(E'_0 ) \subset E_0$ 
		if and only if it is an isomorphism.
	
%	
%	Any \'etale morphism $f$ from a connected graph $\G'$  to a simply connectedis pointwise injective. 
%	
%	Let $\G$ be simply connected and $\G'$ be connected. An \'etale morphism $f\colon \G' \to \G$  satisfies  $f(E'_0 ) \subset E_0$ if and only if $f$ an isomorphism.
\end{cor}

\begin{proof}
	
If $\G', \G$ are connected graphs such that there exists an \'etale morphism $f  \colon \G' \to \G$ and either $\G$ or $\G'$ is isomorphic to the isolated vertex $\C_\nul$, then so is the other, and $f$ is isomorphic to the identity. Therefore, we may assume that both $\G$ and $\G'$ have non-trivial edge set.

Since $\G'$ is connected, for any pair $e'_1$ and $e'_2$ of distinct edges of $\G'$,there is, by \cref{lem: injective path}, an injective path $p \in \Grbig (\Lk, \G')$ connecting $e'_1$ and $e'_2$, and such that $p(1_{\Lk}) \in \{e'_1, \tau' e'_1\}$ and $p(2_{\Lk}) \in \{e'_2, \tau e'_2\}$. 

	If $f\colon \G' \to \G$ is \'etale, then, since such a path $p$ is injective, $f \circ p\colon \Lk \to \G$ is locally injective. 
	
	If $f$ is not injective then there are distinct edges $e'_1$ and $e'_2$ of $\G'$ such that $f(e'_1) = f(e'_2)$. Since $\G'$ is connected, there is, by \cref{lem: injective path}, an injective path $p \in \Grbig (\Lk, \G')$ connecting $e'_1$ and $e'_2$, and such that $p(1_{\Lk}) \in \{e'_1, \tau' e'_1\}$ and $p(2_{\Lk}) \in \{e'_2, \tau e'_2\}$. Moreover, if $f\colon \G' \to \G$ is \'etale, then, since $p$ is injective, $f \circ p\colon \Lk \to \G$ is locally injective. Then $f(e'_1) = f(e'_2)$ implies that $f \circ p$ factors as $\Lk \to \Wl[m] \hookrightarrow \G$ where $m$ divides $k$ and $\Wl[m] \hookrightarrow \G$ is injective. In other words, $ \G$ admits a non-trivial cycle.
	
	Therefore, if $\G$ is simply connected then any \'etale morphism $f \colon \G' \to \G$ from a connected graph $\G'$ is pointwise injective. 
	
	In particular, if $f$ is boundary-preserving, then it is an isomorphism by \cref{graph cover}. The result follows since isomorphisms clearly preserve boundary. %, it suffices to show that $k(f) = 1$.% \warn{notation}. 
%	The result is clear if $\G'  $ (and hence $\G$) is an isolated vertex. Otherwise, for any pair $e'_1$ and $e'_2$ of distinct edges of $\G'$, if $\G'$ is connected, then by \cref{lem: injective path}, there is an injective path
%	%So, assume that $E' = E(G')$ is non-empty, $\G'$ is connected, and $f \in \Gret(\G', \G)$ satisfies $ f(E'_0) \subset E_0$. Let $e_1, e_2$ be distinct edges in $E'$. Since $\G'$ is path connected, there is a path 
%	$p \in \Grbig (\Lk, \G')$ connecting $e'_1$ and $e'_2$ in $\G'$. We may further assume that $p$ is minimal in the sense that $p(1_{\Lk}) \in \{e'_1, \tau' e'_1\}$ and $p(2_{\Lk}) \in \{e'_2, \tau e'_2\}$.%\shorte[e_1]  = p(\shorte[l_0]) $ and $\shorte[e_2] = p (\shorte[l_{2k+1}])$ where $E_0(\Lk) = \{l_0, l_{2k+1}\}$ is the boundary of $\Lk$. \warn{careful-standardise notation for edges of $\Lk$. see proof below}
%
%	If $f\colon \G' \to \G$ is \'etale, then, since such a path $p$ is injective, $f \circ p\colon \Lk \to \G$ is locally injective. So, if 	$f(e'_1) = f(e'_2)$, then $f \circ p$ factors as $\Lk \to \Wl[m] \hookrightarrow \G$ where $m$ divides $k$ and $\Wl[m] \hookrightarrow \G$ is injective, in which case $ \G$ admits a non-trivial cycle.
%	
%	So, if $\G$ is connected then $k = 1$ and $f$ is an isomorphism by \cref{pp iso}.
\end{proof}
\srnote{0103 check references to proof 'lemmas' in this section}



	

\subsection{\'Etale sheaves on $\Gret$}\label{subs. sheaves}
The category $\GS$ of graphical species (\cref{defn: graphical species}) is equivalent to the category of sheaves for the canonical \'etale topology $J$ on $\Gret$ (and its restriction to $\Gr$) induced by jointly surjective collections \{$u_i\colon \mathcal U_i \to \G\}_{i \in I}$ of \'etale morphisms. % that are jointly surjective on their codomain $\G$. 


Recall that a graphical species $S$ is a presheaf on the category $\fisinv$ and that $\Phi\colon \fisinv \hookrightarrow \Gret$ is a full subcategory under the maps $\S \to (\shortmid)$ and $X \to \CX$. It is easy to check that a connected graph with two or more vertices has inner edges. Therefore:

\begin{lem}\label{lem: essential image elementary}
	The essential image of $\fisinv$ in $\Gret$ is the full subcategory $\el$ of connected graphs with no inner edges.
\end{lem}

The equivalence $\sh{\Gret,J}\simeq \GS$ will follow from:
\begin{lem}
	\label{lem: fisinv dense}\label{equiv}
	The inclusion $\Phi\colon \fisinv \hookrightarrow \Gret$ is dense. Hence the functor $\yet\colon \Gret \to \GS$, 
	$\G \longmapsto ( X \mapsto \Gret(\CX, \G))$, as well as its restriction to $\Gr$, is fully faithful.
\end{lem}

\begin{proof}
	\label{essentially surjective}
	
By \cref{lem: essential cover}, it suffices to show that $\esG$ is a skeleton for $\el \ov \G$. 
		
	The essential category $\esG$ is skeletal by definition. For any graph $\C \in \el $, each \'etale morphism $b: \C \to \G$ factors uniquely as an isomorphism in $\el$ followed by some $\iota$ in $\esG$. Hence the inclusion is essentially surjective on objects. It is full, and therefore also an equivalence, by definition of $\esG$ (\cref{def: essential}).
\end{proof}

The category of elements $\elG[S]$ of a graphical species $S$ was defined in \cref{elS}.

\begin{rmk}
	\label{el}
	By an application of the Yoneda lemma, the category $\elG[\yet\G]$ of $\el$-elements is canonically isomorphic to the slice category $\elG \defeq \fisinv \ov \G$, and I will write $\elG$ for both. Since $\Gret$ is a full subcategory of $\GS$ under $\yet$, I will henceforth write $\G$ rather than $\yet \G $ where there is no risk of confusion.
\end{rmk}

\begin{prop}\label{prop: GS sheaves}
	There is a canonical equivalence of categories
	$\sh{\Gret,J}  \simeq \GS$. 
	\end{prop}

\begin{proof}
	This is straightforward from the definitions. More precisely, the fully faithful inclusion $\Phi\colon \fisinv \to \Gret$ induces an \emph{essential geometric morphism} (e.g.\ by \cite[Section~VII.2]{MM94}) between the presheaf categories $\pr{\fisinv}$ and $\pr{\Gret}$. So, the pullback $
	\Phi^* \colon \pr{\Gr} \to \pr{\fisinv}$ %, \ P \longmapsto \ (\C \mapsto P (\Phi \  \C) ) , \ \C \in ob (\el)\] 
	 has fully faithful right and left adjoints $\Phi_* \vdash \Phi^* \vdash \Phi_!$ (by \cite[Section~VII.4]{MM94}),
	and % that are fully faithful since $\Phi\colon\el \hookrightarrow \Gr$ is \cite[pages~377 and 378]{MM94}.
	 	\begin{equation}\label{right adjoint}\Phi_*\colon \pr{\fisinv} \to \pr{\Gr}, \quad S \longmapsto (\G \mapsto \mathrm{lim}_{(\C,b) \in \elG} S(\C)). \end{equation} 
	 	Hence, a presheaf $P$ on $ \Gret$ satisfies $\Phi_* \Phi^* (P)  \cong P$ if and only if $P(\G) \cong \mathrm{lim}_{(\C,b) \in \elG} S(\C)) $ for all graphs $\G$, in which case $P$ is a sheaf, by Lemmas \ref{lem: essential cover} and \ref{equiv}.
	 	Then,
	 	\[P(\G) \cong \pr{\Gret}(y \G, P)  \cong \pr {\Gret}(y \G, \Phi_* \Phi^* (P)) \cong \GS(\yet \G, P), \] where $y: \Gret \to \pr{\Gret}$ denotes the Yoneda embedding, and so $ Y = \Phi^* y$.
	 	\end{proof}%\srnote{remove?}
%by \cref{equiv}, 
I will use the same notation to denote a graphical species $S$ and the corresponding sheaf on $(\Gret, J)$. So, for any graph $\G$,
\[ S(\G) \defeq \mathrm{lim}_{{(\C,b) \in \elG}}S(\C).\] 

As an immediate consequence of the proposition:
\begin{cor}
	The restriction of the \'etale topology $J$ to $\Gr$ induces an equivalence
$ \sh{\Gr, J}\simeq \GS$.
\end{cor}


%(Refer to \cref{rmk: elements of presheaf} for a discussion of element categories.)
\srnote{comment on elements deleted}
Recall \cref{defn: general element} of elements of a presheaf.
\begin{defn}\label{S-graph} 
Let $S$ be a graphical species, viewed as a sheaf on $\Gret$. The category $\Gret(S)$ of \emph{$S$-structured graphs} is defined as $\Gret(S) \defeq \mathsf{el}_{\Gret}(S)$.

%element category $\Gret(S) \defeq (Z_{\Gret}\ov S_{\Gret})^\mathrm{op}.$ %\int_{\Gret}S$. 
	Given a graph $\G $, $S(\G)$ is called the set of \emph{$S$-structures on $\G$} .
	
	%The category $\Gr(S) \defeq (Z_{\Gr}\ov S_{\Gr})^\mathrm{op}$ of {connected} $S$-structured graphs is 
	The full subcategory of $\Gret(S)$ with objects $(\G, \alpha)$ such that $\G$ is connected is denoted by $\Gr(S)\defeq  \mathsf{el}_{\Gr}(S)$.
\end{defn} 

\begin{rmk}\srnote{0503 - double check}
	By the Yoneda lemma, $S(\G)\cong \GS(Y\G, S)$ canonically, so $S(\G)$ is isomorphic to the set of objects of $\Gret(S)$ of the form $(\G, \alpha)$. The same notation $\alpha$ (or $(\G, \alpha)$) will be used for an object of $\Gret(S)$ and the corresponding morphism in $  \GS(\G, S)$.
\end{rmk}

%
\subsection{Directed graphs}\label{subs ex: Directed graphs} 
By way of example, and to provide extra context, this section ends with a discussion of directed graphs. In particular, we see that, if $Di$ is the terminal directed graphical species defined in \cref{ex:direction}, then $\Gret(Di)$ is precisely the category of directed graphs and \'etale morphisms used in \cite{Koc16} to prove a Weber style nerve theorem for properads. 

For any graph $\G$, a $Di$-structure $ \xi\in Di(\G)$ is precisely a partition $E = E_{\In} \amalg E_{\Out}$, where $e \in E_{\In}$ if and only if $\tau e \in E_{\Out}$. So $\tau$ induces bijections $E_{\In} \cong \widetilde E \cong E_{\Out}$. % $\tau\colon E_{\In}\overset{\cong}{\leftrightarrow} E_{\Out}$. 
% An \emph{orientation on a graph $\G$} is a $Di$-structure $ \xi\in Di(\G)$. Hence $\xi$ induces a partition $E = E_{\In} \amalg E_{\Out}$, where $ e \in E_{\In} \Leftrightarrow \tau e \in E_{\Out}$ and hence $\tau\colon E_{\In}\overset{\cong}{\leftrightarrow} E_{\Out}$. 

 So, an object $ (\G,\xi)$ of $\Gr(Di)$ -- called an \textit{orientation on $\G$} -- is given by a diagram of finite sets
 \begin{equation}\label{Directed graph}
 \xymatrix{
 	\widetilde E&& H_{\In} \ar[ll]_-{\widetilde {s_{\In}}} \ar[rr]^-{t_\In} && V && H_{\Out} \ar[ll]_-{t_\Out}\ar[rr]^-{\widetilde {s_{\Out}}}&& \widetilde E},\end{equation}
%\[
%\xymatrix{
%	E_{\In} \ar@/^2.0pc/[rrrrrrrr]^-{\tau}&& H_{\In} \ar[ll]_-{s_\In} \ar[rr]^-{t_\In} && V && H_{\Out} \ar[ll]_-{t_\Out}\ar[rr]^-{s_\Out}&& E_{\Out}\ar@/_2.0pc/[llllllll]},\]
	where the maps $\widetilde {s_\In}, \widetilde {s_\Out}$, and $t_\In, t_\Out$ denote the appropriate (quotients of) restrictions of $s\colon H \to E$, respectively $t\colon H \to V$.
%	Since $ E_{\In} \cong E_{\Out} \cong \widetilde E$ canonically, this is just a diagram
%	\begin{equation}\label{Directed graph}
%	\xymatrix{
%		\widetilde E&& H_{\In} \ar[ll]_-{s_\In} \ar[rr]^-{t_\In} && V && H_{\Out} \ar[ll]_-{t_\Out}\ar[rr]^-{s_\Out}&& \widetilde E},\end{equation}
%	where $s$ is the obvious composition $ H \xrightarrow {s} E \twoheadrightarrow \widetilde E$ of $s$ with the quotient $q\colonE \twoheadrightarrow \widetilde E$.
	Then morphisms in $ \Gret(Di)$ are quadruples of finite set maps making the obvious diagrams commute, and such that the outer left and right squares are pullbacks. This is the definition of the % $\Gret(Di)$ describes the % This  precisely % $\Gret(Di)$ is the %full subcategory of \emph{connected} directed graphs in the 
	 category of directed graphs and \'etale morphisms in \cite[Section~1.5]{Koc16}.
	
\begin{ex}\label{ex: directed lines and wheels}
	
The line graphs $\Lk$ with $E(\Lk) = \{l_i\}_{i = 0}^{2k+1}$ and wheel graphs $\Wl$ with $E(\Wl) = \{a_j\}_{j = 0}^{2m-1}$ admit a distinguished choice of orientation $\theta_{\Lk} \in Di(\Lk)$, $\theta_{\Wl} \in Di(\Wl)$, given by
%Let $\xi_{\Lk}$ be the orientation on the line graph $\Lk$ given by
	\[\theta_{\Lk}\colon E(\Lk) \to \{ \In,  \Out\}, \ l_{2i +1} \mapsto \In  \text{ and } l_{2i} \mapsto \Out \text{ for } 0 \leq i \leq k,\] 
		\[\theta_{\Lk}\colon E(\Lk) \to \{ \In,  \Out\}, \ a_{2j-1} \mapsto \In  \text{ and } e_{2j} \mapsto \Out \text{ for } 1\leq j\leq m,\] 
	A morphism $\gamma\colon (\Lk, \theta_{\Lk}) \to (\G,\xi)$ in $\Gret(Di)$ is a \emph{directed path of length $k$ in $ (\G, \xi)$}, and a \emph{directed cycle of length $m$ in $(\G, \xi)$} is a morphism $ \rho\colon (\Wl,\theta_{\Wl})\to (\G, \xi)$ in $\Gret(Di)$.  
	
	Directed paths and cycles are induced by locally injective morphisms of undirected graphs. So, if a directed graph $(\G, \xi)$ admits a directed cycle, then the underlying graph $\G$ admits a non-trivial cycle (\cref{cycle}).
\end{ex}

\begin{defn}\label{def: DAG}
	A \emph{directed acyclic graph (DAG)} is a directed graph $(\G, \xi)$ without directed cycles. In other words,  $\Gret(Di)\left((\Wl, \theta_{\Wl}), (\G, \xi)\right) = \emptyset$ for all $m \geq 1$.
\end{defn}

There are directed versions of Corollaries \ref{cor:simp conn etale} and \ref{cor:simp conn iso}:

\begin{prop}\label{prop: dag prop}

For all morphisms $ f \in  \Gret (Di)\left((\G', \xi'), (\G, \xi)\right)$ between connected DAGs, the underlying morphism $f \in \Gret(\G', \G)$ is a monomorphism. Moreover, if $(\G, \xi)$ is a DAG and the set $ \Gret (Di)\left((\G', \xi'), (\G, \xi)\right)$ is non-empty, then $(\G',\xi')$ is a DAG. Hence morphisms to DAGs in $\Gret(Di)$ are monomorphisms.
\end{prop}

In particular, the combinatorics of properads, are much simpler than those of wheeled properads or modular operads. 

The proof of \cref{prop: dag prop} follows from the analogous results for undirected graphs (Corollaries \ref{cor:simp conn etale} and \ref{cor:simp conn iso}), and (\ref{Directed graph}). Since it is not necessary for what follows, I leave it as an exercise to the interested reader. 

%\warn{\begin{rmk}
%	Free MO on DAG..???
%\end{rmk}
%}

==> 2503intro.tex <==
\section*{Introduction}


Modular operads, introduced in \cite{GK98} to study moduli spaces of Riemann surfaces, are a
``{`higher genus' analogue of operads \dots in which graphs replace trees in the definition.}'' {\cite[Abstract]{GK98}.
	
	
	
	Roughly speaking, modular operads are $\N$-graded objects $P = \{P(n)\}_{n \in \N}$ that, alongside an operadic {multiplication} (or {composition}) $\circ\colon P(n) \times P(m) \to P({m+n -2})$ for $m,n \geq 1$, admit a {contraction} operation $\zeta \colon P(n) \to P(n-2)$, $n \geq 2$. For example, we may multiply two oriented surfaces by gluing them along chosen boundary components, or contract a single surface by gluing together two distinct boundary components as in \cref{fig. gluing}.
	\begin{figure}[htb!]
		\includegraphics[width=.9\textwidth]{gluing_surfaces.png}
		\caption{Gluing (multiplication) and self-gluing (contraction) of surfaces along boundary components. Moduli of geometric structures -- such as Riemann surfaces -- provide many examples of modular operads.}\label{fig. gluing}
	\end{figure}
\srnote{0315 slight change to caption}
\srnote{0315 R1}
	
	%\warn{wheeled properads in fixed point theory, compact closed categories and roles of duality..}
 % In my PhD thesis \cite{Ray18}, I used `CSM' to refer to modular operads with multiplicative units, and reserved `modular operad' for those without.} 
	%As will be made precise in \cref{sec: definitions}, Examples \ref{ex:direction} and \ref{ex: gk mod op}, modular operads in the original sense of \cite{GK98} describe undirected systems. 	
	\srnote{2403}This work considers a notion of modular operads originally due to Joyal and Kock \cite{JK11},%, in which every colour has an involutive dual.
	\footnote{Joyal and Kock used the term {`compact symmetric multicategories (CSMs)'} in \cite{JK11} to refer to what are here called `modular operads'. Indeed, I adopted this terminology in a previous version of this paper and in \cite{Ray18}.}%Joyal and Kock's definition 
	that incorporates a broad compass of related structures, including modular operads in the orignal sense of \cite{GK98} and their coloured counterparts \cite{Gia13}. Under this general definition, wheeled properads \cite{HRY15, JY15} -- a version of properads \cite{Val07} equipped with a contraction operation -- are `directed' modular operads (this is made precise in \cref{sec: definitions}, Examples \ref{ex:direction} and \ref{ex: gk mod op}). %  as well as directed modular operads, or `wheeled properads' \cite{HRY15, JY15} (see also \cref{ex: wheeled prop}). 
	More generally, compact closed categories \cite{KL80} %-- monoidal categories in which every object has a symmetric dual-- 
	also provide examples of modular operads \cite{Ray21b, Ray21c} (see \cref{ex: compact closed}). These are closely related to circuit algebras that are used in the study of finite-type knot invariants \cite{BND17, DHR20} (see \cref{ex: circuits}). As such, modular operads have applications across a range of disciplines.\srnote{0403 - replaced virtual tangles with finite-type knot invariants...}
	
	However, their combinatorics are complex. In modular operads equipped with a multiplicative unit, contracting this unit leads to an exceptional `loop', that can obstruct the proof of general results. This paper undertakes a detailed investigation into the graphical combinatorics of modular operads, and provides a new approach to understanding such loops.
	
	
	
	%The combinatorics of modular operads are known to be complex. In modular operads equipped with a multiplicative unit, contracting the unit seems to result in creates particularly difficult challenges, usually described in terms of `exceptional' or `degenerate' loops. The goal of this paper is to explain and solve this \textit{problem of loops}.
	
	%This work the combinatorics of modular operads.  understanding the combinatorics of modular operads with a multiplicative unit.
	%The combinatorics of modular operads are governed by undirected graphs that admit cycles. They are 
	
	
	In \cite{JK11}, which forms the inspiration for this work, Joyal and Kock construct modular operads as algebras for an endofunctor (\cref{rmk: pointed endo}) on a category $\GS$ of coloured collections called `graphical species'.  %equipped with an involutive action. 
	Their machinery is significant in its simplicity. It relies only on minimal data and basic categorical constructions, that lend it considerable formal and expressive power.
	
	%However, the combinatorics of modern operads are complex. This is due to the presence of a contraction operation which means that modular operads are governed by graphs that admit cycles, which has presented particular challenges for understanding the combinatorics of modular operads with a multiplicative unit. % Particularly when the multiplication is required to be unital, the combinatorics have not been well understood.%Particularly when the multiplication is required to be unital, they are not well understood. 
	
	
	However, the presence of exceptional loops means that their modular operad endofunctor %defined in \cite{JK11} 
	does not extend to a monad %(\cref{sec: Weber}) 
	on $\GS$. As a consequence, it does not lead to a precise description of the relationship between modular operads and their graphical combinatorics. (See \cref{degenerate} for technical details.)%\footnote{Sections \ref{degenerate}, \ref{s. nerve}, and \cref{comment on JK HRY} provide more information on the main theorem in \cite[Section~6]{JK11}, and its restatement and proof, by other means, in {\cite[Theorem~4.1]{HRY19b}}.}
	
	This paper contains proofs of the following statements that first appeared in \cite{JK11}, and were proved in my PhD thesis \cite{Ray18} (where my methods were similar, though slightly less general, than those presented here):
	
	\srnote{23Feb labelling of theorems - ASK}
	\begin{thmx}%{Monad Existence}
		[Monad existence \cref{CSM monad DT}]%, \cref{s. Unital}]
		\label{thm: main intro}
		The category $\CSM$ of modular operads is isomorphic to the Eilenberg-Moore category of algebras for a monad $\OOO$ on the category $\GS$ of graphical species.
	\end{thmx}
	In particular, $\OOO$ is the \textit{algebraically free monad} \cite{Kel80} on the endofunctor of \cite{JK11}. 
	The \textit{nerve theorem} \cref{thm: nerve intro}, characterises modular operads in terms of a presheaves on a category of graphs.
	
%	Recall that a subcategory $\DCat \hookrightarrow \CCat$ induces a nerve functor $\DCat \to \ps{\CCat}$ f
%	The nerve theorem characterises modular operads in terms of presheaves on a category $\Klgr$ of graphs such that $P \colon \Klgr^{\mathrm{op}} \to \Set$ is the nerve of a modular operad if and only if, for all graphs $\G \in \Klgr$, 
	\begin{thmx}[Nerve \cref{nerve theorem}]
		\label{thm: nerve intro}
		The category $\CSM$ has a full subcategory $\Klgr$ whose objects are graphs. 
		The induced functor $N$ from $\CSM$ to the category $\pr{\Klgr}$ of presheaves on $\Klgr$ is fully faithful. Moreover, there is a canonical (forgetful) functor $j_!\pr{\Klgr} \to \GS$ such that the essential image of $N$ consists of precisely those functors $P \colon \Klgr^{\mathrm{op}} \to \Set$ that satisfy the so-called `Segal condition': $P$ is in the essential image of $N$ if $P$ is completely determined by the graphical species $j_!(P)$. %are completely determined by their image under $jthat satisfy a certain sheaf condition, or `Segal condition', stated in terms of $\GS$. % {Segal condition}.% in the sense of \cite[Lemma~3.6]{BMW12}, 
	\end{thmx}

\srnote{\warn{ASK about new statement 2403} .} %such that, for all graphs $\G \in \Klgr$, $P(\G)$ is completely determined
	
	
	An obvious motivation for establishing such results is provided by the study of weak (up-to-homotopy), or $(\infty, 1)$-modular operads, by weakening the Segal condition of \cref{thm: nerve intro}. % (\cref{nerve theorem}). 
	A number of potential applications of such structures are discussed in the introduction to \cite{HRY19a}. To this end, %Indeed, motivated by applications of $(\infty, 1)$-modular operads, 
	Hackney, Robertson and Yau have also recently proved versions of these theorems, by different methods, and used them to obtain a model of $(\infty,1)$-modular operads that are characterised in terms of a weak Segal condition \cite{HRY19a, HRY19b}. %.motivated by applications of $(\infty, 1)$-modular operads, \cite{HRY, HRY} have also recently proved versions these theorems.
	

	The aim of this work is to prove Theorems \ref{thm: main intro} and \ref{thm: nerve intro} in the manner proposed by \cite{JK11} -- using the abstract machinery,  introduced by Weber \cite{Web07,BMW12}, for establishing nerve theorems  -- and to use these proofs as a route to a full understanding of the underlying combinatorics, and the contraction of multiplicative units in particular. As will be explained in Sections \ref{sec: Weber} and \ref{s. nerve}, this places strict requirements on the relationship between the modular operad monad $\OOO$ and the graphical category $\Klgr$. In fact, to apply Weber's nerve machinery, the category $\Klgr$ must -- in a sense that will be made precise in \cref{sec: Weber} -- be obtained naturally from the definition of $\OOO$. % Precisely, the construction uses the abstract nerve machinery introduced by Weber \cite{Web07,BMW12},  
	 \srnote{Check this change against reviewer's comment. I didn't provide a reference just before the theorem, and instead reqorte the text afterwards} 
%	The aim of this work is to prove Theorems \ref{thm: main intro} and \ref{thm: nerve intro} by methods closely based on those of \cite{JK11}, and to use these proofs as a route to fully understanding the underlying combinatorics, and the contraction of multiplicative units in particular. \srnote{here something about Weber methods...} 
	
	
	Neither the construction of the monad $\OOO$ for modular operads, nor the proof of \cref{thm: nerve intro} is entirely straightforward. First, the method of \cite{JK11}, which is closely related to analogous constructions for operads (see Examples \ref{ex: operad endo} and \ref{ex: operad units}, c.f.~\cite{HRY15,Koc16, MMS09,MW07}) does not lead to a well-defined monad. Second, as a consequence of the contracted units, \srnote{"as a consequence of"} %as will be shown in \cref{s. nerve}, 
	the desired monad, once obtained, does not satisfy the conditions for applying the machinery of \cite{BMW12}. %the abstract nerve machinery introduced by Weber \cite{Web07,BMW12}. 
	To prove the theorems, it is therefore necessary to break the problem into smaller pieces, %dissect the problem into its constituent components, 
	thereby rendering the graphical combinatorics of modular operads completely explicit.
	
	Since the obstruction to obtaining a monad in %extending the modular operad endofunctor of 
	\cite{JK11} arises from the combination of the modular operadic contraction operation and the multiplicative units (see \cref{degenerate}), the approach of this work is to first treat these structures separately -- via a monad $\TT $ %= (T, \mu^\TT, \eta^\TT)$ 
	on $ \GS$ whose algebras are non-unital modular operads, and a monad $\DD $ %= (D, \mu^\DD, \eta^\DD)$
	on $\GS$ that adjoins distinguished `unit' elements --  and then combine them, using the theory of distributive laws \cite{Bec69}.
	
	\cref{thm: main intro} is then a corollary of:
	\begin{thmx}[\cref{monads distribute} {\&} \cref{CSM monad DT}]\label{thm: composite intro}
		There is a distributive law $\lambda$ of $ \TT$ over $\DD$ such that the resulting composite monad $\DD\TT$ on $\GS$ is precisely the modular operad monad $\OOO$ of \cref{thm: main intro}.
	\end{thmx}
	The graphical category $\Klgr$, used to define the modular operadic nerve, arises canonically via the unique fully faithful--bijective on objects factorisation of a functor used in the construction of $\OOO$. Therefore, if the monad $\OOO$ satisfies certain formal conditions -- if it `has aritities' (see \cite{BMW12}) -- \cref{thm: nerve intro} follows from \cite[Section~1]{BMW12}. %In this case the monad is said to `have arities'. \srnote{brackets deleted} %\cref{sec: Weber}, and \cite[Sections~1~\&~2]{BMW12}.))
	
	Though these conditions are not satisfied by $\OOO$ on $\GS$, the distributive law in \cref{thm: composite intro} implies that there is a monad $\TTp$, on the category $\GSp$ of $\DD$-algebras, whose algebras are modular operads. Moreover, \cref{thm: nerve intro} follows from: % It is then sufficient to show that the Weber machinery can be applied to this new monad $\TTp$.%provides us with an another approach. By the classical theory of distributive laws \cite{Bec69}, there is a monad $\TTp$ on the % there is a monad $ \TTp  = (U_*F_*, \mu^{\TTp},\eta^{\TTp})$ defined on the 
	%Eilenberg Moore category $\GSp$ of $\DD$-algebras, whose algebras are also modular operads. Then the nerve theorem \ref{thm: nerve intro} follows easily from
	
	\begin{lemx}[\cref{connected}]\label{prop: arities intro}
		The monad $\TTp$ on $\GSp$ has arities, and hence satisfies the conditions of 
		\cite[Theorem~1.10]{BMW12}.%\footnote{This was also proved in my PhD thesis \cite{Ray18}.}
	\end{lemx}
	%In this case $\TTp$ is said to `have arities'. (See \cref{sec: Weber}, and \cite[Sections~1~\&~2]{BMW12}.)
	
	I conclude this introduction by briefly mentioning three (related) benefits of this abstract approach.
	
	In the first place, the results obtained by this method provide a clear overview of how modular operads fit into the wider framework of operadic structures, and how other general results may be modified to this setting. For example, by \cref{prop: arities intro}, $\TTp$ and $\Klgr$ satisfy the Assumptions 7.9 of \cite{CH15}, which leads to a suitable notion of weak modular operad via the following corollary:
	
	\begin{corx}[\cref{cor: weak}]\label{cor: model}
		There is a model structure on the category of presheaves in simplicial sets on $\Klgr$. The fibrant objects are precisely those presheaves that satisfy a weak Segal condition.
	\end{corx}
	
	% Marcy Robertson and I are comparing this model structure with the model structure for weak modular operads in \cite{HRY19a}, and exploring whether $\Klgr$ itself admits a generalised Reedy structure.
	%
	
	Second, since this work makes the combinatorics of modular operads -- including the tricky bits -- completely explicit, it provides a clear road map for working with and extending the theory. 
	
	One fruitful direction for extending this work is to use iterated distributive laws \cite{Che11} to generalise constructions presented here. In \cite{Ray21a}, I use an iterated distributive law to construct a category of {modular operads with product} (\textit{circuit operads}) -- closely related to small compact closed categories -- as algebras for a composite monad on $\GS$. Once again the distributive laws play an important role in describing the corresponding nerve. Iterated distributive laws may also be used to construct higher modular operads. Using methods similar to \cite[Section~3]{Che11}, it is possible to obtain an appropriate notion of $n$-modular operad for $n \geq 0$. This can be used to give an undirected description of {extended cobordism categories}. 
	
	Finally, in many cases, the complexities of the combinatorics of contractions can provide deep insights into the structures they are intended to model. In current work, also together with L.\ Bonatto, S.\ Chettih, A.\ Linton, M.\ Robertson, N.\ Wahl, I am using these ideas to explore the contraction of spheres to points in the compactification of moduli spaces of algebraic curves.%\warn{conformal structures on surfaces}..
	
	
	%This work falls into three parts. 
	\medspace
	
	
	
	%\subsection{Acknowledgements} 
	{This work owes its existence to the ideas of A. Joyal and J. Kock and I thank Joachim for taking time to speak with me about it. P. Hackney, M. Robertson and D. Yau's work has been an invaluable resource. Conversations with Marcy have been particularly helpful. I gratefully acknowledge the anonymous reviewer whose insights have not only improved the paper, but also increased my appreciation of the mathematics.\srnote{1503 unsure about anything humble}
		
		This article builds on my PhD research at the University of Aberdeen, UK and funded by the EPFL, Switzerland, and I thank my supervisors R. Levi and K. Hess. 
		Thanks to the members of the Centre for Australian Category Theory at Macquarie University for providing the ideal mathematical home for these results to mature, and to R. Garner and J. Power in particular, for their reading of this work. 
		\srnote{1503 - small changes ast sentence}
		\subsection*{Overview of the paper}
		The opening two sections provide context and background for the rest of the work. An axiomatic definition of modular operads is given in \cref{sec: definitions}. 
		%The first section provides an axiomatic definition of modular operads. It begins with a discussion of graphical species. These are presheaves on a category $\fisinv$, that describe the structure on which the modular operadic multiplication and contraction operations may be defined. 
\cref{sec: Weber} is a brief review of Weber's abstract nerve theory, that provides a framework for the later sections. Both these introductory sections include a number of examples to motivate the constructions that follow. %, and in particular, the discussion of graph categories that follows in Sections \ref{s. graphs} and \ref{sec: topology}.
		
		%The second part, comprising Sections \ref{s. graphs} -- \ref{sec: non-unital}, establishes the graphical and functorial machinery for studying the combinatorics of modular operads. In Sections \ref{sec: definitions} and \ref{sec: Weber},
		The (Feynman) graphs of \cite{JK11} are introduced and discussed in detail in \cref{s. graphs}. \cref{sec: topology} focuses on \'etale morphisms of graphs. The construction of the monad $ \TT$ for {non-unital modular operads} is given in \cref{a free monad}. 
		
	%Sections \ref{degenerate} and \ref{s. Unital} deal with the problem of contracting multiplicative units. 
		
		% Before diving into the construction of unital modular operads in \cref{s. Unital}, we pause for a moment in In  we %provide some context and motivation by looking 
		% look in detail at 
		\cref{degenerate} acts as a short intermezzo in which the appearance of exceptional loops in the theory, and why they are problematic in the construction of \cite{JK11}, is explained. %and the essence of why loops are problematic for defining the modular operad monad is revealed (see, in particular, the discussion around equation (\ref{eq: isos don't respect colimt}) and after \cref{rmk: HRY solution}). %Points to note in this section are:
%		\begin{itemize}
%			\item Remarks \ref{rmk: standard solution} and \ref{rmk: HRY solution} refer to other approaches in the literature to the issue of loops. As far as I am aware, the graphical construction presented in this paper is unique in that it \textit{does not} incorporate some version of the exceptional loop into the graphical calculus, in order to model contractions of units. (\cref{rmk: construction unique}.)
%			\item The essence of why loops are problematic for defining the modular operad monad is revealed in the discussion around equation (\ref{eq: isos don't respect colimt}) and after \cref{rmk: HRY solution}: the monad multiplication should be defined in terms of colimit constructions that are defined \textit{on the nose} by a colimit construction, but these are not invariant under isomorphisms that define the monad endofunctor.% that do not respect certain objects, defined \textit{on the nose} by a colimit construction. 
%			\srnote{1503 - tricky} %colimits, that must be defined on the nose. %There appears to be an arrow in the wrong direction.
%		\end{itemize}
		%\cref{s. Unital} is the longest and most important section of the work, and contains the construction of the monad $\OOO$. % for modular operads happens in \cref{s. Unital} most of the new contributions
		The construction of the monad $\OOO$ for modular operads happens in \cref{s. Unital}. This is the longest and most important section of the work, and contains most of the new contributions. 
		
		Though considerable background is needed to understand the details of Sections \ref{degenerate} and \ref{s. Unital}, I note a couple of key points here, as a guide to the reader:
		
		\begin{itemize}
				\item Remarks \ref{rmk: standard solution} and \ref{rmk: HRY solution} refer to other approaches in the literature to the issue of loops. As far as I am aware, the graphical construction presented in this paper is unique in that it \textit{does not} incorporate some version of the exceptional loop into the graphical calculus, in order to model contractions of units. (\cref{rmk: construction unique}.)
			\item 
			
		In \cref{pointed graphical species}, we see that to obtain a graphical description of modular operads, we need -- by  \cref{defn: Modular operad} of modular operads -- to add extra morphisms to the category of graphs.
		This leads to a description of the contracted units in terms of a double cone of graphs (\cref{fig: contracting units}(b)). 
		
	Whereas in the approaches described in Remarks \ref{rmk: standard solution} and \ref{rmk: HRY solution}, exceptional loop arises from adjoining a formal colimit of a pair of parallel morphisms $id, \tau \colon (\shortmid) \rightrightarrows (\shortmid)$ of graphs, in \cref{s. Unital}, the cone is  induced by a formal limit (specifically, the morphism $z: \C_\nul \to (\shortmid)$, \cref{pointed graphical species}) of the same diagram $id, \tau \colon (\shortmid) \rightrightarrows (\shortmid)$. %looks more like a formal limit. \srnote{1503 slight change.} 
			\begin{figure}
				[htb!]
				\begin{tikzpicture}
				\node at (-2,1.8){(a)};
				\node at (-.5,.5){\begin{tikzpicture}[scale = .5]
					
					
					
					
					\draw [ thick]
					(-1.5,-.75)--(-1.5,.75)
					(3,0) circle (.75cm);
					
					
					
					\draw[gray, ->]
					(-1,0 ) -- (2,0);
					\node at (.5,-.5){\tiny{join ends}};
					
					%(-1.5,2.5)--(-1.5,4)
					%(1.5,2.5)-- (1.5,4);
					
					
					\end{tikzpicture}};
				%	\node at (-.5,3){(a)};
%				\node at (2,2.5){\begin{tikzpicture}[scale = .5]
%					
%					
%					
%					\node at (0, .5){\tiny{id}};
%					\node at (0, -.5){\tiny{flip}};
%					\draw [ thick]
%					(-1.5,-.75)--(-1.5,.75)
%					(1.5,-.75)-- (1.5,.75);
%					
%					
%					
%					\draw[gray, ->]
%					(-1.2,.2 ) -- (1.2,.2);
%					\draw[gray, ->]
%					(-1.2,-.2 ) -- (1.2,-.2);
%					%(-1.5,2.5)--(-1.5,4)
%					%(1.5,2.5)-- (1.5,4);
%					
%					
%					\end{tikzpicture}
%				};
\node at (2.5,1.8){(b)};
			\node at (8.5,0){\begin{tikzpicture}[scale = .45]
				\draw[ thin, dashed , red] (-12,4)--(12,-4)
				(-12,-4)--(12,4);
				
				\draw [thick](3,1) arc [start angle=90,   
				end angle=450,
				y radius=1cm, 
				x radius=.5cm]
				%node \node[draw,fill=blue,circle,text=white] at ($(2,0)+(75:2 and 1)$) {A};
				node [pos=.25] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}} ;;
				%                                                  node [pos=.5] {2.10}  
				%                                                  node [pos=.75] {PGF};;
%					\draw [thin,gray, ->] (.2,3.4) arc [start angle=-70,   
%					end angle= 250,
%					y radius=.5cm, 
%					x radius=.5cm];
				\draw[ thin,gray, ->]
				(0,.3) -- (0,1.5)
				(-2.8,1.2) -- (-1, 2.4);
				\draw[thin,gray, ->]
				(-5.8,2.2) -- (-1,2.8);
				\draw[thin,gray, ->]
				(-8.8,3.2) -- (-1,3.2);
				
				
				\draw[thick, gray, ->]
				(0,.3) -- (0,2);
				\draw[thin,gray, ->]
				(2.8,1.2) -- (1, 2.4);
				\draw[thin,gray, ->]
				(5.8,2.2) -- (1,2.8);
				\draw[thin,gray, ->]
				(8.8,3.2) -- (1,3.2);
				
				\draw[ thin, gray, ->]
				(-11,0) -- (-9.4,0);
				\draw[  thin,gray, ->]
				(-8.7,0) -- (-6.3,0);
				\draw[  thin, gray, ->]
				(-5.5,0) -- (-3.1,0);
				\draw[thick, gray, dotted]
				(-12.5,0)--(-11,0);
				\draw[  thin, gray, ->]
				(11,0) -- (9.4,0);
				\draw[  thin,gray, ->]
				(8.7,0) -- (6.3,0);
				\draw[  thin, gray, ->]
				(5.5,0) -- (3.1,0);
				\draw[thick, gray, dotted]
				(12.5,0)--(11,0);
				
				\node at (0,-2){\scriptsize{$\cong$}};
				\node at (0.2, 1){\scriptsize{$z$}};
				%(-2.8,1.2) -- (-1, 2.4);
				%\draw[gray, ->]
				%(-5.8,2.2) -- (-1,2.8);
				%\draw[gray, ->]
				%(-8.8,3.2) -- (-1,3.2);
				
				%\draw[gray, ->]
				%(-1.2,3 ) -- (1.2,3);
				%\draw[gray, ->]
				%(-1.2,3.5 ) -- (1.2,3.5);
				
				\draw[thin,gray, <->]
				(-2.6,-1.2) -- (2.6, -1.2);
				\draw[thin,gray, <->]
				(-5.6,-2.2) -- (5.6, -2.2);
				\draw[thin,gray, <->]
				(-8.6,-3.2) -- (8.6, -3.2);
				\draw [ thick]
				(0,2.5)--(0,4);
				
				%(-1.5,2.5)--(-1.5,4)
				%(1.5,2.5)-- (1.5,4);
				\filldraw  (0,0)        circle (4pt);
				\draw [thick](-3,1) arc [start angle=90,   
				end angle=450,
				y radius=1cm, 
				x radius=.5cm]
				node [pos=.75] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}} ;;
				\draw [thick](6,2) arc [start angle=90,   
				end angle=450,
				y radius=2cm, 
				x radius=1cm]
				node [pos=0] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}}
				node [pos=.5] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}}  ;;
				\draw[thick] (-6,2) arc [start angle=90,   
				end angle=450,
				y radius=2cm, 
				x radius=.75cm]
				node [pos=0] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}}
				node [pos=.5] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}}  ;;
				\draw [thick](9,3) arc [start angle=90,   
				end angle=450,
				y radius=3cm, 
				x radius=1.5cm]
				node [pos=.25] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}}
				node [pos=.6] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}} 
				node [pos=-.1] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}}  ;;
				\draw [thick] (-9,3) arc [start angle=90,   
				end angle=450,
				y radius=3cm, 
				x radius=1.2 cm]
				node [pos=-.25] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}}
				node [pos=-.6] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}} 
				node [pos=.1] {\begin{tikzpicture}\filldraw (0,0) circle (2pt);\end{tikzpicture}}  ;;
				%                  circle
				%                              %  node \node[draw,fill=blue,circle,text=white] at ($(2,0)+(75:2 and 1)$) {A};
				%                                node [pos=.25, draw,fill=blue,circle,text=white] {CVS !!} 
				%                                node [pos=.5] {2.10}  
				%                                node [pos=.75] {PGF};
				%raw(8,0)--(8,-2);
				%                                
				
			\end{tikzpicture}
			
			};
				\end{tikzpicture}
			\caption{(a) Joining the ends of an edge forms an exceptional loop. (b) In \cref{subs. similar} the contraction of units is described in terms of a double cone in the category $\nul\Grsimp$. }% (\cref{subs. similar}).} 
			\label{fig: contracting units}%The map in (a) is a formal coequaliser, while, in (b) $z$ is a formal equaliser of the diagram 
			\end{figure}
		\srnote{2503 - decide where to put the diagram. Here or in Section 7}
			
%			
%			
%			Under this construction, contraction of units is not described by a graph construction that looks like a loop, REF. Instead, the contraction of units may be understood, using the morphism $z$, in terms of a double cone of wheel-like graphs REF.
			
			
%			an exceptional loop. Instead, it is described by a cone-like category (\cref{}) of graphs containing the circle or `wheel graphs' (\cref{fig. line and wheel}) and the singular point or `exceptional vertex' (\cref{defn: valency}). \srnote{\warn{say something about cones?ASK!!}}
			
			
			\item The monad $\DD$ that describes units (\cref{forget monadic}), and the distributive law (\cref{monads distribute} ) induce a notion of equivalence, or `similarity', of graphs whereby it is always possible to work with well-behaved representatives (e.g.~away from the conical singularity in \cref{fig: contracting units}(b)), and only quotient by equivalence at the end. This is important in the proof of \cref{nerve theorem}. 	
		\end{itemize}
		
		Finally, the Nerve \cref{thm: nerve intro} is proved in \cref{s. nerve}, which ends with a % in contains the proof of the nerve theorem, , \cref{cor: model} and a 
		short discussion on weak modular operads.\footnote{Most of Sections \ref{s. graphs}-\ref{sec: non-unital} and \cref{s. nerve} appeared in my PhD thesis \cite{Ray18}. There are some more substantial differences between \cite{Ray18} and Sections \ref{degenerate} and \ref{s. Unital}, since \cite{Ray18} did not make use of the distributive law.}% as well as a brief discussion of the results.
		
		


==> CSMbib.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for Sophie Raynor at 2020-08-25 12:26:21 +1000 


%% Saved with string encoding Unicode (UTF-8) 



@electronic{Ray20,
	Author = {S. Raynor},
	Date-Added = {2020-08-25 12:25:07 +1000},
	Date-Modified = {2020-08-25 12:26:09 +1000},
	Title = {Graphical combinatorics and a distributive law for modular operads}}

@misc{BCL20,
	Archiveprefix = {arXiv},
	Author = {Luciana Basualdo Bonatto and Safia Chettih and Abigail Linton and Sophie Raynor and Marcy Robertson and Nathalie Wahl},
	Date-Added = {2020-08-25 12:24:42 +1000},
	Date-Modified = {2020-08-25 12:24:52 +1000},
	Eprint = {2007.01588},
	Primaryclass = {math.AT},
	Title = {An infinity operad of normalized cacti},
	Year = {2020}}

@article{BHR19,
	Author = {Boavida de Brito, Pedro and Horel, Geoffroy and Robertson, Marcy},
	Date-Added = {2020-08-25 11:35:28 +1000},
	Date-Modified = {2020-08-25 12:24:42 +1000},
	Doi = {10.2140/gt.2019.23.299},
	Fjournal = {Geometry \& Topology},
	Issn = {1465-3060},
	Journal = {Geom. Topol.},
	Mrclass = {18D50 (14G32 32G15 55P48 55U35)},
	Mrnumber = {3921321},
	Mrreviewer = {Alastair Hamilton},
	Number = {1},
	Pages = {299--346},
	Title = {Operads of genus zero curves and the {G}rothendieck-{T}eichm\"{u}ller group},
	Url = {https://doi-org.simsrad.net.ocs.mq.edu.au/10.2140/gt.2019.23.299},
	Volume = {23},
	Year = {2019},
	Bdsk-Url-1 = {https://doi-org.simsrad.net.ocs.mq.edu.au/10.2140/gt.2019.23.299},
	Bdsk-Url-2 = {https://doi.org/10.2140/gt.2019.23.299}}

@incollection{MR2342815,
	Author = {Berger, Clemens and Moerdijk, Ieke},
	Booktitle = {Categories in algebra, geometry and mathematical physics},
	Date-Added = {2020-08-24 19:16:02 +1000},
	Date-Modified = {2020-08-24 19:16:02 +1000},
	Doi = {10.1090/conm/431/08265},
	Mrclass = {18D50 (18G55 55U35)},
	Mrnumber = {2342815},
	Pages = {31--58},
	Publisher = {Amer. Math. Soc., Providence, RI},
	Series = {Contemp. Math.},
	Title = {Resolution of coloured operads and rectification of homotopy algebras},
	Url = {https://doi-org.simsrad.net.ocs.mq.edu.au/10.1090/conm/431/08265},
	Volume = {431},
	Year = {2007},
	Bdsk-Url-1 = {https://doi-org.simsrad.net.ocs.mq.edu.au/10.1090/conm/431/08265},
	Bdsk-Url-2 = {https://doi.org/10.1090/conm/431/08265}}

@article{Ray20a,
	Author = {Raynor, S.},
	Date-Added = {2019-11-05 17:09:37 +1100},
	Date-Modified = {2019-11-05 17:10:36 +1100},
	Journal = {In preparation},
	Title = {A functorial approach to (higher) circuit algebras},
	Year = {2020}}

@article{DHR19,
	Author = {Dansco, Halacheva, Robertson},
	Date-Added = {2019-11-05 17:08:15 +1100},
	Date-Modified = {2019-11-05 17:09:15 +1100},
	Journal = {In preparation},
	Title = {WHEELED PROPS AND CIRCUIT ALGEBRAS},
	Year = {2019}}

@article{BND17,
	Author = {Bar-Natan, Dror and Dancso, Zsuzsanna},
	Date-Added = {2019-11-05 17:07:07 +1100},
	Date-Modified = {2019-11-05 17:07:17 +1100},
	Doi = {10.1007/s00208-016-1388-z},
	Fjournal = {Mathematische Annalen},
	Issn = {0025-5831},
	Journal = {Math. Ann.},
	Mrclass = {57M25 (17B01 57Q45)},
	Mrnumber = {3623232},
	Mrreviewer = {Ismar Voli\'{c}},
	Number = {3-4},
	Pages = {1517--1586},
	Title = {Finite type invariants of w-knotted objects {II}: tangles, foams and the {K}ashiwara-{V}ergne problem},
	Url = {https://doi.org/10.1007/s00208-016-1388-z},
	Volume = {367},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1007/s00208-016-1388-z}}

@article{Ray19,
	Author = {Raynor, S.},
	Date-Added = {2019-11-05 16:54:19 +1100},
	Date-Modified = {2019-11-05 16:55:01 +1100},
	Journal = {Under review},
	Title = {A distributive law for compact symmetric multicategories},
	Year = {2019}}

@book{Koc04,
	Author = {Kock, Joachim},
	Date-Added = {2019-08-23 15:14:05 +1000},
	Date-Modified = {2019-08-23 15:14:27 +1000},
	Isbn = {0-521-83267-5; 0-521-54031-3},
	Mrclass = {57R56 (16L60 18D10 53D45 81T45)},
	Mrnumber = {2037238},
	Mrreviewer = {Lowell Abrams},
	Pages = {xiv+240},
	Publisher = {Cambridge University Press, Cambridge},
	Series = {London Mathematical Society Student Texts},
	Title = {Frobenius algebras and 2{D} topological quantum field theories},
	Volume = {59},
	Year = {2004}}

@article{Til96,
	Author = {Tillmann, Ulrike},
	Date-Added = {2019-08-23 15:14:05 +1000},
	Date-Modified = {2019-08-23 15:14:17 +1000},
	Doi = {10.1515/crll.1996.479.67},
	Fjournal = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's Journal]},
	Issn = {0075-4102},
	Journal = {J. Reine Angew. Math.},
	Mrclass = {55U99 (18B99 55P99 57M99)},
	Mrnumber = {1414388},
	Mrreviewer = {J. P. May},
	Pages = {67--75},
	Title = {The classifying space of the {$(1+1)$}-dimensional cobordism category},
	Url = {https://doi.org/10.1515/crll.1996.479.67},
	Volume = {479},
	Year = {1996},
	Bdsk-Url-1 = {https://doi.org/10.1515/crll.1996.479.67}}

@article{Shi08,
	Author = {J.C. Shillcock},
	Date-Added = {2019-08-20 17:46:46 +1000},
	Date-Modified = {2019-08-20 17:46:46 +1000},
	Journal = {HFSP Journal},
	Note = {doi:10.2976/1.2833599},
	Pages = {1-6},
	Title = {Insight or illusion? Seeing inside the cell with mesoscopic simulations},
	Volume = {2(1)},
	Year = {2008}}

@article{Spi13,
	Author = {D. Spivak},
	Date-Added = {2019-08-20 17:46:46 +1000},
	Date-Modified = {2019-08-20 17:46:46 +1000},
	Journal = {{P}reprint},
	Note = {ar{X}iv:1305.0297},
	Title = {The operad of wiring diagrams},
	Year = {2013}}

@article{ST15,
	Author = {{Spivak}, D.~I. and {Tan}, J.~Z.},
	Date-Added = {2019-08-20 17:46:46 +1000},
	Date-Modified = {2019-08-20 17:46:46 +1000},
	Journal = {{P}reprint},
	Note = {ar{X}iv:1502.07380},
	Title = {{Nesting of dynamic systems and mode-dependent networks}},
	Year = 2015}

@article{Oll09,
	Author = {Yann Ollivier},
	Date-Added = {2019-08-20 17:46:28 +1000},
	Date-Modified = {2019-08-20 17:46:28 +1000},
	Doi = {https://doi.org/10.1016/j.jfa.2008.11.001},
	Issn = {0022-1236},
	Journal = {Journal of Functional Analysis},
	Keywords = {Ricci curvature, Markov chains, Metric geometry, Concentration of measure},
	Number = {3},
	Pages = {810 - 864},
	Title = {Ricci curvature of Markov chains on metric spaces},
	Url = {http://www.sciencedirect.com/science/article/pii/S002212360800493X},
	Volume = {256},
	Year = {2009},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S002212360800493X},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.jfa.2008.11.001}}

@article{PBM11,
	Author = {R. Perin and T. Berger and H. Markram},
	Date-Added = {2019-08-20 17:46:28 +1000},
	Date-Modified = {2019-08-20 17:46:28 +1000},
	Journal = {PNAS},
	Note = {Article 1},
	Title = {A synaptic organizing principle for cortical neuronal groups},
	Volume = {109},
	Year = {2011}}

@article{Pon16,
	Abstract = {The Lefschetz number and fixed point index can be thought of as two different descriptions of the same invariant. The Lefschetz number is algebraic and defined using homology. The index is defined more directly from the topology and is a stable homotopy class. Both the Lefschetz number and index admit generalizations to coincidences and the comparison of these invariants retains its central role. In this paper, we show that the identification of the Lefschetz number and index using formal properties of the symmetric monoidal trace extends to coincidence invariants. This perspective on the coincidence index and Lefschetz number also suggests difficulties for generalizations to a coincidence Reidemeister trace.},
	Author = {Ponto, Kate},
	Date-Added = {2019-08-20 17:46:28 +1000},
	Date-Modified = {2019-08-20 17:46:28 +1000},
	Day = {01},
	Doi = {10.1007/s11784-015-0269-5},
	Issn = {1661-7746},
	Journal = {Journal of Fixed Point Theory and Applications},
	Month = {Mar},
	Number = {1},
	Pages = {147--165},
	Title = {Coincidence invariants and higher Reidemeister traces},
	Url = {https://doi.org/10.1007/s11784-015-0269-5},
	Volume = {18},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1007/s11784-015-0269-5},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/s11784-015-0269-5}}

@phdthesis{Ray18,
	Author = {S. Raynor},
	Date-Added = {2019-08-20 17:46:28 +1000},
	Date-Modified = {2019-08-20 17:46:28 +1000},
	School = {University of Aberdeen},
	Title = {Compact Symmetric Multicategories and the problem of loops},
	Year = {2018}}

@article{Ray19b,
	Author = {Raynor, S.},
	Date-Added = {2019-08-20 17:46:28 +1000},
	Date-Modified = {2019-11-05 17:07:07 +1100},
	Journal = {In preparation, expected submission December 2019},
	Title = {C{S}{M}s with product: an iterated distributive law for compact closed categories},
	Year = {2019}}

@article{Rets17,
	Abstract = {The lack of a formal link between neural network structure and its emergent function has hampered our understanding of how the brain processes information. We have now come closer to describing such a link by taking the direction of synaptic transmission into account, constructing graphs of a network that reflect the direction of information flow, and analyzing these directed graphs using algebraic topology. Applying this approach to a local network of neurons in the neocortex revealed a remarkably intricate and previously unseen topology of synaptic connectivity. The synaptic network contains an abundance of cliques of neurons bound into cavities that guide the emergence of correlated activity. In response to stimuli, correlated activity binds synaptically connected neurons into functional cliques and cavities that evolve in a stereotypical sequence towards peak complexity. We propose that the brain processes stimuli by forming increasingly complex functional cliques and cavities.},
	Author = {Reimann, Michael W. and Nolte, Max and Scolamiero, Martina and Turner, Katharine and Perin, Rodrigo and Chindemi, Giuseppe and D{\l}otko, Pawe{\l} and Levi, Ran and Hess, Kathryn and Markram, Henry},
	Date-Added = {2019-08-20 17:46:28 +1000},
	Date-Modified = {2019-08-20 17:46:28 +1000},
	Doi = {10.3389/fncom.2017.00048},
	Issn = {1662-5188},
	Journal = {Frontiers in Computational Neuroscience},
	Pages = {48},
	Title = {Cliques of Neurons Bound into Cavities Provide a Missing Link between Structure and Function},
	Url = {https://www.frontiersin.org/article/10.3389/fncom.2017.00048},
	Volume = {11},
	Year = {2017},
	Bdsk-Url-1 = {https://www.frontiersin.org/article/10.3389/fncom.2017.00048},
	Bdsk-Url-2 = {http://dx.doi.org/10.3389/fncom.2017.00048}}

@book{Lur11,
	Author = {A. Lurie},
	Date-Added = {2019-08-20 17:46:08 +1000},
	Date-Modified = {2019-08-20 17:46:08 +1000},
	Title = {Higher Algebra}}

@article{HRY19b,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190601144H},
	Archiveprefix = {arXiv},
	Author = {{Hackney}, Philip and {Robertson}, Marcy and {Yau}, Donald},
	Date-Added = {2019-08-20 17:45:31 +1000},
	Date-Modified = {2019-08-20 17:45:31 +1000},
	Eid = {arXiv:1906.01144},
	Eprint = {1906.01144},
	Journal = {arXiv e-prints},
	Keywords = {Mathematics - Category Theory, Mathematics - Algebraic Topology},
	Month = {Jun},
	Pages = {arXiv:1906.01144},
	Primaryclass = {math.CT},
	Title = {{Modular operads and the nerve theorem}},
	Year = {2019}}

@article{HRY19a,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190601143H},
	Archiveprefix = {arXiv},
	Author = {{Hackney}, Philip and {Robertson}, Marcy and {Yau}, Donald},
	Date-Added = {2019-08-20 17:45:31 +1000},
	Date-Modified = {2019-08-20 17:45:31 +1000},
	Eid = {arXiv:1906.01143},
	Eprint = {1906.01143},
	Journal = {arXiv e-prints},
	Keywords = {Mathematics - Algebraic Topology, Mathematics - Category Theory},
	Month = {Jun},
	Pages = {arXiv:1906.01143},
	Primaryclass = {math.AT},
	Title = {{A graphical category for higher modular operads}},
	Year = {2019}}

@article{JK11,
	Author = {Joyal, A. and Kock, J.},
	Date-Added = {2019-08-20 17:45:31 +1000},
	Date-Modified = {2019-08-20 17:45:31 +1000},
	Journal = {Electronic Note in Theoretical Computer Science},
	Note = {Proceedings of the 6th International Workshop on Quantum Physics and Logic (QPL 2009)},
	Number = {2},
	Pages = {105 - 113},
	Title = {Feynman Graphs, and Nerve Theorem for Compact Symmetric Multicategories (Extended Abstract)},
	Volume = {270},
	Year = {2011}}

@article{Gia13,
	Author = {Jeffrey Giansiracusa},
	Date-Added = {2019-08-20 17:45:06 +1000},
	Date-Modified = {2019-08-20 17:45:06 +1000},
	Journal = {Morfismos},
	Number = {2},
	Pages = {101--125},
	Title = {Moduli spaces and modular operads},
	Volume = {17},
	Year = {2013}}

@inproceedings{DCH19,
	Author = {Gabriel C. Drummond-Cole and Philip Hackney},
	Date-Added = {2019-08-20 17:44:46 +1000},
	Date-Modified = {2019-08-20 17:44:46 +1000},
	Title = {Dwyer--{K}an homotopy theory for cyclic operads},
	Year = {2018}}

@article{DH15,
	Author = {W. Dwyer and K. Hess},
	Date-Added = {2019-08-20 17:44:46 +1000},
	Date-Modified = {2019-08-20 17:44:46 +1000},
	Journal = {preprint},
	Note = {arXiv:1312.1269v2 [math.AT]},
	Title = {RESOLUTIONS OF RIGHT-ANGLED ARTIN MONOIDS AND OPERADS},
	Year = {2015}}

@article{Fon15,
	Author = {Fong, B.},
	Date-Added = {2019-08-20 17:44:46 +1000},
	Date-Modified = {2019-08-20 17:44:46 +1000},
	Journal = {Theory and Applications of Categories},
	Number = {33},
	Pages = {1096--1120},
	Title = {Decorated cospans},
	Volume = {30},
	Year = {2015}}

@phdthesis{Fon16,
	Author = {{Fong}, B.},
	Date-Added = {2019-08-20 17:44:46 +1000},
	Date-Modified = {2019-08-20 17:44:46 +1000},
	Journal = {{P}reprint},
	Note = {ar{X}iv:1609.05382},
	School = {Oxford University},
	Title = {{The Algebra of Open and Interconnected Systems}},
	Year = 2016}

@inproceedings{DJP17,
	Author = {Martin Doubek and Branislav Juro and Lada Peksova},
	Date-Added = {2019-08-20 17:44:14 +1000},
	Date-Modified = {2019-08-20 17:44:14 +1000},
	Title = {Properads and Homotopy Algebras Related to Surfaces.},
	Year = {2017}}

@misc{Bae17,
	Author = {J. Baez},
	Date-Added = {2019-08-20 17:43:37 +1000},
	Date-Modified = {2019-08-20 17:43:37 +1000},
	Howpublished = {http://math.ucr.edu/home/baez/networks/},
	Keywords = {Networks, Chemical reaction networks, Petri net, Quantum, Stochastic},
	Lastchecked = {29 September 2017},
	Title = {{N}etwork theory page},
	Url = {http://math.ucr.edu/home/baez/networks/},
	Bdsk-Url-1 = {http://math.ucr.edu/home/baez/networks/}}

@article{BCR17,
	Author = {{Baez}, J.~C. and {Coya}, B. and {Rebro}, F.},
	Date-Added = {2019-08-20 17:43:37 +1000},
	Date-Modified = {2019-08-20 17:43:37 +1000},
	Journal = {{P}reprint},
	Note = {ar{X}iv:1707.08321},
	Title = {Props in Network Theory},
	Year = 2017}

@article{BO15,
	Author = {{Baez}, J.~C. and {Otter}, N.},
	Date-Added = {2019-08-20 17:43:37 +1000},
	Date-Modified = {2019-08-20 17:43:37 +1000},
	Journal = {{P}reprint},
	Note = {ar{X}iv:1512.03337},
	Title = {{Operads and Phylogenetic Trees}},
	Year = 2015}

@article{BP17,
	Author = {{Baez}, J.~C. and {Pollard}, B.~S.},
	Date-Added = {2019-08-20 17:43:37 +1000},
	Date-Modified = {2019-08-20 17:43:37 +1000},
	Doi = {10.1142/S0129055X17500283},
	Eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0129055X17500283},
	Journal = {Reviews in Mathematical Physics},
	Number = {09},
	Pages = {1750028},
	Title = {A compositional framework for reaction networks},
	Url = {http://www.worldscientific.com/doi/abs/10.1142/S0129055X17500283},
	Volume = {29},
	Year = {2017},
	Bdsk-Url-1 = {http://www.worldscientific.com/doi/abs/10.1142/S0129055X17500283},
	Bdsk-Url-2 = {http://dx.doi.org/10.1142/S0129055X17500283}}

@article{BN15,
	Author = {Ba{\v s}i{\'c}, M. and Nikolaus, T.},
	Date-Added = {2019-08-20 17:43:37 +1000},
	Date-Modified = {2019-08-20 17:43:37 +1000},
	Journal = {Homology, Homotopy and Applications},
	Number = {09},
	Title = {Homology of dendroidal sets},
	Volume = {19},
	Year = {2015}}

@article{Bas10,
	Author = {D. S. Bassett and others},
	Date-Added = {2019-08-20 17:43:37 +1000},
	Date-Modified = {2019-08-20 17:43:37 +1000},
	Journal = {PLos Comp. Biology},
	Note = {e1000748},
	Title = {Efficient physical embedding of topologically complex information processing networks in brains and computer circuits},
	Volume = {6},
	Year = {2010}}

@inproceedings{AC04,
	Acmid = {1021878},
	Address = {Washington, DC, USA},
	Author = {Abramsky, S. and Coecke, B.},
	Booktitle = {Proceedings of the 19th Annual IEEE Symposium on Logic in Computer Science},
	Date-Added = {2019-08-20 17:43:14 +1000},
	Date-Modified = {2019-08-20 17:43:14 +1000},
	Doi = {10.1109/LICS.2004.1},
	Isbn = {0-7695-2192-4},
	Numpages = {11},
	Pages = {415--425},
	Publisher = {IEEE Computer Society},
	Series = {LICS '04},
	Title = {A Categorical Semantics of Quantum Protocols},
	Url = {https://doi.org/10.1109/LICS.2004.1},
	Year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.1109/LICS.2004.1},
	Bdsk-Url-2 = {http://dx.doi.org/10.1109/LICS.2004.1}}

@misc{QuaOx,
	Author = {S. Abramsky and B. Coecke and others},
	Date-Added = {2019-08-20 17:43:14 +1000},
	Date-Modified = {2019-08-20 17:43:14 +1000},
	Howpublished = {http://www.cs.ox.ac.uk/activities/quantum/},
	Keywords = {Quantum, Category, Logic, Semantics, Computations, Physics},
	Lastchecked = {29 September 2017},
	Title = {{H}omepage of {O}xford {Q}uantum {G}roup},
	Url = {http://www.cs.ox.ac.uk/activities/quantum/},
	Bdsk-Url-1 = {http://www.cs.ox.ac.uk/activities/quantum/}}

@article{AB11,
	Author = {S. Abramsky and A. Brandenburger},
	Date-Added = {2019-08-20 17:43:00 +1000},
	Date-Modified = {2019-08-20 17:43:00 +1000},
	Doi = {10.1088/1367-2630/13/11/113036},
	Issn = {1327-2630},
	Journal = {New Journal of Physics},
	Pages = {113036-113075},
	Title = {The Sheaf-Theoretic Structure of Non-Locality and Contextuality},
	Url = {http://iopscience.iop.org/1367-2630/13/11/113036},
	Volume = {13},
	Year = {2011},
	Bdsk-Url-1 = {http://iopscience.iop.org/1367-2630/13/11/113036},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/1367-2630/13/11/113036}}

@incollection{AC08,
	Author = {Abramsky, Samson and Coecke, Bob},
	Booktitle = {Handbook of quantum logic and quantum structures---quantum logic},
	Doi = {10.1016/B978-0-444-52869-8.50010-4},
	Mrclass = {81P10 (18B99 18D10 81P45)},
	Mrnumber = {2724650},
	Mrreviewer = {Benno van den Berg},
	Pages = {261--323},
	Publisher = {Elsevier/North-Holland, Amsterdam},
	Title = {Categorical quantum mechanics},
	Url = {https://doi.org/10.1016/B978-0-444-52869-8.50010-4},
	Year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1016/B978-0-444-52869-8.50010-4}}

@article{Bar07,
	Author = {Barannikov, Serguei},
	Doi = {10.1093/imrn/rnm075},
	Fjournal = {International Mathematics Research Notices. IMRN},
	Issn = {1073-7928},
	Journal = {Int. Math. Res. Not. IMRN},
	Mrclass = {18D50 (53D45 81T18)},
	Mrnumber = {2359547},
	Mrreviewer = {Domenico Fiorenza},
	Number = {19},
	Pages = {Art. ID rnm075, 31},
	Title = {Modular operads and {B}atalin-{V}ilkovisky geometry},
	Url = {https://doi.org/10.1093/imrn/rnm075},
	Year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.1093/imrn/rnm075}}

@article{BB17,
	Author = {Batanin, M. A. and Berger, C.},
	Fjournal = {Theory and Applications of Categories},
	Issn = {1201-561X},
	Journal = {Theory Appl. Categ.},
	Mrclass = {18D20 (18C15 18D50 55P48)},
	Mrnumber = {3607212},
	Mrreviewer = {Javier J. Guti\'{e}rrez},
	Pages = {Paper No. 6, 148--253},
	Title = {Homotopy theory for algebras over polynomial monads},
	Volume = {32},
	Year = {2017}}

@incollection{Bec69,
	Author = {Beck, Jon},
	Booktitle = {Sem. on {T}riples and {C}ategorical {H}omology {T}heory ({ETH}, {Z}\"{u}rich, 1966/67)},
	Mrclass = {18.20},
	Mrnumber = {0241502},
	Mrreviewer = {J. R. Isbell},
	Pages = {119--140},
	Publisher = {Springer, Berlin},
	Title = {Distributive laws},
	Year = {1969}}

@article{BM06,
	Author = {Berger, Clemens and Moerdijk, Ieke},
	Doi = {10.1016/j.top.2006.05.001},
	Fjournal = {Topology. An International Journal of Mathematics},
	Issn = {0040-9383},
	Journal = {Topology},
	Mrclass = {18D50 (18G55 55P48 55U35)},
	Mrnumber = {2248514},
	Mrreviewer = {Agust\'{\i} Roig},
	Number = {5},
	Pages = {807--849},
	Title = {The {B}oardman-{V}ogt resolution of operads in monoidal model categories},
	Url = {https://doi.org/10.1016/j.top.2006.05.001},
	Volume = {45},
	Year = {2006},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.top.2006.05.001}}

@incollection{BM07,
	Author = {Berger, Clemens and Moerdijk, Ieke},
	Booktitle = {Categories in algebra, geometry and mathematical physics},
	Doi = {10.1090/conm/431/08265},
	Mrclass = {18D50 (18G55 55U35)},
	Mrnumber = {2342815},
	Pages = {31--58},
	Publisher = {Amer. Math. Soc., Providence, RI},
	Series = {Contemp. Math.},
	Title = {Resolution of coloured operads and rectification of homotopy algebras},
	Url = {https://doi.org/10.1090/conm/431/08265},
	Volume = {431},
	Year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.1090/conm/431/08265}}

@article{BMW12,
	Author = {Berger, Clemens and Melli\`es, Paul-Andr\'{e} and Weber, Mark},
	Doi = {10.1016/j.jpaa.2012.02.039},
	Fjournal = {Journal of Pure and Applied Algebra},
	Issn = {0022-4049},
	Journal = {J. Pure Appl. Algebra},
	Mrclass = {18C10 (18B40 18C15 18D50)},
	Mrnumber = {2925893},
	Mrreviewer = {Enrico Vitale},
	Number = {8-9},
	Pages = {2029--2048},
	Title = {Monads with arities and their associated theories},
	Url = {https://doi.org/10.1016/j.jpaa.2012.02.039},
	Volume = {216},
	Year = {2012},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.jpaa.2012.02.039}}

@book{BorIII94,
	Author = {Borceux, Francis},
	Isbn = {0-521-44180-3},
	Mrclass = {18-02 (18B25 18F20)},
	Mrnumber = {1315049},
	Mrreviewer = {Martin Hyland},
	Note = {Categories of sheaves},
	Pages = {xviii+522},
	Publisher = {Cambridge University Press, Cambridge},
	Series = {Encyclopedia of Mathematics and its Applications},
	Title = {Handbook of categorical algebra. 3},
	Volume = {52},
	Year = {1994}}

@book{Bor94,
	Author = {Borceux, Francis},
	Isbn = {0-521-44178-1},
	Mrclass = {18-02 (18Axx)},
	Mrnumber = {1291599},
	Mrreviewer = {Martin Hyland},
	Note = {Basic category theory},
	Pages = {xvi+345},
	Publisher = {Cambridge University Press, Cambridge},
	Series = {Encyclopedia of Mathematics and its Applications},
	Title = {Handbook of categorical algebra. 1},
	Volume = {50},
	Year = {1994}}

@book{BorII94,
	Author = {Borceux, Francis},
	Isbn = {0-521-44179-X},
	Mrclass = {18-02 (18Exx)},
	Mrnumber = {1313497},
	Mrreviewer = {Martin Hyland},
	Note = {Categories and structures},
	Pages = {xviii+443},
	Publisher = {Cambridge University Press, Cambridge},
	Series = {Encyclopedia of Mathematics and its Applications},
	Title = {Handbook of categorical algebra. 2},
	Volume = {51},
	Year = {1994}}

@incollection{BM08,
	Author = {Borisov, Dennis V. and Manin, Yuri I.},
	Booktitle = {Geometry and dynamics of groups and spaces},
	Doi = {10.1007/978-3-7643-8608-5_4},
	Mrclass = {18D50 (18D10 18D15)},
	Mrnumber = {2402406},
	Mrreviewer = {Beno\^{\i}t Fresse},
	Pages = {247--308},
	Publisher = {Birkh\"{a}user, Basel},
	Series = {Progr. Math.},
	Title = {Generalized operads and their inner cohomomorphisms},
	Url = {https://doi.org/10.1007/978-3-7643-8608-5_4},
	Volume = {265},
	Year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1007/978-3-7643-8608-5_4}}

@article{Che11,
	Author = {Cheng, Eugenia},
	Doi = {10.1017/S0305004110000599},
	Fjournal = {Mathematical Proceedings of the Cambridge Philosophical Society},
	Issn = {0305-0041},
	Journal = {Math. Proc. Cambridge Philos. Soc.},
	Mrclass = {18C20 (18D05)},
	Mrnumber = {2784770},
	Mrreviewer = {Enrico Vitale},
	Number = {3},
	Pages = {459--487},
	Title = {Iterated distributive laws},
	Url = {https://doi.org/10.1017/S0305004110000599},
	Volume = {150},
	Year = {2011},
	Bdsk-Url-1 = {https://doi.org/10.1017/S0305004110000599}}

@article{CL07,
	Author = {Chuang, J. and Lazarev, A.},
	Doi = {10.4310/CNTP.2007.v1.n4.a1},
	Fjournal = {Communications in Number Theory and Physics},
	Issn = {1931-4523},
	Journal = {Commun. Number Theory Phys.},
	Mrclass = {81T45 (18D50 81Q30)},
	Mrnumber = {2412267},
	Mrreviewer = {David Chataur},
	Number = {4},
	Pages = {605--649},
	Title = {Dual {F}eynman transform for modular operads},
	Url = {https://doi.org/10.4310/CNTP.2007.v1.n4.a1},
	Volume = {1},
	Year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.4310/CNTP.2007.v1.n4.a1}}

@article{CM13,
	Author = {Cisinski, Denis-Charles and Moerdijk, Ieke},
	Doi = {10.1112/jtopol/jtt006},
	Fjournal = {Journal of Topology},
	Issn = {1753-8416},
	Journal = {J. Topol.},
	Mrclass = {18D50 (18D30 55P48 55U10)},
	Mrnumber = {3100888},
	Mrreviewer = {David Chataur},
	Number = {3},
	Pages = {705--756},
	Title = {Dendroidal sets and simplicial operads},
	Url = {https://doi.org/10.1112/jtopol/jtt006},
	Volume = {6},
	Year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1112/jtopol/jtt006}}

@article{DJM15,
	Author = {Doubek, Martin and Jur\v{c}o, Branislav and M\"{u}nster, Korbinian},
	Doi = {10.1007/jhep12(2015)158},
	Fjournal = {Journal of High Energy Physics},
	Issn = {1126-6708},
	Journal = {J. High Energy Phys.},
	Mrclass = {81R10},
	Mrnumber = {3464644},
	Number = {12},
	Pages = {158, front matter+54pp},
	Title = {Modular operads and the quantum open-closed homotopy algebra},
	Url = {https://doi.org/10.1007/jhep12(2015)158},
	Year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1007/jhep12(2015)158}}

@article{Dou17,
	Author = {Doubek, Martin},
	Doi = {10.1007/s10485-017-9491-1},
	Fjournal = {Applied Categorical Structures. A Journal Devoted to Applications of Categorical Methods in Algebra, Analysis, Order, Topology and Computer Science},
	Issn = {0927-2852},
	Journal = {Appl. Categ. Structures},
	Mrclass = {18D50},
	Mrnumber = {3720407},
	Mrreviewer = {Loic Foissy},
	Number = {6},
	Pages = {1187--1198},
	Title = {The modular envelope of the cyclic operad {$\Cal{A}ss$}},
	Url = {https://doi.org/10.1007/s10485-017-9491-1},
	Volume = {25},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1007/s10485-017-9491-1}}

@incollection{GK95,
	Author = {Getzler, E. and Kapranov, M. M.},
	Booktitle = {Geometry, topology, \& physics},
	Mrclass = {19D55 (08A99 16E40 18G60)},
	Mrnumber = {1358617},
	Mrreviewer = {Alexander A. Voronov},
	Pages = {167--201},
	Publisher = {Int. Press, Cambridge, MA},
	Series = {Conf. Proc. Lecture Notes Geom. Topology, IV},
	Title = {Cyclic operads and cyclic homology},
	Year = {1995}}

@article{Get98,
	Author = {Getzler, E.},
	Doi = {10.1007/s002200050365},
	Fjournal = {Communications in Mathematical Physics},
	Issn = {0010-3616},
	Journal = {Comm. Math. Phys.},
	Mrclass = {14H10 (14H15 14H52)},
	Mrnumber = {1627677},
	Mrreviewer = {Andreas Gathmann},
	Number = {2},
	Pages = {481--492},
	Title = {The semi-classical approximation for modular operads},
	Url = {https://doi.org/10.1007/s002200050365},
	Volume = {194},
	Year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.1007/s002200050365}}

@article{GK98,
	Author = {Getzler, E. and Kapranov, M. M.},
	Doi = {10.1023/A:1000245600345},
	Fjournal = {Compositio Mathematica},
	Issn = {0010-437X},
	Journal = {Compositio Math.},
	Mrclass = {18C15 (08A02 14H10 57M50)},
	Mrnumber = {1601666},
	Mrreviewer = {Alexandre I. Kabanov},
	Number = {1},
	Pages = {65--126},
	Title = {Modular operads},
	Url = {https://doi.org/10.1023/A:1000245600345},
	Volume = {110},
	Year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.1023/A:1000245600345}}

@incollection{Get09,
	Author = {Getzler, Ezra},
	Booktitle = {Algebra, arithmetic, and geometry: in honor of {Y}u. {I}. {M}anin. {V}ol. {I}},
	Doi = {10.1007/978-0-8176-4745-2_16},
	Mrclass = {18D50 (18C35 57R56)},
	Mrnumber = {2641184},
	Pages = {675--698},
	Publisher = {Birkh\"{a}user Boston, Inc., Boston, MA},
	Series = {Progr. Math.},
	Title = {Operads revisited},
	Url = {https://doi.org/10.1007/978-0-8176-4745-2_16},
	Volume = {269},
	Year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1007/978-0-8176-4745-2_16}}

@article{GLW11,
	Author = {Guti\'{e}rrez, Javier J. and Lukacs, Andor and Weiss, Ittay},
	Doi = {10.1016/j.jpaa.2010.10.003},
	Fjournal = {Journal of Pure and Applied Algebra},
	Issn = {0022-4049},
	Journal = {J. Pure Appl. Algebra},
	Mrclass = {55U05 (18D50)},
	Mrnumber = {2771637},
	Mrreviewer = {Timothy Porter},
	Number = {7},
	Pages = {1669--1687},
	Title = {Dold-{K}an correspondence for dendroidal abelian groups},
	Url = {https://doi.org/10.1016/j.jpaa.2010.10.003},
	Volume = {215},
	Year = {2011},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.jpaa.2010.10.003}}

@book{HRY15,
	Author = {Hackney, Philip and Robertson, Marcy and Yau, Donald},
	Doi = {10.1007/978-3-319-20547-2},
	Isbn = {978-3-319-20546-5; 978-3-319-20547-2},
	Mrclass = {55P48 (18D50 55U35)},
	Mrnumber = {3408444},
	Mrreviewer = {David Chataur},
	Pages = {xv+358},
	Publisher = {Springer, Cham},
	Series = {Lecture Notes in Mathematics},
	Title = {Infinity properads and infinity wheeled properads},
	Url = {https://doi.org/10.1007/978-3-319-20547-2},
	Volume = {2147},
	Year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1007/978-3-319-20547-2}}

@article{HRY18,
	Author = {Hackney, Philip and Robertson, Marcy and Yau, Donald},
	Doi = {10.4310/HHA.2018.v20.n2.a11},
	Fjournal = {Homology, Homotopy and Applications},
	Issn = {1532-0073},
	Journal = {Homology Homotopy Appl.},
	Mrclass = {18D50 (18A20 18G30 18G55 55P48 55U35)},
	Mrnumber = {3812464},
	Mrreviewer = {Beno\^{\i}t Fresse},
	Number = {2},
	Pages = {217--238},
	Title = {On factorizations of graphical maps},
	Url = {https://doi.org/10.4310/HHA.2018.v20.n2.a11},
	Volume = {20},
	Year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.4310/HHA.2018.v20.n2.a11}}

@article{JM94,
	Author = {Joyal, A. and Moerdijk, I.},
	Doi = {10.1016/0168-0072(94)90069-8},
	Fjournal = {Annals of Pure and Applied Logic},
	Issn = {0168-0072},
	Journal = {Ann. Pure Appl. Logic},
	Mrclass = {03G30 (54C10)},
	Mrnumber = {1303663},
	Mrreviewer = {Peter Johnstone},
	Number = {1},
	Pages = {51--86},
	Title = {A completeness theorem for open maps},
	Url = {https://doi.org/10.1016/0168-0072(94)90069-8},
	Volume = {70},
	Year = {1994},
	Bdsk-Url-1 = {https://doi.org/10.1016/0168-0072(94)90069-8}}

@incollection{Kau18,
	Author = {Kaufmann, Ralph M.},
	Booktitle = {2016 {MATRIX} annals},
	Mrclass = {18F99 (16T15 18D50)},
	Mrnumber = {3792531},
	Mrreviewer = {Loic Foissy},
	Pages = {375--438},
	Publisher = {Springer, Cham},
	Series = {MATRIX Book Ser.},
	Title = {Lectures on {F}eynman categories},
	Volume = {1},
	Year = {2018}}

@article{Kel80,
	Author = {Kelly, G. M.},
	Doi = {10.1017/S0004972700006353},
	Fjournal = {Bulletin of the Australian Mathematical Society},
	Issn = {0004-9727},
	Journal = {Bull. Austral. Math. Soc.},
	Mrclass = {18C15 (18A40)},
	Mrnumber = {589937},
	Mrreviewer = {V\'{a}clav Koubek},
	Number = {1},
	Pages = {1--83},
	Title = {A unified treatment of transfinite constructions for free algebras, free monoids, colimits, associated sheaves, and so on},
	Url = {https://doi.org/10.1017/S0004972700006353},
	Volume = {22},
	Year = {1980},
	Bdsk-Url-1 = {https://doi.org/10.1017/S0004972700006353}}

@article{KL80,
	Author = {Kelly, G. M. and Laplaza, M. L.},
	Doi = {10.1016/0022-4049(80)90101-2},
	Fjournal = {Journal of Pure and Applied Algebra},
	Issn = {0022-4049},
	Journal = {J. Pure Appl. Algebra},
	Mrclass = {18D15 (18C10)},
	Mrnumber = {593254},
	Mrreviewer = {M. Barr},
	Pages = {193--213},
	Title = {Coherence for compact closed categories},
	Url = {https://doi.org/10.1016/0022-4049(80)90101-2},
	Volume = {19},
	Year = {1980},
	Bdsk-Url-1 = {https://doi.org/10.1016/0022-4049(80)90101-2}}

@article{Koc16,
	Author = {Kock, Joachim},
	Doi = {10.1007/s13348-015-0160-0},
	Fjournal = {Collectanea Mathematica},
	Issn = {0010-0757},
	Journal = {Collect. Math.},
	Mrclass = {18F20 (05C20 05C65 18D50)},
	Mrnumber = {3484016},
	Mrreviewer = {Marko \v{Z}ivkovi\'{c}},
	Number = {2},
	Pages = {155--190},
	Title = {Graphs, hypergraphs, and properads},
	Url = {https://doi.org/10.1007/s13348-015-0160-0},
	Volume = {67},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1007/s13348-015-0160-0}}

@article{Koc18,
	Author = {Kock, Joachim},
	Doi = {10.5565/PUBLMAT6221802},
	Fjournal = {Publicacions Matem\`atiques},
	Issn = {0214-1493},
	Journal = {Publ. Mat.},
	Mrclass = {18D50 (05C99)},
	Mrnumber = {3815283},
	Mrreviewer = {Marko \v{Z}ivkovi\'{c}},
	Number = {2},
	Pages = {331--353},
	Title = {Cospan construction of the graph category of {B}orisov and {M}anin},
	Url = {https://doi.org/10.5565/PUBLMAT6221802},
	Volume = {62},
	Year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.5565/PUBLMAT6221802}}

@article{KSW17,
	Author = {Kondo, Satoshi and Siegel, Charles and Wolfson, Jesse},
	Doi = {10.2140/gt.2017.21.903},
	Fjournal = {Geometry \& Topology},
	Issn = {1465-3060},
	Journal = {Geom. Topol.},
	Mrclass = {14H10 (18D50)},
	Mrnumber = {3626593},
	Mrreviewer = {Hsian-Hua Tseng},
	Number = {2},
	Pages = {903--922},
	Title = {Modular operads of embedded curves},
	Url = {https://doi.org/10.2140/gt.2017.21.903},
	Volume = {21},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.2140/gt.2017.21.903}}

@book{Lei04,
	Author = {Leinster, Tom},
	Doi = {10.1017/CBO9780511525896},
	Isbn = {0-521-53215-9},
	Mrclass = {18D50 (55P48)},
	Mrnumber = {2094071},
	Mrreviewer = {R. H. Street},
	Pages = {xiv+433},
	Publisher = {Cambridge University Press, Cambridge},
	Series = {London Mathematical Society Lecture Note Series},
	Title = {Higher operads, higher categories},
	Url = {https://doi.org/10.1017/CBO9780511525896},
	Volume = {298},
	Year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.1017/CBO9780511525896}}

@book{MM94,
	Author = {Mac Lane, Saunders and Moerdijk, Ieke},
	Isbn = {0-387-97710-4},
	Mrclass = {03G30 (18B25 54B40)},
	Mrnumber = {1300636},
	Mrreviewer = {M. Makkai},
	Note = {A first introduction to topos theory, Corrected reprint of the 1992 edition},
	Pages = {xii+629},
	Publisher = {Springer-Verlag, New York},
	Series = {Universitext},
	Title = {Sheaves in geometry and logic},
	Year = {1994}}

@book{Mac98,
	Author = {Mac Lane, Saunders},
	Edition = {Second},
	Isbn = {0-387-98403-8},
	Mrclass = {18-02},
	Mrnumber = {1712872},
	Pages = {xii+314},
	Publisher = {Springer-Verlag, New York},
	Series = {Graduate Texts in Mathematics},
	Title = {Categories for the working mathematician},
	Volume = {5},
	Year = {1998}}

@article{MMS09,
	Author = {Markl, M. and Merkulov, S. and Shadrin, S.},
	Doi = {10.1016/j.jpaa.2008.08.007},
	Fjournal = {Journal of Pure and Applied Algebra},
	Issn = {0022-4049},
	Journal = {J. Pure Appl. Algebra},
	Mrclass = {18D50 (18G55)},
	Mrnumber = {2483835},
	Mrreviewer = {Bruno Vallette},
	Number = {4},
	Pages = {496--535},
	Title = {Wheeled {PROP}s, graph complexes and the master equation},
	Url = {https://doi.org/10.1016/j.jpaa.2008.08.007},
	Volume = {213},
	Year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.jpaa.2008.08.007}}

@article{Mar01,
	Author = {Markl, Martin},
	Doi = {10.1007/PL00005575},
	Fjournal = {Communications in Mathematical Physics},
	Issn = {0010-3616},
	Journal = {Comm. Math. Phys.},
	Mrclass = {55P48 (18D50 81T30 81T70)},
	Mrnumber = {1845329},
	Mrreviewer = {J. Stasheff},
	Number = {2},
	Pages = {367--384},
	Title = {Loop homotopy algebras in closed string field theory},
	Url = {https://doi.org/10.1007/PL00005575},
	Volume = {221},
	Year = {2001},
	Bdsk-Url-1 = {https://doi.org/10.1007/PL00005575}}

@incollection{Mar08,
	Author = {Markl, Martin},
	Booktitle = {Handbook of algebra. {V}ol. 5},
	Doi = {10.1016/S1570-7954(07)05002-4},
	Mrclass = {18D50},
	Mrnumber = {2523450},
	Pages = {87--140},
	Publisher = {Elsevier/North-Holland, Amsterdam},
	Series = {Handb. Algebr.},
	Title = {Operads and {PROP}s},
	Url = {https://doi.org/10.1016/S1570-7954(07)05002-4},
	Volume = {5},
	Year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1016/S1570-7954(07)05002-4}}

@article{Mar16,
	Author = {Markl, Martin},
	Doi = {10.4171/JNCG/248},
	Fjournal = {Journal of Noncommutative Geometry},
	Issn = {1661-6952},
	Journal = {J. Noncommut. Geom.},
	Mrclass = {81T30 (14H81 18D35 18D50 32G15)},
	Mrnumber = {3519052},
	Mrreviewer = {Ali Shojaei-Fard},
	Number = {2},
	Pages = {775--809},
	Title = {Modular envelopes, {OSFT} and nonsymmetric (non-{$\Sigma$}) modular operads},
	Url = {https://doi.org/10.4171/JNCG/248},
	Volume = {10},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.4171/JNCG/248}}

@article{MW07,
	Author = {Moerdijk, Ieke and Weiss, Ittay},
	Doi = {10.2140/agt.2007.7.1441},
	Fjournal = {Algebraic \& Geometric Topology},
	Issn = {1472-2747},
	Journal = {Algebr. Geom. Topol.},
	Mrclass = {55P48 (18D10 18G30 55U10 55U40)},
	Mrnumber = {2366165},
	Pages = {1441--1470},
	Title = {Dendroidal sets},
	Url = {https://doi.org/10.2140/agt.2007.7.1441},
	Volume = {7},
	Year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.2140/agt.2007.7.1441}}
	
		@book {Lam66,
    AUTHOR = {Lambek, Joachim},
     TITLE = {Completions of categories},
    SERIES = {Seminar lectures given in 1966 in Z\"{u}rich. Lecture Notes in
              Mathematics, No. 24},
 PUBLISHER = {Springer-Verlag, Berlin-New York},
      YEAR = {1966},
     PAGES = {iv+70},
   MRCLASS = {18.00},
  MRNUMBER = {0209330},
MRREVIEWER = {F. M. Sioson},
}


@article{Pek18,
	Author = {Peksov\'{a}, Lada},
	Doi = {10.5817/am2018-5-299},
	Fjournal = {Universitatis Masarykianae Brunensis. Facultas Scientiarum Naturalium. Archivum Mathematicum},
	Issn = {0044-8753},
	Journal = {Arch. Math. (Brno)},
	Mrclass = {18D50 (18F99)},
	Mrnumber = {3887356},
	Number = {5},
	Pages = {299--312},
	Title = {Properads and homological differential operators related to surfaces},
	Url = {https://doi.org/10.5817/am2018-5-299},
	Volume = {54},
	Year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.5817/am2018-5-299}}

@incollection{Seg88,
	Author = {Segal, G. B.},
	Booktitle = {Differential geometrical methods in theoretical physics ({C}omo, 1987)},
	Mrclass = {58D30 (14H15 32G15 81E05 81E40)},
	Mrnumber = {981378},
	Mrreviewer = {Yukihiko Namikawa},
	Pages = {165--171},
	Publisher = {Kluwer Acad. Publ., Dordrecht},
	Series = {NATO Adv. Sci. Inst. Ser. C Math. Phys. Sci.},
	Title = {The definition of conformal field theory},
	Volume = {250},
	Year = {1988}}

@article{Seg68,
	Author = {Segal, Graeme},
	Fjournal = {Institut des Hautes \'{E}tudes Scientifiques. Publications Math\'{e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes \'{E}tudes Sci. Publ. Math.},
	Mrclass = {55.52},
	Mrnumber = {0232393},
	Mrreviewer = {A. K. Bousfield},
	Number = {34},
	Pages = {105--112},
	Title = {Classifying spaces and spectral sequences},
	Url = {http://www.numdam.org/item?id=PMIHES_1968__34__105_0},
	Year = {1968},
	Bdsk-Url-1 = {http://www.numdam.org/item?id=PMIHES_1968__34__105_0}}

@incollection{Seg04,
	Author = {Segal, Graeme},
	Booktitle = {Topology, geometry and quantum field theory},
	Mrclass = {81T40 (57R56 81T45)},
	Mrnumber = {2079383},
	Mrreviewer = {Thomas M. Fiore},
	Pages = {421--577},
	Publisher = {Cambridge Univ. Press, Cambridge},
	Series = {London Math. Soc. Lecture Note Ser.},
	Title = {The definition of conformal field theory},
	Volume = {308},
	Year = {2004}}

@article{VSL15,
	Author = {Vagner, Dmitry and Spivak, David I. and Lerman, Eugene},
	Fjournal = {Theory and Applications of Categories},
	Issn = {1201-561X},
	Journal = {Theory Appl. Categ.},
	Mrclass = {93A30 (18D50 37A99)},
	Mrnumber = {3431301},
	Mrreviewer = {R. Gylys},
	Pages = {Paper No. 51, 1793--1822},
	Title = {Algebras of open dynamical systems on the operad of wiring diagrams},
	Volume = {30},
	Year = {2015}}

@article{Val07,
	Author = {Vallette, Bruno},
	Doi = {10.1090/S0002-9947-07-04182-7},
	Fjournal = {Transactions of the American Mathematical Society},
	Issn = {0002-9947},
	Journal = {Trans. Amer. Math. Soc.},
	Mrclass = {18D50 (16W30 17B62 55P48)},
	Mrnumber = {2320654},
	Mrreviewer = {Eugen Paal},
	Number = {10},
	Pages = {4865--4943},
	Title = {A {K}oszul duality for {PROP}s},
	Url = {https://doi.org/10.1090/S0002-9947-07-04182-7},
	Volume = {359},
	Year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.1090/S0002-9947-07-04182-7}}

@article{Web07,
	Author = {Weber, Mark},
	Fjournal = {Theory and Applications of Categories},
	Issn = {1201-561X},
	Journal = {Theory Appl. Categ.},
	Mrclass = {18D50 (55P48)},
	Mrnumber = {2369114},
	Mrreviewer = {R. H. Street},
	Pages = {No. 22, 665--732},
	Title = {Familial 2-functors and parametric right adjoints},
	Volume = {18},
	Year = {2007}}

@book{JY15,
	Author = {Yau, Donald and Johnson, Mark W.},
	Doi = {10.1090/surv/203},
	Isbn = {978-1-4704-2197-7},
	Mrclass = {18D99 (13D10 55U40 81T30)},
	Mrnumber = {3329226},
	Mrreviewer = {Bruno Vallette},
	Pages = {xxxii+311},
	Publisher = {American Mathematical Society, Providence, RI},
	Series = {Mathematical Surveys and Monographs},
	Title = {A foundation for {PROP}s, algebras, and modules},
	Url = {https://doi.org/10.1090/surv/203},
	Volume = {203},
	Year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1090/surv/203}}

@article{BFMS17,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv171100037B},
	Archiveprefix = {arXiv},
	Author = {{Baez}, John C. and {Foley}, John and {Moeller}, Joseph and {Pollard}, Blake S.},
	Eid = {arXiv:1711.00037},
	Eprint = {1711.00037},
	Journal = {arXiv e-prints},
	Keywords = {Mathematics - Category Theory},
	Month = {Oct},
	Pages = {arXiv:1711.00037},
	Primaryclass = {math.CT},
	Title = {{Network Models}},
	Year = {2017}}

@article{HLR19,
	Author = {Hess, K., and Levi, R. and Raynor, S.},
	Fjournal = {In preparation},
	Journal = {In preparation},
	Title = {Enriched categories of plastic networks},
	Year = {2019}}
	

